Inspection planning under execution uncertainty

Autonomous inspection tasks necessitate path-planning algorithms to efficiently gather observations from points of interest (POI). However, localization errors commonly encountered in urban environments can introduce execution uncertainty, posing challenges to successfully completing such tasks. Unfortunately, existing algorithms for inspection planning do not explicitly account for execution uncertainty, which can hinder their performance. To bridge this gap, we present IRIS-under uncertainty (IRIS-U^2), the first inspection-planning algorithm that offers statistical guarantees regarding coverage, path length, and collision probability. Our approach builds upon IRIS -- our framework for deterministic inspection planning, which is highly efficient and provably asymptotically-optimal. The extension to the much more involved uncertain setting is achieved by a refined search procedure that estimates POI coverage probabilities using Monte Carlo (MC) sampling. The efficacy of IRIS-U^2 is demonstrated through a case study focusing on structural inspections of bridges. Our approach exhibits improved expected coverage, reduced collision probability, and yields increasingly precise statistical guarantees as the number of MC samples grows. Furthermore, we demonstrate the potential advantages of computing bounded sub-optimal solutions to reduce computation time while maintaining statistical guarantees.

==> sections/Algorithmic_background_old.tex <==
\section{Algorithmic background}
\label{Sec:Algorithmic background}
\OS{This is almost word-by-word self plagiarized from the ICRA21 paper-reword}

In this section, we provide some algorithmic background.
We start (Sec.~\ref{subsec:iris}) by describing \iris~\cite{fu2019toward, FuSA21}, a state-of-the-art inspection-planning algorithm that we will used to solve Prob.~\ref{prob-1}.
%
We then continue (Sec.~\ref{subsec:MC-methods}) to review key statistical concepts that will be used in our analysis.

\subsection{Incremental Random Inspection-roadmap Search (\iris)}
\label{subsec:iris}
\iris solves the continuous inspection-planning problem when there is no uncertainty.  It incrementally constructs a sequence of increasingly-dense graphs, or roadmaps, embedded in the C-space and computes an inspection plan over the roadmaps as they are constructed. 
%
To build the roadmap, \iris builds an \algname{RRG}~\cite{Karaman2011_IJRR} rooted at the start configuration. %
Computing an optimal-inspection plan on a roadmap~$\G = (\V, \E)$ with~$n$ vertices is computationally hard because we need to compute the shortest path on a so-called \textit{inspection graph}.
Here, each vertex corresponds to a vertex $v \in \V$ of the original graph $\G$ and a subset $I$ of  $\I$, representing a path ending at $v$ while inspecting $I$.
% 
Thus, the inspection graph has $O(n\times \vert2^{\I}\vert)$ vertices.
% 
%\IF{should that be $n^{|\I|}$?}\MF{Yes, you are correct.}
% 
To search this inspection graph,  \iris employs a novel search algorithm that approximates~$\pi^*$, the optimal inspection path on the graph. 
%
To this end, \iris uses two parameters, $\eps$ and $p$, to ensure that the path obtained from the graph-search phase is no longer than $1+\eps$ the length of~$\pi^*$ and covers at least $p$ percent of the POIs covered by~$\pi^*$.
% 
To ensure convergence to the optimal inspection path, $\eps$ is reduced and $p$ is increased between search iterations. This is referred to as \emph{tightening} the approximation factors.

We now briefly describe the graph-search algorithm as it is key to understanding the algorithmic contributions of this work.
% 
For an in-depth description of the search algorithm, the rest of the framework, and its theoretical guarantees, see~\cite{fu2019toward, FuSA21}. 
%
The search runs an \algname{A*}-like search~\cite{Hart1968_TSSC} but instead of having each node%
\footnote{A node, representing a search state, is different from a vertex, representing a configuration in the underlying roadmap.}
represent a path from the start vertex $\mathbf{q}_s$, each node is a \emph{path pair} \pp that is composed of a so-called \textit{achievable path} (\ap) and \textit{potentially achievable path} (\pap).
% 
As its name suggests, an \ap represents a path in the graph from $\mathbf{q}_s$.
% 
In contrast, a \pap is not necessarily realizable and is used to bound the quality of paths represented by a specific \pp.
% 
A $\pp = (P, \tilde{P})$, where $P$ is the \ap and $\tilde{P}$ is the \pap, is said to be \ep-bounded if 
% (i)~the cost of the \ap is no more than $1+\eps$ the cost of the \pap 
(i) $\ell(P) \leq (1+\eps)\ell(\tilde{P})$
and
% (ii)~the coverage of the \pap is at least $p$-percent the coverage of the \pap.
(ii)~$\vert\S(P)\vert \geq p\cdot\vert\S(\tilde{P})\vert$.

Similar to \algname{A*}, the algorithm uses an OPEN and CLOSED list to track nodes that have not and have been considered, respectively.
% 
It starts with the trivial path pair, $\pp_{\mathbf{q}_s}$, where both \ap and \pap represent the trivial path $\{\mathbf{q}_s\}$.

At each iteration, it pops a node from the OPEN list, and checks if the search can terminate. If not, the node is \emph{extended} and added to the CLOSED list. 
% 
While doing so, the algorithm tests if successor nodes can \emph{subsume} or be \emph{subsumed} by another node. 
% 
These two core operations (extending and subsuming) are key to the efficiency of the algorithm and we now elaborate on them for a given path pair $\pp_u = (P_u, \tilde{P_u})$ (here $P_u$ is \ap and $\tilde{P_u}$ is \pap):
\begin{enumerate}
    \item 
    \textbf{Extending operation:} 
    Extending $\pp_u$ by edge $e = (u,v) \in \E$ 
    (denoted $\pp_u + e$) 
    will extend both $P_u$ and $\tilde{P_u}$ by edge $e$. 
    The resulting path pair is $\pp_v = (P_v, \tilde{P_v})$, where 
    the \ap satisfies 
    $\S(P_v) = \S(P_u) \cup \S(v), \ell(P_v) = \ell(P_u) + \ell(e)$,
    and the \pap satisfies 
    $\S(\tilde{P_v}) = \S(\tilde{P_u}) \cup \S(v), \ell(\tilde{P_v}) = \ell(\tilde{P_u}) + \ell(e)$.
    % 
    \item \textbf{Subsuming operation:} 
    Given two path pairs $\pp_1= (P_1, \tilde{P_1})$ and $\pp_2 = (P_2, \tilde{P_2})$ that end at the same vertex, 
    the operation of $\pp_1$ subsuming $\pp_2$ 
    (denoted $\pp_1 \oplus \pp_2$) 
    will create a new path pair 
    % 
    $\pp_1\oplus\pp_2 := \left(P_1, \left(\S(\tilde{P_1}) \cup \S(\tilde{P_2}), \min(\ell(\tilde{P_1}), \ell(\tilde{P_2}))\right)\right)$.
    % 
\end{enumerate}
Roughly speaking, the subsuming operation allows to reduce the number of paths considered by the search.
However, to ensure that the solution returned by the algorithm approximates the optimal inspection path, subsuming only occurs when the resultant \pp is \ep-bounded.

\subsection{Monte-Carlo methods and statistical method}
\label{subsec:Monte-Carlo methods statistical tests}
Monte-Carlo methods are a common tool to estimate and bound stochastic values and processes by  repeated random sampling to obtain numerical results. These results are then used to \emph{estimate} the true (unknown) values. 

Estimation is typically done using the notion of \emph{confidence intervals} (CI) and \emph{confidence levels} (CL)~\cite{hazra2017using}~\cite{neyman1937outline}.
Roughly speaking, The CL is the percentage of times expected to get close (defined via the CI) to the value estimated while the CI consists of the upper and lower bounds of estimates expected to find at a given CL.

In our setting we will consider the estimation of both the mean and success probability of random processes.
To do so, we will use $Z^*(\cdot)$ and $T^*(\cdot)$, the so-called ``critical points'' for the z-distribution and t-distribution that can be evaluated for any value using statistical tables~\cite{}.
    
\begin{enumerate}
    \item \textbf{Mean calculation:} 
    Let $X$ be some random process with unknown mean value~$\bar{x}$.
    Let $x_1, \ldots, x_m$ be $m$ samples drawn from $X$ and let 
    $\hat{x}$ and $\hat{s}$ be their mean and standard variation  respectively.
    %
    For any $\alpha \in [0,1]$ we can say with CL of~$1-\alpha$ that~$\bar{x}$, the true unknown mean value of $X$   is within the following CI:
    \begin{equation}\label{eq:CI_calculation_value}
        \text{CI}(CL):=\hat{x} \pm Z^*(CL) \cdot \left( \hat{s} / \sqrt{m} \right).
    \end{equation}
    
    \item \textbf{Success probability calculation:} 
    Let $X$ be a random variable whose true unknown probability of success is~$\bar{p}$.
    Let $x_1, \ldots, x_m$ be the outcome of $m$ samples drawn from $X$ (i.e., $x_i \in \{0, 1 \}$)
    and let $\hat{p}$ be the estimated success probability.
    %
    For any $\alpha \in [0,1]$ we can say with CL of~$1-\alpha$ that~$\bar{p}$, the true unknown success probability  of $X$ is within the following CI:
    \begin{equation}\label{eq:CI_calculation_proportions}
        \text{CI}(CL):=\hat{p} \pm Z^*(CL) \cdot \sqrt{\frac{\hat{p}(1-\hat{p})}{m}}.
    \end{equation}
\end{enumerate}


\subsection{Null Hypothesis Testing}
\label{subsec:Null Hypothesis Testing}


The so-called \emph{null hypothesis}, denoted as~$H_0$ is a typical statistical theory which suggests that two samples are identical. 
%
The so-called alternate hypothesis, denoted as $H_1$, is the mutually-exclusive hypotheses.

\emph{Null hypothesis testing} is a formal approach to deciding between $H_0$ and $H_1$.
One of its outcome is the so-called \emph{$p$-value} which indicates you how likely the data observed is to have occurred under the null hypothesis.
All these tests are based on the same general logic in which we assume that the null hypothesis is true and determine how likely the specific sample relationship would be if the null hypothesis were true.
If the sample relationship would be extremely unlikely, then we reject $H_0$ and retain $H_1$ and vice versa if it would not be extremely unlikely.

In our setting we will be interested in null hypothesis testing in the context of comparing either 
the mean of two population's samples or 
two proportion's samples.
%
Specifically, 
\begin{enumerate}
    \item \textbf{Comparing the mean of two sample sets:} 
    Let $X$ and~$Y$ be random processes with unknown mean values~$\bar{x}$ and~$\bar{y}$, respectively
    Let $x_1, \ldots, x_n$ and 
    $y_1, \ldots y_m$
    be $n$ and $m$ samples drawn from $X$ and $y$, respectively and let 
    $\hat{x}$, $\hat{y}$ and $\hat{s_X}$ and $\hat{s_Y}$ be their means and standard variations  respectively.
    %
    Here, the null hypothesis is~$H_0:= \bar{x} =\bar{y}$ (namely, that both sample sets have the same mean), and the alternative hypothesis is~$H_1:=\bar{x} \geq \bar{y}$.
    %
   \textcolor{red}
   {
   Consequently, we denote the $p$-value in this setting as~$\gamma$, such that:
    % \begin{equation}
    % \label{eq:p-value-populations}
    %     \alpha(\bar{X} \geq \bar{Y}):=\probP(\underbrace{\hat{X} \geq \hat{Y}}_{H_1} \vert \underbrace{\bar{X} = \bar{Y}}_{H_0}).
    % \end{equation}
    \begin{equation}
    \label{eq:p-value-populations}
        \gamma(\underbrace{\hat{X} \geq \hat{Y}}_{\text{Data observed}}):=\probP(\hat{X} \geq \hat{Y} \vert \underbrace{\bar{X} = \bar{Y}}_{H_0}).
    \end{equation}
    }
    
    To evaluate Eq.~\ref{eq:p-value-populations} we use the so-called \emph{t-test} method~\cite{cressie1986use} where we compute 
    \begin{equation}
        %t = \frac{\hat{X} - \hat{Y}}{\sqrt{\frac{\hat{s}_X^2}{n}+\frac{\hat{s}_Y^2}{n}}}.
        t = \frac{\hat{x} - \hat{y}}{\sqrt{{\hat{s}_x^2} / {n} + {\hat{s}_y^2} / {m}}},
    \end{equation}
      \textcolor{red}
   {
    and the computed value of~$t$ produces the p-value~$\gamma(\bar{X} \geq \bar{Y})$ using the standard t-statistic tables.
%
    Now, let's define a desire significant level as~$\pval_\text{sl}$. Then, given the produced value of~$\gamma(\bar{X} \geq \bar{Y})$, and the threshold value of~$\pval_\text{sl}$ we can evaluate whether to reject the null hypothesis. 
    That is, we reject the null hypothesis if~$\gamma(\bar{X} \geq \bar{Y}) \textless \pval_\text{sl}$.
    }
    % and for any desired confidence level $1 - \alpha$, the computed value of~$t$ can then be compared against threshold values available in standard t-statistic tables to evaluate whether to reject the null hypothesis. 
    
    \item \textbf{Comparing success probabilities of two sample sets:}
    Let $X$ and $Y$ be a random variable whose true unknown probability of success is~$\bar{p_x}$ and~$\bar{p_y}$, respectively.
    Let $x_1, \ldots, x_n$ and $y_1, \ldots, y_m$ be the outcome of $n$ and~$m$ samples drawn from $X$ and $Y$, respectively 
    and let $\hat{p}_x$ and $\hat{p}_y$ be their estimated success probability, respectively.
    %
    Here, the null hypothesis is~$H_0:= \bar{p}_x =\bar{p}_y$ (namely, that both sample sets have the same probability of success), and the alternative hypothesis is~$H_1:=\bar{p}_x \geq \bar{p}_y$.
    %
    To evaluate the  $p$-value in this setting we use again the  t-test but in this setting $t$ is defined to be 
    \begin{equation}
        t = \frac{\hat{p}_x - \hat{p}_y}
                 {\sqrt{
                    \hat{p}_x \cdot (1 - \hat{p}_x) / n
                    +
                    \hat{p}_y \cdot (1 - \hat{p}_y) / n
                 }}.
    \end{equation}
    
\end{enumerate}



\subsection{False discovery rate \OS{alt sec}}
\label{subsec:False discovery rate}
Recall that the $p$-value is the probability of obtaining test results at least as extreme as the result actually observed, under the assumption that the null hypothesis is correct. This is also known as a \emph{false positives} (FP) result. 
%
When performing the comparison several times, we need to consider the multiple hypotheses setting. This is done using the notion of \emph{false discovery rate} (FDR) which indicates how many of the significant results will be false positives.
That is, the FDR is the expected ratio between the number of FP classifications and the total number of positive classifications which include both false positives (FP) and true positives (TP). Namely:
$$\text{FDR = FP / (FP + TP)}.$$

\OS{following paragraph is still untouched}


The desired value of the FDR is~$1$ such that there will not be any TP results. There are several method to control the FDR to equal~$1$ and a common method is Benjamini–Hochberg (BH) method~\cite{benjamini1995controlling}.
That is, let's define~$\pval_\text{BH}$ to be the threshold required value of BH method. Then, given~$d$ number of comparison tests with~$d$ p-value results, the BH is performed in the following way:
\begin{enumerate}
    \item List the p-values in ascending order and denote them as~$\pval_1,\pval_2,\ldots,\pval_d$.
    \item For a given~$\pval_\text{BH}$, and for~$i=1,2,\ldots,d$ find the largest~$i$ such that~$\pval_i \leq \frac{i}{d} \cdot \pval_\text{BH}$.
    \item Reject the null hypothesis only for~$1,\ldots,i$ tests.
\end{enumerate}



% \subsection{Monte Carlo methods}
% \label{subsec:MC-methods}
% Monte Carlo methods are a very common concept for quantifying values in various areas such as predictive modeling.
% This method leverages distributions of probability (Normal, Gaussian, Uniform, etc.) for any variable which has uncertainty. Based on the number of samples specified, this process of using random values is repeated numerous times, and as the more samples, the higher likelihood the outcome will converge to a value.
% % Using this method makes it possible to test the estimation quality by a statistical hypothesis testing~\cite{lehmann2005testing}.

% Generally, we can use the Confidence interval (CI) and confidence level (CL) approach~\cite{hazra2017using}~\cite{neyman1937outline}
% to estimate with CL that the output value is within some CI depending on the number of the MC samples.
% The CL is usually represented by z-statistic denote as~$Z^*(CL)$, but for small MC sample it is represented by t-statistic denote as~$T^*(CL)$ (For instance,~$Z^*(0.95) = 1.96$). 

% There are two different cases: 
% (i) \emph{Mean calculation} and 
% (ii) \emph{success probability calculation}:
% \begin{enumerate}
%     \item \textbf{Mean calculation:} Given~$m$ samples with a mean estimated value~$\hat{x}$ and estimated standard deviation~$\hat{s}$ we can say with CL of~$1-\alpha$ that the true unknown mean value~$\bar{x}$ is within the following CI:
%     \begin{equation}\label{eq:CI_calculation_value}
%         \text{CI}:=\hat{x} \pm Z^*(\text{CL})\frac{\hat{s}}{\sqrt{m}}.
%     \end{equation}
%     \item \textbf{Success probability calculation:} Given~$m$ samples with estimated success probability~$\hat{p}$ we can say with CL of~$1-\alpha$ that the true unknown success probability~$\bar{p}$ is within the following CI:
%     \begin{equation}\label{eq:CI_calculation_proportions}
%         \text{CI}:=\hat{p} \pm Z^*(\text{CL})\sqrt{\frac{\hat{p}(1-\hat{p})}{m}}
%     \end{equation}
% \end{enumerate}




% \subsection{Null Hypothesis Testing}
% \label{subsec:Null Hypothesis Testing}
% The null hypothesis denote as~$H_0$ is that the true excepted value of two different samples are equal. In addition, there is an alternative hypothesis denote as~$H_1$ that two different samples are has different values.
% The null hypothesis test produces a p-value probability (called also type I error or false positives (FP) result) to get the alternative hypothesis~$H_1$ though null hypothesis~$H_0$ is true. 

% Here, we mention it in the context of two types of tests:
% (i) Comparison of two populations' samples, and (ii) Comparison of two proportions' samples.

% In the first test, we assume to be given two sample group~$X$ and~$Y$, with~$n$ and~$m$ samples, where the null  hypothesis is~$H_0:= \bar{X} =\bar{Y} $, and the alternative hypothesis~$H_1:=\bar{X} \geq \bar{Y}$. 
% In this type of test we use \emph{two-Sample t-test} method~\cite{cressie1986use} that produce a p-value denoted as:
% \begin{equation}\label{eq:p-value-populations}
%  \alpha(\bar{X} \geq \bar{Y}):=\probP(\hat{X} \geq \hat{Y} \vert \bar{X} = \bar{Y}),
% \end{equation}
% where, the term~$\bar{X} \geq \bar{Y}$ is indicate the~$H_1$ hypothesis and~$H_0$ is~$\bar{X} =\bar{Y}$.

% We first calculate the value of~$t$ defined by:
% \begin{equation}
%     t = \frac{\hat{X} - \hat{Y}}{\sqrt{\frac{\hat{s}_X^2}{n}+\frac{\hat{s}_Y^2}{n}}}.
% \end{equation}
% The value of~$t$ is the input of t-statistic table that produces the probability of~$\alpha(\bar{X} \geq \bar{Y})$. 
% Then, we have probability of~$\alpha(\bar{X} \geq \bar{Y})$ to get the alternative hypothesis~$H_1:=\bar{X} \geq \bar{Y}$ though null hypothesis~$H_0:= \bar{X} -\bar{Y} = 0$ is true.

% Similarly for the second test, we assume to be given two sample group~$p_1$ and~$p_2$, with~$n$ and~$m$ samples, we have a null hypothesis~$H_0:= \bar{p}_1 -\bar{p}_2 = 0$ and an alternative hypothesis~$H_1:=\bar{p}_1 \geq \bar{p}_2$.
% Thus we defined this test as:
% \begin{equation}\label{eq:p-value-proportions}
%     \alpha(\bar{p}_1 \geq \bar{p}_2):=\probP(\hat{p}_1 \geq \hat{p}_2 \vert \bar{p}_1 = \bar{p}_2).
% \end{equation}
% Then, given the estimated values~$\hat{p}_1$ and~$\hat{p}_2$ we define~$t$ as:
% \begin{equation}
%     t = \frac{\hat{p}_1 -\hat{p}_2-0}
%              {
%              \sqrt{
%              \frac{\hat{p}_1 \cdot (1-\hat{p}_1)}{n_1} +
%              \frac{\hat{p}_2 \cdot (1-\hat{p}_2)}{n_2}
%              }
%              },
% \end{equation}
% Then, we say that we have probability of~$\alpha(\bar{p}_1 \geq \bar{p}_2)$ to get the alternative hypothesis~$H_1:=\bar{p}_1 \geq \bar{p}_2$ though null hypothesis~$H_0:= \bar{p}_1 -\bar{p}_2 = 0$ is true.

% Finally, it is common to define significance level threshold~$\tau_{\alpha}$ and say that if~$\{\alpha(\bar{X}~\geq~\bar{Y})~\text{or}~\alpha(\bar{p}_1 \geq \bar{p}_2)\} \leq \tau_{\alpha}$, is interpreted as indicating evidence that~$\bar{X} \geq \bar{Y}$ or~$\bar{p}_1 \geq \bar{p}_2$.

% \subsection{False discovery rate}
% \label{subsec:False discovery rate}
% As stated, the p-value is the result of the comparison between two samples that called also the false positives (FP) result. However, when performing the comparison several times, we need to consider the probabilities of multiple hypotheses.
% To this end, we use the definition of false discovery rate (FDR).
% The FDR indicates how many of the significant results will be false positives.
% That is, the FDR is the expected ratio of the number of FP classifications to the total number of positive classifications which include both false positives (FP) and true positives (TP). Namely:
% $$\text{FDR = FP / (FP + TP)}.$$

% There are several method to control the FDR to be less than a threshold required value and a common method is Benjamini–Hochberg (BH) method~\cite{benjamini1995controlling}.
% That is, let define~$\tau_\text{BH}$ to be the threshold required value of BH method. Then, given~$d$ number of significant results (that exceeds the significance level threshold~$\tau_{\alpha}$), the BH is performed in the following way:
% \begin{enumerate}
%     \item List the p-values in ascending order and denote them as~$\pval_1,\pval_2,\ldots,d$.
%     \item For a given~$\tau_\text{BH}$, and for~$i=1,2,\ldots,d$ find the largest~$i$ such that~$\pval_i \leq \frac{i}{d} \cdot \tau_\text{BH}$.
%     \item Reject the null hypothesis for all~$1,\ldots,i$ tests.
% \end{enumerate}

% Then, we say that the expected false positives result from those~$i$ significant results is less or equal to~$\tau_\text{BH}$.

% \DA{We can save in an array only the~$\max \pval_i$ and test if~$\pval_i \leq \frac{1}{d} \cdot \tau_{\alpha}$. However, this is a tough requirement (especially for high values of~$d$.}




























==> sections/Introduction.tex <==
\section{Introduction and related work}
\label{Sec:Introduction and related work}
We consider the problem of planning in an offline phase a collision-free path for a robot to inspect a set of \emph{points of interest}~(POIs) using onboard sensors.
This can be a challenging task, especially in urban environments as dynamics (e.g.,  control constraints) and localization errors (e.g., inaccuracies in location estimates) increase the task's complexity. In particular, localization can be a significant source of uncertainty in urban environments, leading to missed POIs and compromising the efficiency and accuracy of inspection missions.

One application that motivates this work is the inspection of bridges using \emph{unmanned aerial vehicles}~(UAVs)~\cite{bircher2016three}. Almost~$40\%$ of the bridges in the United States of America exceed their~$50$-year design life~\cite{mcguire2016bridge}, and regular inspections are critical to ensuring bridge safety. UAVs, or drones, can be used to efficiently inspect the bridge structure, allowing it to be visually assessed at close range without the need for human inspectors to walk across the deck or utilize under-bridge inspection units~\cite{chan2015towards}.
%
In such settings, the UAV is usually equipped with a camera to inspect the POIs, and a navigation system to determine its location.
The navigation system typically fuses information from different sensors such as a \emph{global navigation satellite system}~(GNSS) and inertial sensors. However, GNSS signals can be blocked or distorted by the bridge, leading to location inaccuracies that rely mainly on inertial measurements and can compromise the effectiveness of the inspection mission (see Fig.~\ref{fig:figure12}).
% \begin{figure}[t!]
%    \centering
%          \centering
%          % \begin{subfigure}
%          \includegraphics[width=0.5\textwidth]{figs/Figure1.png}
%          % \includegraphics[width=0.5\textwidth]{figs/Figure1_draft.jpeg}
%           % \includegraphics[width=0.5\textwidth]{figs/Figure1_draft1.jpeg}
%          \caption{\DA{update figure} The figure depicts the blue command path and its field of view (FOV) towards the POI strip. Also shown are several possible execution paths in green and the FOV of one of them towards the POI strip. Due to localization uncertainty, the execution paths deviate from the command path, resulting in differences in execution coverage as shown by the color scale at the top of the figure. }
%          \label{fig:figure12}
%            % \end{subfigure}
% \end{figure}

\begin{figure}[t!]
   \centering
         \centering
% \includegraphics[width=0.5\textwidth]{figs/Figure1_update.pdf}
\includegraphics[width=0.5\textwidth]{figs/Figure1_update.eps}
% \fbox{\includegraphics[width=0.5\textwidth,clip]{figs/Figure1_update.pdf}}
         \caption{
         %
         %\DA{How to give credit for the picture? }
         A UAV executing a bridge-inspection task, following a command path pre-computed offline (dark blue). 
         The UAV relies on GNSS satellite signals for navigation but the bridge obstructs one satellite signal during a particular segment of its path (light blue).
         This leades to a substantial deviation from the command path which hinders the UAV's ability to inspect the  POIs and may result in a collision with the bridge.}
         \label{fig:figure12}
\end{figure}

In this study, we aim to address the problem of offline path planning for inspection tasks in urban environments, where uncertainty during mission execution can lead to missed POIs.
Our objective is to devise a method that can pre-compute a path before the inspection mission begins, which serves as a command path robust enough to accommodate uncertainties during execution.

Several approaches have been proposed to perform inspection planning without accounting for uncertainty. Some algorithms decompose the region containing the POIs into sub-regions and solve for each sub-region separately~\cite{galceran2013survey}, while others divide the problem into two NP-hard problems:~(i)~solving the art gallery problem to compute a small set of viewpoints that collectively observe all the POIs, and~(ii)~solving the traveling salesman problem to compute the shortest path to visit this set of viewpoints~\cite{danner2000randomized, englot2010inspection, englot2012sampling, papachristos2019autonomous}. Another common approach is to simultaneously compute both inspection points (i.e., points from which POIs are inspected) and the trajectory to visit these inspection points using sampling-based techniques~\cite{papadopoulos2013asymptotically, bircher2017incremental}. However, these approaches do not consider the execution uncertainty, which can lead to missed POIs due to differences between the path executed and the path planned.

Using these methods for planning with low uncertainty can be done using an upgraded navigation system that relies on RF tools like WIFI~\cite{sun2014wifi}, Bluetooth~\cite{rida2015indoor}, or acoustic waves~\cite{whitcomb1999combined}, or more expensive and heavy sensors like mobile LIDAR mapping~\cite{haala2008mobile}, or tactical grade inertial sensors and RTK/dGNSS~\cite{klein2011vehicle}. However, these solutions may require a supportive communication infrastructure or more expensive and heavy sensors.
% Using these methods for planning with low uncertainty can be done using an upgraded navigation system that does not rely on GNSS, such as RF tools like WIFI~\cite{sun2014wifi}, Bluetooth~\cite{rida2015indoor}, or acoustic waves~\cite{whitcomb1999combined}, or more expensive and heavy sensors like mobile LIDAR mapping~\cite{haala2008mobile}, visual odometry and SLAM techniques, or tactical grade inertial sensors and RTK/dGNSS~\cite{klein2011vehicle}. However, these solutions may require a supportive communication infrastructure or more expensive and heavy sensors.

Various approaches have been proposed to address localization uncertainty for safe path planning (which only considers a motion between states without inspection points).
For instance, minimum-distance collision-free paths can be computed while bounding the uncertainty by, e.g., a self-localization error ellipsoid, or uncertainty corridor~\cite{pepy2006safe, alami1994planning, candido2010minimum}. 
Another approach~\cite{delamer2019solving}, uses a mixed-observability Markov decision process approach to account for a-priori probabilistic sensor availability and path execution error propagation.
Englot et al.~\cite{englot2016sampling} suggest an RRT*-based method which minimizes the maximum uncertainty of any path segment along a path. Sampling-based planners that explicitly reason about the evolution of the robot's belief have also been proposed~\cite{Wu.ea.22,zheng2023ibbt,DBLP:conf/icra/HoSL22,DBLP:journals/trob/PedramFT23}.
% suggest a method called Informed Batch Belief Trees (IBBT) that produces motion plans under uncertainty from a start position to a goal position in the so-called belief space.

\check{Inspection tasks introduce further complications as they require reasoning about an exceptionally large search space that captures the interaction between the POIs locations, the locations from which POIs can be inspected, and the order of visitation. As a result, the computational complexity of inspection planning can be quite large, even in the absence of localization uncertainty~\cite{bircher2017incremental,DBLP:journals/ijrr/FuKSA23}.} 
\check{In our previous work, we introduced the \iris algorithm, which is a highly effective approach for deterministic inspection planning~\cite{DBLP:journals/ijrr/FuKSA23}. Importantly, \iris has guarantees asymptotic convergence to optimal oslutions while being several orders of magnitude faster than previous work providing similar guarantees. Unfortunately, extending \iris to the uncertain setting is highly nontrivial.}
%

\check{Roughly speaking, this is because  the efficiency of \iris is due to a novel graph-search algorithm that searches in the space of possible paths. The search is guided by reasoning about which POIs have been seen along any given path. Thus, accounting for location uncertainty (as is commonly done) and not inspection uncertainty does not suffice. The crux of the problem is how to (i)~account for and compute inspection uncertainty and (ii)~how to integrate this measure into \iris in a systematic way. 
%
To illustrate the complexity of this challenge, consider that \iris operates within a discrete roadmap, representing a finite set of paths computable by the algorithm, albeit exponentially large. However, when factoring in uncertainties, the paths actually traversed by the robot may diverge from this predefined roadmap.
}




However, when it comes to localization uncertainty in inspection tasks, additional challenges arise due to the uncertainty of inspecting the POIs. 
Papachristos et al.~\cite{papachristos2019autonomous} proposed a planner that propagates the covariance matrix of the \emph{extended Kalman filter}~(EKF) to maintain a belief state about the robot's location and the POI inspected.
%
However, while this approach excels in online scenarios where it can utilize real-time measurements, it may encounter challenges in offline inspection planning where the planning process occurs before the actual execution.
% Specifically, during offline planning, the covariance matrix may include regions where GNSS outages are expected\kiril{This statement is a bit unclear; shouldn't different areas have different matrices?}, despite the availability of complete GNSS-INS measurements in a specific online scenario. If the planned path passes through these regions during execution, the robot may experience GNSS outages, leading to increased localization errors and potentially compromising the inspection task.
%\begin{color}{red}
    Specifically, the covariance matrix is established based on a specific online scenario, utilizing received GNSS signals, and it characterizes the extent of uncertainty associated with the localization process tied that of a particular signal. Consequently, this uncertainty may encompass areas where GNSS outages are anticipated but not pertinent within the context of that specific scenario. However, when transitioning from an offline planning phase to an execution phase, there's a possibility that new localization errors can emerge, distinct from those encountered during the offline planning phase and potentially compromising the inspection task. \kiril{This paragraph should be rewritten. I don't understand it. I've also looked into the paper and their approach for inspection doesn't seem to explicitly account for uncertainty. If this is the case, we should revise this paragraph stating that there are no other algorithms that account for uncertainty. Please check me on that.}
    \DA{In their paper there is no inspection planning under localization uncertainty: It handle the following:
    \begin{itemize}
        \item autonomous area exploration and mapping when no prior knowledge of the environment is available
        \item informative path planning for terrain monitoring
        \item full coverage inspection planning provided a prior model of the environment.
    \end{itemize}
    The third algorithm is similar to our problem (inspection planning) and as I understand it, it does not consider uncertainty.
    The first algorithm goal is to map an unknown area. However, this algorithm considers uncertainty (and also the uncertainty in viewing the desired landmarks) while mapping an unknown area. Thus, I mention this approach to handling localization uncertainty even if it is a different problem. In addition, this problem is an online problem and it can be solved via the covariance matrix of the EKF, and this is what I wrote in the former paragraph.
    In addition, in the field of path planning under uncertainty, this is a common approach to handling the uncertainty via the covariance matrix of the EKF. Here (in an offline mission), using the EKF can cause to miss POI.
    \textbf{Maybe we should consider this approach of handling uncertainty as the base-line algorithm??}
    However, I don't know how we can use it and simulate this approach without MC since we need to check if we can see POIs from the robot location.
    }
    
     
    %that the robot's trajectory could intersect with the uncertainty region within the covariance matrix, potentially coinciding with areas affected by GNSS outages. This situation can lead to the emergence of different location errors, distinct from those encountered during the offline planning phase and potentially compromising the inspection task.
%\end{color}



% To address this, Papachristos et. al~\cite{papachristos2019autonomous} proposed the Structural Inspection Planner (SIPlanner) algorithm. This algorithm takes a two-step approach by computing an Autonomous Global Plan (AGP) followed by solving a Travelling Salesman Problem (TSP), which plans a path through a small set of viewpoints while maintaining low localization uncertainty. Nonetheless, even a small localization uncertainty can cause some POIs to be missed, particularly in the presence of obstacles, making full coverage unattainable.

% \begin{color}{red}
\vspace{5pt}
\noindent \textbf{Contribution.}
\check{We present \iris-under uncertainty ({\irisuu})---the first algorithm for offline inspection planning that systematically accounts for execution uncertainty. Our algorithm combines the capabilities of (i) \iris, which efficiently explores the space of high-quality inspection plans in the deterministic setting, together with (ii) \emph{Monte Carlo}~(MC) sampling to reason about uncertainty via POI inspection probabilities. Importantly, our approach does not merely utilize those two components in a decoupled manner, by, e.g., interleaving between planning and uncertainty estimation~\cite{?} \kiril{find citation}, but rather uses the uncertainty to guide the exploration of the search space.} \kiril{Perhaps a stronger or more precise description can be given?} \check{During its run \irisuu efficiently reasons about a variety of possible paths produced by MC samples and estimates POI inspection probabilities,  collision probabilities, and path length. 
  To integrate those probabilities within a search-based approach in a computationally efficient manner we develop novel mechanisms for extending, subsuming and dominating nodes.  This transformed probability then serves as the optimization objective for the algorithm.}


On the theoretical side, \irisuu estimates with a certain \emph{confidence level}~(CL) the desired performance criteria (i.e., path length, coverage, and collision probabilities)  within some \emph{confidence interval}~(CI) depending on the number of the MC samples used~\cite{hazra2017using}. 
%
However, when selecting an execution path from multiple optional paths, straightforward statistical analysis may be biased toward false negatives and either require offline prepossessing to provide guarantees or should be used as guidelines (see details in Appendix~\ref{subsec:Illustrative example for possible false negatives}). 
%
We choose the latter approach and outline a procedure to set a user-defined parameter for providing a CI, which becomes tighter as the number of samples increases and which becomes true asymptotically.
%
Additionally, we highlight the potential benefits of using a bounded sub-optimal solution in certain situations to reduce computation time while still providing guarantees through the CI boundaries.

We demonstrate the effectiveness of \irisuu through a simulated case study of structural inspections of bridges using a UAV in an urban environment. Our results show that \irisuu is able to achieve a desired level of coverage, while also reducing collision probability and tightening the CI lower boundaries as the number of MC samples increases. 


The rest of this paper is organized as follows. In Sec.~\ref{Sec:ProblemDefinition}, we formulate the problem of offline path planning for inspection tasks under execution uncertainty. In Sec.~\ref{Sec:Algorithmic background}, we describe the algorithmic background and in Sec.~\ref{sec:method} we describe our proposed approach in detail. 
Then in Sec.~\ref{Sec:DemoScenario} and~\ref{Sec:BridgeScenario} we present the results of our simulated experiments. Finally, in Sec.~\ref{Sec:Conclusion and future work}, we summarize our main contributions and discuss future work.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/MethodOld.tex <==
\section{Methods}
\label{sec:method}
In this section, we present our method \emph{IRIS-under-uncertainty},~\irisuu, that expands \iris to consider the execution uncertainty within the inspection-planning algorithm.




\subsection{Algorithmic approach}
\label{subsec:alg-approach}
A common approach to address execution uncertainty is to directly minimize or limit localization uncertainty~\cite{papachristos2019autonomous}.
%
While highly-efficient in collision avoidance, this approach may cause the inspected coverage of the command path and the executed path to dramatically differ, especially in the presence of obstacles (for a visualization, see Fig.~\ref{fig:})
\footnote{\OS{In this figure it would be great to show that due to obstacles even small localization uncertainty can cause dramatic changes in coverage. Thus we would like to see two paths: one that minimizes localization uncertainty and the second which directly maximizes expected coverage.}}. 
%
Thus, instead of reasoning about localization uncertainty, in \irisuu we directly estimate in the offline phase the expected coverage.

\irisuu follows the same algorithmic steps as \iris. Namely, we iteratively build a graph embedded in the search space and compute an inspection path.
%
Then, recall that the output of \iris is a path~$\pi$ that the robot is instructed to visit in the execution stage whose length and coverage are $\ell(\pi)$ and $\mathcal{S}(\pi)$, respectively. In \irisuu we refer to this as the \emph{command path} that due to execution uncertainty (as detailed in Sec.~\ref{Sec:pdef}), may result with a different path in the execution phase. 
%
Then, instead of a known and constant value of~$\ell(\pi)$ and $\mathcal{S}(\pi)$, the algorithm results with 
expected length~$\bar{\ell}(\pi)$ and expected coverage~$\bar{\mathcal{S}}(\pi)$ that were detailed in Eq.~\ref{eq:expected-l} and~\ref{eq:expected-s}.


To account for the inspection uncertainty,~\irisuu takes a Monte-Carlo-approach and maintaining for each path~$\pi$ (represented by a node in the search graph) an estimation of the \emph{probability} that every POI will be inspected (in contrast to discrete set of POIs used by \iris).
%
Specifically, we define for each path~$\pi$ the \emph{inspection probability vector} (IPV):
\begin{equation}
\label{eq:IPV}
    \rm{IPV}(\pi) := \{ \hat{p}_1^\pi, \ldots, \hat{p}_k^\pi \}.
\end{equation}
Here $\hat{p}_j^\pi$ estimates the probability that POI $\iota_j$ is viewed when executing $\pi$.
%
Shifting from sets of POIs inspected to IPVs requires addressing two key challenges:
\begin{itemize}
    \item[\textbf{C1}]
    Given a path $\pi$, how to estimate its IPV and how to use IPVs to compute $\hat{\ell}(\pi)$ and $\vert\mathcal{S}(\pi)\vert$?
    
    \item[\textbf{C2}]
    How to modify the primitive operations used by \iris's search algorithm (namely, extending a node, subsuming a node, and testing if one node dominates another) to account for the IPVs?
\end{itemize}



\subsection{Computing and using IPVs (challenge \textbf{C1})}
\label{subsec:c1}
\subsubsection{Basic notations}
Given a command path $\pi$, we wish to estimate its expected coverage and length by taking a Monte Carlo (MC) approach.
%
Specifically, we initialize our algorithm by sampling~$m$ different parameters $\Nloc^1, \ldots, \Nloc^m$ from~$\Dloc$ and~$m$ different parameters $\Ncon^1, \ldots, \Ncon^m$ from~$\Dcon$.
%
Now, given a command path $\pi$, we estimate $\expL$ and~$\expS$ by simulating~$m$ execution paths $\pi^e_1, \ldots, \pi^e_m$ using the $m$ motion models. Namely, 
\begin{equation}\label{eq:motion_model_paths}
    \pi^e_i:=\mathcal{M}(\pi, \Nloc^i, \Ncon^i).
\end{equation}

Now, set $\xi_{i,j} \in \{0,1\}$ to be a variable that is set to one if path $\pi^e_i$ covers the $j$'th POI.
Namely,
$$
\xi_{i,j}:=
    \begin{cases}
     1 & \iota_j \in \mathcal{S}(\pi^e_i), \\
     0 & \text{else}.
    \end{cases}
$$
%
Finally, the IPV (Eq.~\ref{eq:IPV}) is computed by setting:
\begin{equation}\label{eq:p_pi_j}
    \hat{p}_j^\pi:= 
    \frac{1}{m} \sum_{i=1}^{i=m} \xi_{i,j}.
\end{equation}
%
Now, the estimated expected coverage is defined as:
\begin{equation}\label{eq:estimated expected coverage}
    \vert \hat{\mathcal{S}}(\pi) \vert 
    := 
    \sum_{j=1}^{j=k} \hat{p}^\pi_{j}.
\end{equation}
%
Similarly, the estimated expected path length $\expL$ is defined as:
\begin{equation}\label{eq:estimated expected length}
\hat{\ell}(\pi):=
    \frac{1}{m} \sum_{j=1}^{j=m} \ell (\pi^e_j).
\end{equation}


\subsection{Modifying primitive search operations (challenge \textbf{C2}) \OS{alt sec}}
% Before we explain how we modify in \irisuu primitive operations that were originally used in \iris, we start with several basic definitions.

% \vspace{2mm}
% \begin{dfn}
% Let
% $\rm{IPV}(\pi_1) := \{ \hat{p}_1^{\pi_1}, \ldots, \hat{p}_k^{\pi_1} \}$
% and
% $\rm{IPV}(\pi_2) := \{ \hat{p}_1^{\pi_2}, \ldots, \hat{p}_k^{\pi_2} \}$
% be the  IPVs of paths $\pi_1$ and~$\pi_2$, respectively.
% %
% Then, we say that~$\rm{IPV}(\pi_1)$ \emph{dominates} $\rm{IPV}(\pi_2)$ if:
% $$\forall j \in [1 \ldots k],~\hat{p}_j^{\pi_1} \geq \hat{p}_j^{\pi_2}.$$
% \OS{COMPLETE}
% \end{dfn}

% \vspace{2mm}
% \begin{dfn}
% Let
% $\hat{\ell}(\pi_1)$ and $\hat{\ell}(\pi_2)$
% be the estimated expected path length  of paths $\pi_1$ and~$\pi_2$, respectively.
% Then, we say that $\pi_1$ \emph{dominates} $\pi_2$ with respect to path length if:
% $$\hat{\ell}(\pi_1) \leq \hat{\ell}(\pi_2).$$
% \end{dfn}

% In this section we will explain the primitive operations used in \irisuu's \astar-like search.
% However, before we explain how we modify in \irisuu primitive operations that were originally used in \iris, we start with several basic definitions.

In this section we will explain how we modify the primitive operations used in \irisuu's \astar-like search that were originally used in \iris. 
However, before we explain it, we start with several basic definitions:

\begin{itemize}
    \item \begin{dfn}
    We define a \emph{pruning p-value set}~$\PvalPrun$ (will be used in the pruning operation in Sec.~\ref{subsec:Node pruning}) as:
    \begin{equation}
        \PvalPrun:=\{\pval_1,\pval_2,\ldots\},
    \end{equation}
    such that each element~$\pval_i$ has a value of~$\left[ 0,1\right]$
\end{dfn}
\vspace{2mm}
\item 
\begin{dfn}
Let~$\Pi^e := \{\pi_{1}^e \ldots \pi_{m}^e \}$ be a set of~$m$ execution paths such that~$\pi^e_{i}:=\mathcal{M}(\pi, \Nloc^i, \Ncon^i)$.
    We define a \emph{collision vector}~$\colVec$:
    $$
    \colVec:=\{\colVec_1,\ldots,\colVec_m\},
    $$
    such that each element~$\colVec_j$ indicates whether the path~$\pi^e_j$ is collision-free. Namely: 
      \begin{equation*}
    \colVec_j:=
        \begin{cases}
          0,& \text{if } \pi^e_j \text{ is collision free}\\
        1, & \text{otherwise}
        \end{cases}
    \end{equation*}
    % \colProbHat_i$ has a value of~$\left[ 0,1 \right].
\end{dfn}

\begin{dfn}
Let~$\colVec$ be a collision vector, such that:
  $$
    \colVec:=\{\colVec_1,\ldots,\colVec_m\}.
    $$
    Then, we define a \emph{estimated collision probability}~$\colProbHat$ as :
    $$
    \colProbHat:=\frac{1}{m} \sum_{j=1}^{j=m} \colVec_j
    $$
\end{dfn}


\end{itemize}





%  Let~$n$ be a node:
%     $$
%     n = 
%         \langle
%             u, \pi_u, \Pi^e_u, \hat{\rm{IPV}}_u, \hat{\ell}_u,
%             \tilde{\rm{IPV}}_u,\tilde{\ell}_u,\Pval_u
%         \rangle.
%     $$
%     where
%     $\Pi^e_u := \{\pi_{1,u}^e \ldots \pi_{m,u}^e \}$ is a set of execution paths such that $\pi^e_{i,u}:=\mathcal{M}(\pi_u, \Nloc^i, \Ncon^i)$. 
    
% \begin{dfn}
%     We define~$\colProbHat$ as a collision free array with size~$m$ (size of the Monte Carlo sample) in which each element~$j=1,2,\ldots,m$ indicate if the path~$\pi^e_j$ is collision free, such that:
%     \begin{equation*}
%     \colProbHat_j:=
%         \begin{cases}
%           0,& \text{if } \pi^e_j \text{ is collision free}\\
%     1,              & \text{otherwise}
%         \end{cases}
%     \end{equation*}
% \end{dfn}

% Then, the extending operation finish with calculate the collision free array which used to define the collision probability denote as~$p^{\text{col}}$ with:
% \begin{equation}
%     p^{\text{col}}:=\frac{1}{m}\sum_{i=1}^{i=m} \colProbHat.
% \end{equation}



\vspace{2mm}
\subsubsection{Node definition}
\label{subsec:Node definition}
A node $n$ in our search algorithm is a tuple of:
$$
n = 
\langle
    u, \pi_u, \Pi^e_u, \hat{\rm{IPV}}_u, \hat{\ell}_u,
    \tilde{\rm{IPV}}_u,\tilde{\ell}_u,\Pval_u,\colProbHat_u
\rangle.
$$
Such that,
$u$ is a roadmap vertex,
$\pi_u$ is a path from the start vertex to $u$,
$\Pi_u^e = \{ \pi_{1,u}^e, \ldots, \pi_{m,u}^e\}$ are $m$ simulated execution paths calculated using Eq.~\ref{eq:motion_model_paths},
$\hat{\rm{IPV}}_u = \{ \hat{p}_1^{\pi_u}, \ldots, \hat{p}_k^{\pi_u} \}$ is the estimated IPV,
$\hat{\ell}_u$ is the estimated path length.
In addition,~$\tilde{\rm{IPV}}_v$ and~$\tilde{\ell}_v$ are the estimated IPV and path length of the \pap that will be used in the subsuming operation (see Sec.\ref{subsec:Node subsuming}).
%
Finally,~$\Pval_u$ is the pruning p-value set of node~$n$, and~$\colProbHat_u$ is the collision probability of node~$n$.

The search algorithm begins with \emph{initial node}~$n^\text{init}$ and ends with a \emph{goal node}~$n^\text{goal}$ that are defined as follow:

\begin{itemize}
    \item \begin{dfn}
    We define the initial node~$n^\text{init}$ as a tuple of:
    $$
\langle
    u, \pi_u, \Pi^e_u, \hat{\rm{IPV}}_u, \hat{\ell}_u,
    \tilde{\rm{IPV}}_u,\tilde{\ell}_u,\Pval_u,\colProbHat_u
\rangle,$$
such that $u$ is the initial roadmap vertex,
$\pi_u$ is a only the initial vertex $u$,
$\Pi_u^e = \{ \pi_{1,u}^e, \ldots, \pi_{m,u}^e\}$ are $m$ initial possible configuration \DA{I need to define it properly}, and 
$\hat{\rm{IPV}}_u = \{ \hat{p}_1^{\pi_u}, \ldots, \hat{p}_k^{\pi_u} \}$ is the estimated IPV.
In addition, 
$\hat{\ell}_u$,~$\tilde{\rm{IPV}}_v$ and~$\tilde{\ell}_v$ are zero, and~$\Pval_u$ is an empty pruning p-value set.
\end{dfn}
\vspace{2mm}
   \item \begin{dfn}
   Let~$n$ be a node
    $$
    n=
\langle
    u, \pi_u, \Pi^e_u, \hat{\rm{IPV}}_u, \hat{\ell}_u,
    \tilde{\rm{IPV}}_u,\tilde{\ell}_u,\Pval_u,\colProbHat_u
\rangle,$$
such that~$\hat{\rm{IPV}}(\pi_u) := \{ \hat{p}_1^{\pi_u}, \ldots, \hat{p}_k^{\pi_u} \}$
and
$\tilde{\rm{IPV}}(\pi_u) := \{ \tilde{p}_1^{\pi_u}, \ldots, \tilde{p}_k^{\pi_u} \}$.
Then, we say that~$n$ is~$n^\text{goal}$ if:
$$
\sum_{j=1}^{i=k}  \hat{p}_j^{\pi_u} \geq \kappa  \cdot \sum_{j=1}^{i=k} \tilde{p}_j^{\pi_u}.
$$
\end{dfn}
\end{itemize}

\vspace{2mm}
\subsubsection{Node extension}
\label{subsec:Node extension}
Let $u,v \in \mathcal{V}$ be two rodamap vertices such that $(u,v) \in \mathcal{E}$.
and let $n_u= 
\langle
    u, \pi_u, \Pi^e_u, \hat{\rm{IPV}}_u, \hat{\ell}_u, \tilde{\rm{IPV}}_u,\tilde{\ell}_u,\Pval_u,\colProbHat_u
\rangle$ be a node in the search algorithm to $u$.
We define the operation of \emph{extending}~$n_u$ by the edge $(u,v)$ as creating a new node 
$n_v= 
\langle
    v, \pi_v, \Pi^e_v, \hat{\rm{IPV}}_v, \hat{\ell}_v, \tilde{\rm{IPV}}_v,\tilde{\ell}_v,\Pval_v,\colProbHat_v
\rangle$
such that:
%
\begin{itemize}
    \item $\pi_v$ is the result of concatenating $\pi_v$ with the path $\pi_{u\rightarrow v}$ from~$u$ to $v$.
    Namely, 
    $$\pi_v:= \pi_u \circ \pi_{u\rightarrow v}.$$
    
    \item $\Pi^e_v := \{\pi_{1,v}^e \ldots \pi_{m,v}^e \}$ is set of execution paths such that $\pi^e_{i,v}:=\mathcal{M}(\pi_v, \Nloc^i, \Ncon^i)$. Notice that this can be efficiently computed by denoting:
    $$\pi^e_{j,u\rightarrow v}:=\mathcal{M}(\pi_{u\rightarrow v}, \Nloc^i, \Ncon^i),$$
    and setting:
    $$\pi^e_{j,v}:= \pi^e_{j,u} \circ \pi^e_{j,u\rightarrow v}.$$
    
    \item 
    % $\colProbHat_v$ is collision probability such that:
    %  \begin{equation*}
    % \colProbHat_{v,i}:=
    %     \begin{cases}
    %       0,& \text{if } \pi^e_{i,v} \text{ is collision free},\\
    % 1,              & \text{otherwise}.
    %     \end{cases}
    % \end{equation*}
    % Notice that this also can be efficiently computed by setting:
    

    $\colProbHat_v$ is the collision probability of node~$v$, such that:
    $$
    \colProbHat_v:=1-\left(1-\colProbHat_u \right) \cdot \left(1-\frac{1}{m} \sum_{j=1}^{j=m} \colVec_j \right).
    $$
    Where:
    \begin{equation*}
    \colVec_j:=
        \begin{cases}
          0,& \text{if } \pi^e_{j,u\rightarrow v} \text{ is collision free},\\
          1,  & \text{otherwise}.
        \end{cases}
    \end{equation*}
    
    \item $\hat{\rm{IPV}}_v: = \{ \hat{p}_1^\pi_v, \ldots, \hat{p}_k^\pi_v \}$ is obtained by assuming that (i)~POI inspection is done at vertices and that (ii)~each such action is independently. Consequentially,
    $$
    \forall i\in [1,m]~\hat{p}_j^{\pi_v} := 
     1-(1-\hat{p}^{\pi_{u \rightarrow v}}_{i}) \cdot (1-\hat{p}_i^{\pi_{u}}).
    $$
    \DA{We need to consider: If each~$\hat{p}_j^{\pi_v}$ is close enough (with some $\epsilon$?) to 1 then we consider it as 1.}
    \item $\hat{\ell}_v$ is the estimated path length of $\pi_v$. Notice that this can be efficiently computed by setting
    $$
        \hat{\ell}_v: = \hat{\ell}_u + \hat{\ell}(\pi_{u\rightarrow v}).
    $$
    
    \item The estimated IPV and the path length of the \pap's both with the p-value array. remain unchanged.
    Namely,
    $$
    \tilde{\rm{IPV}}_v := \tilde{\rm{IPV}}_u,
    \quad
    \tilde{\ell}_v := \tilde{\ell}_u,
    \quad
    \Pval_v := \Pval_u.
    $$
\end{itemize}

\vspace{2mm}
\subsubsection{Node dominating}
\label{subsec:Node dominating}
Before we explain the dominating operation, we start with the following definitions.

\vspace{2mm}
\begin{dfn}
Let
$\hat{\rm{IPV}}(\pi_1) := \{ \hat{p}_1^{\pi_1}, \ldots, \hat{p}_k^{\pi_1} \}$
and
$\hat{\rm{IPV}}(\pi_2) := \{ \hat{p}_1^{\pi_2}, \ldots, \hat{p}_k^{\pi_2} \}$
be the  IPVs of paths $\pi_1$ and~$\pi_2$, respectively.
%
Then, we say that~$\hat{\rm{IPV}}(\pi_1)$ \emph{dominates} $\hat{\rm{IPV}}(\pi_2)$ with respect to the coverage (denoted $\hat{\rm{IPV}}(\pi_1) \wedge \hat{\rm{IPV}}(\pi_2)$) if:
$$\forall j \in [1 \ldots k],~\hat{p}_j^{\pi_1} \geq \hat{p}_j^{\pi_2}.$$
\OS{COMPLETE}
\end{dfn}

\vspace{2mm}
\begin{dfn}
Let
$\hat{\ell}(\pi_1)$ and $\hat{\ell}(\pi_2)$
be the estimated expected path length  of paths $\pi_1$ and~$\pi_2$, respectively.
Then, we say that $\pi_1$ \emph{dominates} $\pi_2$ with respect to path length (denoted $\pi_1 \wedge \pi_2$) if:
$$\hat{\ell}(\pi_1) \leq \hat{\ell}(\pi_2).$$
\end{dfn}


We now ready to define the dominating operation.
Let
$n_1$ and~$n_2$ be two nodes both starting at the same vertex and ending at the same vertex~$u$.
Specifically assume that 
$
n_i= 
\langle
    u, \pi_{u,i}, \Pi^e_{u,i}, \hat{\rm{IPV}}_{u,i}, \hat{\ell}_{u,i}, \tilde{\rm{IPV}}_{u,i},\tilde{\ell}_{u,i},\Pval_{u,i},\colProbHat_{u,i}
\rangle$ for $i \in \{1,2\}$.
Then, node~$n_1$ dominates~$n_2$ (denoted $n_1 \wedge n_2$) if~(i)~$\hat{\rm{IPV}}_{u,1}$ dominates~$\hat{\rm{IPV}}_{u,2}$ and (ii)~$\pi_{u,1}$ dominates~$\pi_{u,2}$.


\vspace{2mm}
\subsubsection{Node subsuming}
\label{subsec:Node subsuming}
Before we explain the subsuming operation, we start with the following definition.

\begin{itemize}
    \item 
\begin{dfn}\label{def:ek_bounded}
    Let~$n$ be a node:
    $$
    n = 
        \langle
            u, \pi_u, \Pi^e_u, \hat{\rm{IPV}}_u, \hat{\ell}_u,
            \tilde{\rm{IPV}}_u,\tilde{\ell}_u,\Pval_u,\colProbHat_u
        \rangle.
    $$
    In addition, let
$\hat{\rm{IPV}}(\pi_{u}) := \{ \hat{p}_1^{\pi_{u}}, \ldots, \hat{p}_k^{\pi_{u}} \}$
and
$\tilde{\rm{IPV}}(\pi_{u}) := \{ \tilde{p}_1^{\pi_{u}}, \ldots, \tilde{p}_k^{\pi_{u}} \}$
be the achievable and potential achievable IPVs of paths $\pi_{u}$, respectively.
Similarly, let~$\hat{\ell}_u$ and~$\tilde{\ell}_u$ be the achievable and potential achievable path length of~$\pi_{u}$, respectively.
    We say that~$n$ is \ek-bounded if:
    % \frac{1}{m}\sum_{j=1}^{i=k} 
    \begin{equation*}
        \begin{split}
            \sum_{j=1}^{i=k}  \hat{p}_j^{\pi_u} \geq \kappa  \cdot \sum_{j=1}^{i=k} \max \left( \tilde{p}_j^{\pi_u},\hat{p}_j^{\pi_u} \right), \\
            \hat{\ell}_u \leq (1+\epsilon) \cdot \tilde{\ell}_u.
        \end{split}
    \end{equation*}
\end{dfn}
\end{itemize}
\vspace{2mm}
Now we ready to define the subsuming operation.
% The purpose of the subsuming operation is to maintain the \pap properties in order to bound the optimal solution. This operation is defined as follow:
Let
$n_1$ and~$n_2$ be two nodes both starting at the same vertex and ending at the same vertex~$u$.
Specifically assume that 
$
n_i= 
\langle
    u, \pi_{u,i}, \Pi^e_{u,i}, \hat{\rm{IPV}}_{u,i}, \hat{\ell}_{u,i}, \tilde{\rm{IPV}}_{u,i},\tilde{\ell}_{u,i},\Pval_{u,i},\colProbHat_{u,i}
\rangle$ for $i \in \{1,2\}$.

The operation of $n_1$ subsuming $n_2$ 
(denoted $n_1 \oplus n_2$) 
will create a new node:~
$$
 n_3 = 
        \langle
            u, \pi_{u,3}, \Pi^e_{u,3}, \hat{\rm{IPV}}_{u,3}, \hat{\ell}_{u,3},
            \tilde{\rm{IPV}}_{u,3},\tilde{\ell}_{u,3},\Pval_{u,3},\colProbHat_{u,3}
        \rangle,
$$
such that the following properties get the value of node~$n_1$:
\begin{equation*}
    \begin{split}
        \pi_{u,3} = \pi_{u,1},
        \Pi^e_{u,3} = \Pi^e_{u,1},\\
        \hat{\rm{IPV}}_{u,3} = \hat{\rm{IPV}}_{u,1}, \hat{\ell}_{u,3} = \hat{\ell}_{u,1},\\
        \Pval_{u,3} = \Pval_{u,1},
        \colProbHat_{u,3} = \colProbHat_{u,1}.
    \end{split}
\end{equation*}

In contrast, the \pap properties get new values, such that:
\begin{equation*}
    \tilde{\ell}_{u,3}:= \min{(\tilde{\ell}_{u,1},\tilden {\ell}_2)},
\end{equation*}
and, each element~$j$ of~$\tilde{\rm{IPV}}_{u,3}$ is defined as:
\begin{equation*}
    \tilde{p}_j^{\pi_{u,3}}:= \max{(\tilde{p}_j^{\pi_{u,1}},\tilde{p}_j^{\pi_{u,2}})}.
\end{equation*}

Yet, the subsuming operation has not been completed. That is, the resultant node has to maintain the optimal inspection path relative to the parameters~$\kappa$ and~$\epsilon$.
Thus, the subsuming only occurs if the resultant node~$n_{u,3}:=n_1 \oplus n_2$ is \ek-bounded (Def.~\ref{def:ek_bounded}).
% Then, if~$n_3$ is \ek-bounded we assign~$n_1= n_3$.
 
% \DA{Do we need to add Lemma?}
% Notice that, the purpose of the \pap properties is only to represent the bounded achievable values. Thus, there is no need to update the p-values for those comparisons.  

\vspace{2mm}
\subsubsection{Node pruning}
\label{subsec:Node pruning}
% In our algorithm the node pruning occurs in two cases:
% \begin{itemize}
%     \item If node~$n_1$ dominates~$n_2$ (see Sec.~\ref{subsec:Node dominating}), then node~$n_2$ is pruned.
%     \item If the resultant subsuming node~$n_3:=n_1 \oplus n_2$ is \ek-bounded (see Sec.~\ref{subsec:Node pruning}), then node~$n_2$ is pruned and we assign~$n_1=n_3$. 
% \end{itemize}
In our algorithm, if node~$n_1$ dominates~$n_2$ (see Sec.~\ref{subsec:Node dominating}), then node~$n_2$ is pruned.
However, if node~$n_2$ is decided to be pruned we need to update the pruning p-value set~$\Pval_{u,1}$ to reflect the p-value of this operation.
To do so, we will start with defining the following definitions:

% To do so, recall that we addressing the p-value as the statistic result of comparing two population's samples or two proportion's samples (see Sec.~\ref{subsec:Null Hypothesis Testing}).

% However, the comparisons are different in each operation (dominating or subsuming) so, we will define each of them separately:

% % \begin{itemize}
% %     \item 
% For the dominating operation we will start with defining the following definitions:

\vspace{2mm}
\begin{dfn}
Let~$n_1$ and~$n_2$ be the two nodes of the dominating operation. In addition, let
$\hat{\rm{IPV}}(\pi_{u,1}) := \{ \hat{p}_1^{\pi_{u,1}}, \ldots, \hat{p}_k^{\pi_{u,1}} \}$
and
$\hat{\rm{IPV}}(\pi_{u,2}) := \{ \hat{p}_1^{\pi_{u,2}}, \ldots, \hat{p}_k^{\pi_{u,2}} \}$
be the IPVs of paths $\pi_{u,1}$ and~$\pi_{u,2}$ related to~$n_1$ and ~$n_2$, respectively.
We define~$\Pval^\text{IPV}$ as the \emph{IPV p-value vector}:
$$ 
\Pval^\text{IPV}:= \{\pval^\text{IPV}_1,\ldots,\pval^\text{IPV}_k \},
$$
such that, each element~$\pval^\text{IPV}_j$, is defined by the t-test result of:
$$\pval^\text{IPV}_j:=\pval(\hat{p}_j^{\pi_{u,1}} \geq \hat{p}_j^{\pi_{u,2}}).$$
\end{dfn}

\vspace{2mm}
\begin{dfn}
Let~$n_1$ and~$n_2$ be the two nodes of the dominating operation. In addition,
let
$\hat{\ell}(\pi_{u,1})$ and $\hat{\ell}(\pi_{u,2})$
be the estimated expected path length  of paths $\pi_{u,1}$ and~$\pi_{u,2}$, respectively.
 we define~$\pval^\ell$ as the \emph{length p-value} such that:
$$\pval^\ell:=\pval(\hat{\ell}(\pi_{u,1}) \leq \hat{\ell}(\pi_{u,2})).
$$
\end{dfn}

Now, we ready to define the \emph{dominating p-value vector}:

\vspace{2mm}
\begin{dfn}
Let~$\Pval^\text{IPV}$ and~$\pval^\ell$ be the IPV p-value vector and the length p-value of the dominating operation, respectively.
Then we define~$\Pval_\text{dom}$ as the dominating p-value vector, such that:
    $$
    \Pval_\text{dom}:=\{\pval^\text{IPV}_1,\ldots,\pval^\text{IPV}_k,\pval^\ell\},
    $$
\end{dfn}

Then, following the BH method (see Sec~\ref{subsec:False discovery rate}) we define the \emph{BH dominating p-value} as follow: 

\vspace{2mm}
\begin{dfn}
    Let~$\Pval_\text{dom}$ be a dominating p-value vector.
    In addition, let~$\pval_{\text{dom}_1},\ldots,\pval_{\text{dom}_{k+1}}$ be the element of~$\Pval_\text{dom}$ listing in ascending order. 
    We say that the BH dominating p-value~$\pval_\text{dom}^\text{BH}$ is the equivalent  p-value for the dominating operation and calculate it as:
    \begin{equation}\label{eq:pval_BH}
        \pval_\text{dom}^\text{BH}:=\min_{i} \frac{\pval_{\text{dom}_i} \cdot i}{k+1}
    \end{equation}
\end{dfn}

\vspace{2mm}
Finally, at the end of the node pruning after the dominating operation we update the set~$\Pval_{u,1}$ by concatenating~$\pval_\text{dom}^\text{BH}$ with~$\Pval_{u,1}$, such that: 
$$
\Pval_{u,1}=  \Pval_{u,1} \sqcup \pval_\text{dom}^\text{BH}.
$$

Now we can formally define the \emph{dominate-prune} operation:
\begin{dfn}
Let
Let~$n_1$ and~$n_2$ be the two nodes of the dominating operation, such that~$n_1 \wedge~n_2$. 
Then, the operation~$n_1$ dominate-prune~$n_2$ (denoted as $n_1 \wedge \otimes~n_2$) will result with a node~$n_1$ such that~$\Pval_{u,1}$ will be updated to: 
$$
\Pval_{u,1}=  \Pval_{u,1} \sqcup \pval_\text{dom}^\text{BH}.
$$
\end{dfn}

% \item For the subsuming operation we will start with defining the following definitions:

% \vspace{2mm}
% \begin{dfn}
%     Let~$n_3$ be the resultant node of the subsuming operation~$n_1 \oplus n_2$. In addition, let
% $\hat{\rm{IPV}}(\pi_{u,3}) := \{ \hat{p}_1^{\pi_{u,3}}, \ldots, \hat{p}_k^{\pi_{u,3}} \}$
% and
% $\tilde{\rm{IPV}}(\pi_{u,3}) := \{ \tilde{p}_1^{\pi_{u,3}}, \ldots, \tilde{p}_k^{\pi_{u,3}} \}$
% be the achievable and potential achievable IPVs of paths $\pi_{u,3}$, respectively.
% We define~$\pval^{\text{IPV}_\kappa}$ as the \emph{IPV,$\kappa$ p-value} as the t-test result of:
% $$\pval^{\text{IPV}_\kappa}:=\pval \left( \sum_{j=1}^{i=k}  \hat{p}_j^{\pi_u} \geq \kappa  \cdot \sum_{j=1}^{i=k} \max \left( \tilde{p}_j^{\pi_u},\hat{p}_j^{\pi_u} \right) \right).$$
% \end{dfn}

% \vspace{2mm}
% \begin{dfn}
%   Let~$n_3$ be the resultant node of the subsuming operation~$n_1 \oplus n_2$. In addition, let~$\hat{\ell}(\pi_{u,3})$ and $\tilde{\ell}(\pi_{u,3})$
% be the estimated expected path length of the achievable and potential achievable paths, respectively.
%  we define~$\pval^{\ell_\epsilon}$ as the \emph{length,~$\epsilon$ p-value} such that:
% $$\pval^{\ell_\epsilon}:=\pval \left( \hat{\ell}(\pi_{u,3}) \leq \left( 1+\epsilon \right)\tilde{\ell}(\pi_{u,3}) \right).
% $$
% \end{dfn}

% Now, we ready to define the \emph{subsuming p-value vector}:

% \vspace{2mm}
% \begin{dfn}
% Let~$\pval^{\text{IPV}_\kappa}$ and~$\pval^{\ell_\epsilon}$ be the IPV,$\kappa$ and length,~$\epsilon$ p-value of the subsuming operation, respectively.
% Then we define~$\Pval_\text{sub}$ as the subsuming p-value vector, such that:
%     $$
%     \Pval_\text{sub}:=\{\pval^{\text{IPV}_\kappa},\pval^{\ell_\epsilon}\},
%     $$
% \end{dfn}

% \vspace{2mm}
% Then, following the BH method (see Sec~\ref{subsec:False discovery rate}) we define the \emph{BH subsuming p-value} as follow: 

% \vspace{2mm}
% \begin{dfn}
%     Let~$\Pval_\text{sub}$ be a subsuming p-value vector.
%     In addition, let~$\pval_{\text{sub}_1},\pval_{\text{sub}_{2}}$ be the element of~$\Pval_\text{sub}$ listing in ascending order. 
%     We say that the BH dominating p-value~$\pval_\text{dom}^\text{BH}$ is the equivalent p-value for the subsuming operation and calculate it as:
%     \begin{equation}\label{eq:pval_BH}
%         \pval_\text{sub}^\text{BH}:=\min_{i} \frac{\pval_{\text{sub}_i} \cdot i}{2}
%     \end{equation}
% \end{dfn}

% \vspace{2mm}
% Finally, at the end of the node pruning after the subsuming operation we update the set~$\Pval_{u,1}$ by concatenating~$\pval_\text{sub}^\text{BH}$ with~$\Pval_{u,1}$, such that: 
% $$
% \Pval_{u,1}=  \Pval_{u,1} \sqcup \pval_\text{sub}^\text{BH}.
% $$

% Now we can formally define the \emph{subsume-prune} operation:
% \begin{dfn}
% Let~$n_1$ and~$n_2$ be the two nodes of the subsuming operation, such that~$n_1 \oplus n_2$ is~$\epsilon,\kappa-\text{bounded}$. 
% Then, the operation~$n_1$ subsume-prune~$n_2$ (denoted as $n_1 \oplus \otimes~n_2$) will result with a node~$n_1 \oplus n_2$ with updated value of~$\Pval_{u,1}$ such that:
% $$
% \Pval_{u,1}=  \Pval_{u,1} \sqcup \pval_\text{sub}^\text{BH}.
% $$
% \end{dfn}

% \end{itemize}


\OS{Do we do pruning using our approximation factors?}

\OS{When we prune a node, what do we do with its \pap?}

\OS{Fill in similar to the prev secs}


\vspace{2mm}
\subsection{\irisuu algorithm flow}
\label{subsec:Algorithm flow}
In this section we describe the \irisuu algorithm flow with pseudo-code (Alg.~\ref{alg:irisuuAlgo}). Our algorithm is based and similar to \iris and uses also two priority queues OPEN and CLOSED to consider node changes during the search.
During the algorithm we denote~$n^\text{texted},n^\text{OPEN}$ and~$n^\text{CLOSED}$ as the extended node, and the node form the OPEN and CLOSED list, respectively.

\irisuu starts with an empty CLOSED list and with an OPEN list with ~$n^\text{init}$.
Then, the search is proceeding by pop from the OPEN list the node with max coverage. If it meet the requirements of~$n^\text{goal}$ we terminate the search and return the last popped node (line 4-7) 
If not, we extend~$n^\text{extend}$ of all neighboring edges~$e$ of $u$ in $\G$ (line 9).

Then, if there exists a node~$n^\text{CLOSED}$ in CLOSED list that dominates~$n^\text{extend}$ (lines 11-14), Then,~$n^\text{extend}$ is discarded and~$n^\text{CLOSED}$ is updated by dominate-prune ($\wedge \otimes$) with~$n^\text{extend}$ (line 15-17).

If there is not such a node in the CLOSED list we start to compare~$n^\text{extend}$ to the nodes in the OPEN list.
If there is~$n^\text{OPEN}$ such that~$n^\text{OPEN} \oplus n^\text{extend}$ is $\epsilon,\kappa-\text{bounded}$ (line 19), then~$n^\text{extend}$ is discarded and~$n^\text{OPEN}$ is updated by subsuming it with~$n^\text{extend}$ (line 20).

If not, we check if there is~$n^\text{OPEN}$ such that~$n^\text{extend} \oplus n^\text{OPEN}$ is $\epsilon,\kappa-\text{bounded}$ (line 26). If so,~$n^\text{OPEN}$ is discarded and removed from the OPEN list (line 27) and~$n^\text{extend}$ is updated by subsuming it with ~$n^\text{OPEN}$ (line 28).

Finally, If~$n^\text{extend}$ pass all these tests, then~$n^\text{extend}$ is inserted to the OPEN list for the next while loop (line 29). Notice that, if the while loop reaches a condition of an empty OPEN list, then it means that \irisuu results with no solution and return NULL (line 30).


\vspace{2mm}
\begin{algorithm}
    \caption{\irisuu algorithm pseudo-code}\label{alg:irisuuAlgo}
    \hspace*{\algorithmicindent} \textbf{Input: } $\left( \G,n^\text{start},\epsilon,\kappa \right)$ \\
    \hspace*{\algorithmicindent} \textbf{Output: } $n$
    \begin{algorithmic}[1]
%    \Procedure{MyProcedure}{$x,y$}
%     % Input:
%     \Comment{Input: x}
%     % Output:
%     \Comment{Output:y}
\State CLOSED \gets~$\emptyset$
\State OPEN \gets $n^\text{init}$  
\While {OPEN \ne~$\emptyset$} 
    \State $n \gets$ OPEN.extract\_node\_with\_max\_coverage()
    \State CLOSED.insert($n$)
\If {$n \text{ is } n^\text{goal}$}
\State \Return $n$
\EndIf
\item[]
\For{$e=(u,v) \in \text{neighbors}(u,\G)$}
{\State $n^\text{extend} \gets$ extend($n,u$)
\State valid = \textbf{True}
\For{$n^\text{CLOSED} \in$ CLOSED}
{\If{$n^\text{CLOSED} \wedge~n^\text{extend}$}
\State valid = \textbf{False}
\State \textbf{break}
\EndIf
}
\EndFor
}
\item[]
\If{!valid}
\State $n^\text{CLOSED} \gets n^\text{CLOSED}$ \wedge \otimes $ n^\text{extend}$
% \State $n^\text{CLOSED} \gets n^\text{CLOSED}$ dominate-prune $n^\text{extend}$
\State \textbf{continue}
\EndIf
\item[]
\For{$n^\text{OPEN} \in$ OPEN}
{\If{$n^\text{OPEN} \oplus n^\text{extend}$ is $\epsilon,\kappa-\text{bounded}$}
\State $n^\text{OPEN} \gets n^\text{OPEN} \oplus n^\text{extend}$
\State valid = \textbf{False}
\State \textbf{break}
\EndIf
}
\EndFor
\item[]
\If{!valid} 
% \State $n^\text{OPEN}\gets n^\text{OPEN}$ \oplus \otimes $ n^\text{extend}$
% \State $n^\text{OPEN}\gets n^\text{OPEN}$ subsume-prune $n^\text{extend}$
\State \textbf{continue}
\EndIf
\item[]
\For{$n^\text{OPEN} \in$ OPEN}
{
\If{$n^\text{extend} \oplus n^\text{OPEN}$ is $\epsilon,\kappa-\text{bounded}$}
\State OPEN.remove($n^\text{OPEN}$)
\State $n^\text{extend} \gets n^\text{extend} \oplus n^\text{OPEN}$
% \State $n^\text{extend} \gets n^\text{extend}$ \oplus \otimes $ n^\text{OPEN}$
% \State $n^\text{extend} \gets n^\text{extend}$ subsume-prune $n^\text{OPEN}$
\EndIf
}
\EndFor
\EndFor
\item[]
\State OPEN~$\gets n^\text{extend}$
\EndWhile


\State \Return NULL
    \end{algorithmic}
    \end{algorithm}

\subsection{Theoretical guarantees \OS{alt sec}}
\footnote{
\OS{Define the simplifying assumption of ``Different Past, Same Future'' (DPSF)}}
Let the result of \irisuu algorithm be a goal node:
$$
n^\text{goal} = 
\langle
    u, \pi_u, \Pi^e_u, \hat{\rm{IPV}}_u, \hat{\ell}_u,
    \tilde{\rm{IPV}}_u,\tilde{\ell}_u,\Pval_u,\colProbHat_u
\rangle,
$$

\begin{lemma}[Bounding executed path's expected length]
Let $\pi$ be the path obtained by executing the command path~$\pi_{u}$ and recall that 
its length is a  random variable.
For any desired CL of $1 - \alpha$, with $\alpha \in [0,1]$, 
we can bound  the expected path length $\bar{\ell}(\pi)$. 
%
Specifically, with CL of~$1 - \alpha$ we have that
\begin{equation}
    \bar{\ell}(\pi) \in \left[ \hat{\ell}(\pi_u) - \delta_\ell^-,\hat{\ell}(\pi_u) + \delta_\ell^+ \right].
\end{equation}
Here, we define 
$\delta_\ell^- := \min\{\delta_{\ell} (\pi_u,CL), \hat{\ell}(\pi_u)\}$,
and
$\delta_\ell^+ := \delta_{\ell} (\pi_u,CL)$,
where
\begin{equation}\label{eq:delta_ell}
\delta_\ell(\pi_u,CL):= 
    Z^*(CL) 
        \cdot 
    \frac{
         \sqrt{\sum_{j=1}^m{\left(\ell(\pi^e_j) - \hat{\ell}(\pi_u) \right)^2 }}
        }
        {m}.
\end{equation}
\end{lemma}

\vspace{2mm}
\begin{proof}
Let~$\Pi^e_u$ be~$m$ Monte Carlo execution sample paths of~$n^\text{goal}$, and let~$\hat{\ell}(\pi_u)$ be its average path length.
Then, according to CL and CI theory, the predicted CI of the executed path length of  path~$\pi$ is depended with CL and expressed by~$\delta_\ell(\pi_u,CL)$ Eq.~\ref{eq:delta_ell} (implementation of Eq.~\ref{eq:CI_calculation_value}).
However, we know that~$\hat{\ell}(\pi_u)$ must be greater than zero. Thus, we defined~$\delta_\ell^-$ as~$\min\{\delta_{\ell} (\pi_u,CL), \hat{\ell}(\pi_u)\}$ such that~$\hat{\ell}(\pi_u) - \delta_\ell^- \geq 0$. 
\end{proof}

\begin{lemma}[Bounding executed path's expected coverage]
Let $\pi$ be the path obtained by executing the command path~$\pi_{u}$ and recall that 
its coverage is a  random variable.
For any desired CL of $1 - \alpha$, with $\alpha \in [0,1]$, 
we can bound the expected path coverage $\vert \bar{\S}(\pi) \vert$. 
%
Specifically, with CL of~$1 - \alpha$ we have that:
\begin{equation}
    \bar{\S}(\pi) \in 
    \left[ 
        \sum_{j=0}^{j=k} \left( \hat{p}^{\pi_u}_j - \delta_{\mathcal{S},j}^- \right), \sum_{j=0}^{j=k} \left( \hat{p}^{\pi_u}_j + \delta_{\mathcal{S},j}^+ \right)
    \right].
\end{equation}
Here, we define 
$\delta_\mathcal{S}_j^- := \min\{  \delta_{\S,j}(\pi_u, CL)  , \hat{p}^{\pi_u}_j\}$,
and
$\delta_\mathcal{S}_j^+ := \min\{  \delta_{\S,j}(\pi_u, CL)  , 1 - \hat{p}^{\pi_u}_j\}$
where:
\begin{equation}\label{eq:delta_S}
\delta_{\mathcal{S},j}(\pi_u, CL):= 
    Z^*(CL) 
        \cdot 
    \sqrt\frac{
          \hat{p}^{\pi_u}_j \cdot (1- \hat{p}^{\pi_u}_j)
        }
        {{m}}.
\end{equation}
\end{lemma}

\vspace{2mm}
\begin{proof}
Let~$\Pi^e_u$ be~$m$ Monte Carlo execution sample paths of~$n^\text{goal}$, and let~$\hat{\rm{IPV}}(\pi_{u}) := \{ \hat{p}_1^{\pi_{u}}, \ldots, \hat{p}_k^{\pi_{u}} \}$ be its IPV.
Then, according to CL and CI theory, the predicted CI of the executed each element of the IPV of path~$\pi$ is depended with CL and expressed by~$\delta_{\mathcal{S},j}(\pi_u, CL)$ Eq.~\ref{eq:delta_S} (implementation of Eq.~\ref{eq:CI_calculation_proportions}).
However, we know that~$\hat{p}^{\pi_u}_j$ must be in range of~$\left[0,1\right]$. Thus, we defined~$\delta_\mathcal{S}_j^-$ as~$\min\{  \delta_{\S,j}(\pi_u, CL)  , \hat{p}^{\pi_u}_j\}$ such that~$\hat{p}^{\pi_u}_j - \delta_{\mathcal{S},j}^- \geq 0$. Similarly, we defined~$\delta_\mathcal{S}_j^+$ as~$\min\{  \delta_{\S,j}(\pi_u, CL)  , 1 - \hat{p}^{\pi_u}_j\}$ such that~$\hat{p}^{\pi_u}_j + \delta_{\mathcal{S},j}^+ \leq 1$.
\end{proof}

\begin{lemma}[Bounding executed path's collision]
Let $\pi$ be the path obtained by executing the command path~$\pi_{u}$ and recall that whether the path is collision-free or not is a random variable. 
For any desired CL of $1 - \alpha$, with $\alpha \in [0,1]$, 
we can bound the expected path's collision probability $\colProbBar_u$. 
%
Specifically, with CL of~$1 - \alpha$ we have that:
\begin{equation}
    \colProbBar_u \in 
    \left[ 
        \left( {\colProbHat_u} - \delta_{\colProbHat}^- \right),  \left( {\colProbHat_u} + \delta_{\colProbHat}^+ \right)
    \right].
\end{equation}
Here, we define 
$\delta_{\colProbHat}^- := \min\{  \delta_{\colProbHat_u}(CL)  , \colProbHat_u\}$,
and
$\delta_\mathcal{S}_j^+ := \min\{  \delta_{\colProbHat_u}(CL)  , 1 - \colProbHat_u\}$
where:
\begin{equation}\label{eq:delta_Col}
\delta_{\colProbHat_u}(CL):= 
    Z^*(CL) 
        \cdot 
    \sqrt\frac{
          \colProbHat_u \cdot (1- \colProbHat_u)
        }
        {{m}}.
\end{equation}
\end{lemma}

\vspace{2mm}
\begin{proof}
Let~$\colProbHat_u$ be the estimated collision probability of~$m$ Monte Carlo sample paths of~$n^\text{goal}$.
Then, according to CL and CI theory, the predicted CI of the executed collision probability of path~$\pi$ is depended with CL and expressed by~$\delta_{\colProbHat_u}(CL)$ Eq.~\ref{eq:delta_Col} (implementation of Eq.~\ref{eq:CI_calculation_proportions}).
However, we know that~$\colProbHat_u$ must be in range of~$\left[0,1\right]$. Thus, we defined~$\delta_{\colProbHat}^-$ as~$\min\{  \delta_{\colProbHat_u}(CL)  , \colProbHat_u\}$ such that~${\colProbHat_u} - \delta_{\colProbHat}^- \geq 0$. Similarly, we defined~$\delta_{\colProbHat}^+$ as~$\min\{  \delta_{\colProbHat_u}(CL)  , 1 - \colProbHat_u\}$ such that~${\colProbHat_u} + \delta_{\colProbHat}^+ \leq 1$.
\end{proof}



\begin{lemma}[Bounding executed path's sub-optimality]
Let~$\tilde{\rm{IPV}}_u:= \{ \tilde{p}_1^{\pi_{u}}, \ldots, \tilde{p}_k^{\pi_{u}} \}$ and~$\tilde{\ell}_u$ be the \pap properties of~$n^\text{goal}$, respectively. In addition, let~$\Pval_u$ be the pruning p-value set of~$n^\text{goal}$ and let~$\pval_{u,1},\pval_{u,2},\ldots,\pval_{u,d}$ be its elements listing in ascending order.
Then, we define~$\pval_\text{prun}^\text{BH}$ as:
    \begin{equation}\label{eq:pval_BH}
        \pval_\text{prun}^\text{BH}:=\min_{i} \frac{\pval_{u,i} \cdot i}{d},
    \end{equation} 
and say that we have a probability of~$1-\pval_\text{prun}^\text{BH}$ that there is no other \pap  with a coverage greater than~$\sum_{j=1}^{j=k} \tilde{p}_j^{\pi_{u}}$
and with a path length shorter than~$\tilde{\ell}_u$.
\end{lemma}

\vspace{2mm}
\begin{proof}
During the search, the remaining nodes in the OPEN list subsumed all other nodes reaching the same vertex and are maintaining the \pap properties~$\tilde{\rm{IPV}}_u$ and~$\tilde{\ell}_u$.


The subsuming operation maintained the \pap  with other node in the OPEN set except for nodes that were dominated by the nodes of CLOSED set.
\end{proof}

%  


% Using this calculation, we say with probability of existing path with more coverage than  at most~$\tau_\text{BH}(\Pval_u)$, that there is no other path with smaller expected length that achieves coverage larger or equal to $\kappa \cdot \vert \mathcal{I} \vert $. 



% \subsubsection{Demo illustration problem}
% In this section we illustrate \irisuu method using a demo problem. 
% The problem includes a requirement to inspect 3 POI by selecting command path~$\pi$ along a roadmap~$\mathcal{G}$ with 5 vertices and 5 edges in presence of 3 obstacles (Figure.~\ref{fig:Illustration}).
%  \begin{figure}[ht]
%     \centering
%      \includesvg[inkscapelatex=false, width=0.5\textwidth]{figs/Illustration.svg}
%      \caption{A roadmap~$\mathcal{G}$ with A,B,C,D,E vertices and 5 edges. In addition, the obstacles are marked in brown rectangles and the POI are marked in red circles.}
%      \label{fig:Illustration}
% \end{figure}

% As depicted in Fig.\ref{fig:Illustration_calc} the algorithm was performed using~$3$ MC samples and initiated the first search node from a vertex A as~$n_A := \langle  IPV = \{0.5,0.4,0\},\hat{l} = 0 \rangle$.
% Then, the search is split into two branches~$\{A \rightarrow B, A \rightarrow C\}$.
% In each branch, the value of the IPV and~$\hat{l}$ of the extended node is updated using the value of~$n_A$ and the transition value table.
% For instance, the IPV of~$n_{A \rightarrow B}$ is updated to:
% \begin{equation*}
%     \begin{split}
% IPV = \{1-(1-1)\cdot(1-0.5),\\
%         1-(1-0.67)\cdot(1-0.4),\\
%         1-(1-0)\cdot(1-0)\} = \\
%         =\{1,0.8,0\}.
% \end{split}
% \end{equation*}
% In the same way, the estimated length of~$n_{A \rightarrow B}$ is updated to:
% $$\hat{l} = 0 + 1.5.$$

% Then, following this guideline, the branches extend and reach a vertex D where the two branches meet together. 
% That is, the first branch has values of:
% $$n_{A \rightarrow B \rightarrow D} := \langle  IPV = \{1,0.8,0.67\},\hat{l} = 3.5 \rangle,$$ and the second branch has values of:
% $$n_{A \rightarrow C \rightarrow D} := \langle  IPV = \{0.5,0.4,0.89\},\hat{l} = 3.8 \rangle.$$

%  \begin{figure}[ht]
%     \centering
%      \includesvg[inkscapelatex=false, width=0.5\textwidth]{figs/Illustration_calc.svg}
%      \caption{Extending the search nodes}
%      \label{fig:Illustration_calc}
% \end{figure}

% At this point the algorithm test the node pruning operation. 
% To do so, we use the comparison equations (Eq.~\ref{eq:p-value-populations},~\ref{eq:p-value-proportions}).
% We can see the results in Fig.\ref{fig:Illustration_calc1}.
%  \begin{figure}[ht]
%     \centering
%      \includesvg[inkscapelatex=false, width=0.5\textwidth]{figs/Illustration_calc_1.svg}
%      \caption{Pruning operation result}
%      \label{fig:Illustration_calc1}
% \end{figure}
% The comparison of the path length result with~$t = 2.32$~\ref{eq:p-value-populations}, then assign is into the t-statistic table result with~$\gamma_{\ell} = 0.92$.
% In a similar way, the comparison of the coverage was performed using Eq.\ref{eq:p-value-proportions} and result with~$t_1 = 1.73,t_2=1.09,t_3=-0.67$, where~$i$ index in~$t_i$ is refer to the POI number. Assign these value into the t-statistic result with~$\gamma_{\mathcal{S}_1} = 0.88,\gamma_{\mathcal{S}_1} = 0.80,\gamma_{\mathcal{S}_1} = 0.28$. Thus, the total value of~$\gamma_\mathcal{S}$ is equal to~$0.2$.
% Following this calculation we say that~$n_{A \rightarrow B \rightarrow D}$ stochastically dominates~$n_{A \rightarrow C \rightarrow D}$ with probability of~$\gamma_{\ell} \cdot \gamma_\mathcal{S} = 19[\%]$.

% \DA{Notice that we get only~$19[\%]$ for the pruning operation. This (maybe) highlights the need to set a limit for this action}

% It can be seen that the search is not over yet, and that branch~$n_{A \rightarrow B \rightarrow D}$ still does not provide full coverage for the entire POI. However, even at this stage we can evaluate the quality of the solution using equations~\ref{eq:CI_calculation_value},~\ref{eq:CI_calculation_proportions}.
% That is, suppose we require a CL of~$95[\%]$. Then, because of the small number of samples ($3$) we will have to use~$T^*$, when in this case we get~$T^*=4.3$.
% Calculating the values of~$n_{A \rightarrow B \rightarrow D}$ into these equations produces~$\delta_\ell(\pi) = 0.5$.
% Thus, we have a CL of~$95[\%]$ the path length is in~$[3,4]$.

% Similarly, the confidence interval of each POI is:~$\delta_\mathcal{S}_1 = 0, \delta_\mathcal{S}_2 = 0.99, \delta_\mathcal{S}_3 = 1.167$, where the index~$i$ in~$\delta_\mathcal{S}_i$ is the number of the POI.
% Then, due to the very low number of samples, the values of~$\delta_\mathcal{S}_2$ and~$\delta_\mathcal{S}_3$ are high. 
% In this case, the CI value of each POI is limited to~$[0,1]$.
% That is, as state, we need to calculate each side separately and consider the limited values of~$[0,1]$:
% Thus, the positive side is~$1+\textbf{0},0.8+\textbf{0.2},0.67+\textbf{0.33}$, where the value of~$0,0.2,0.33$ are~$\delta_\mathcal{S}(\pi, j)^+$. In addition, the negative side is~$1-\textbf{0},0.8-\textbf{0.8},0.67-\textbf{0.67}$ where the value~$0,-0.8,-0.67$ are~$\delta_\mathcal{S}(\pi, j)^-$.
% Finally, we can say that we have CL of~$95[\%]$ that the number of the POI inspected is in~$[1,3]$.





% % \subsubsection{Bounding path quality}
% % Given a command path $\pi$ for which we sampled $m$ execution paths $\pi^e_1, \ldots, \pi^e_m$,
% % we can bound the quality of our estimated length and coverage.
% % Specifically, following the approach described in Sec.~\ref{subsec:MC-methods} we have the following results:

% % For any, desired CL between zero and one there is a probability of~$1-\alpha$ (with $\alpha := 1 - \text{CL}$) that the expected path length $\bar{\ell}(\pi)$ 
% % will be in the interval $\hat{\ell}(\pi) \pm \delta_\ell(\pi)$,\footnote{Strictly speaking, $\delta_\ell (\pi)$ should include $\alpha$ as an additional parameter and should be written as $\delta_\ell (\pi, \alpha)$. However, this is omitted for brevity. We do the same for the following derivations.}
% % where 
% % \begin{equation}
% % \delta_\ell(\pi):= 
% %     Z^*(\text{CL}) 
% %         \cdot 
% %     \frac{
% %          \sqrt{\sum_{j=1}^m{\left(\ell(\pi^e_j) - \hat{\ell}(\pi) \right)^2 }}
% %         }
% %         {m}.
% % \end{equation}
% % %
% % Stated alternatively,
% % \begin{equation}
% % \label{eq:bounding-length}
% %     \probP
% %      \left(
% %       \vert  \hat{\ell}(\pi) -\hat{\ell}(\pi) \vert \leq \delta_\ell(\pi) 
% %      \right) 
% %      \geq 1-\alpha.
% % \end{equation}


% % To bound the expected coverage $\vert \bar{\mathcal{S}}(\pi) \vert $, we first bound the uncertainty for each individual POI.
% % Specifically, or any, desired CL between zero and one there is a probability of~$1-\alpha$ (with $\alpha := 1 - \text{CL}$) that the $j$'th POI will be in the interval~$\hat{p}^{\pi}_j \pm \delta_\mathcal{S}(\pi, j)$
% % where 
% % \begin{equation}
% % \delta_\mathcal{S}(\pi, j):= 
% %     Z^*(\text{CL}) 
% %         \cdot 
% %     \sqrt\frac{
% %           \hat{p}^{\pi}_j \cdot (1- \hat{p}^{\pi}_j)
% %         }
% %         {{m}}.
% % \end{equation}

% % We assume independence between inspecting different POIs which allows us to use  the Wald confidence interval~\cite{fagerland2015recommended}.
% % Namely, we define the total confidence interval as the sum of all the confidence intervals of the individual POIs~$\delta_\mathcal{S}:=\sum_{j=1}^{j=m}\delta_\mathcal{S}(\pi, j)$.
% % Subsequently, there is a probability of~$1-\alpha$ that the number of the inspected POI will be in the interval~$\vert \hat{\mathcal{S}}(\pi) \vert  \pm \delta_\mathcal{S}$.

% % In practice, naive calculation of confidence intervals may yield results out of the range $[0,1]$ which is meaningless when discussing probabilities.
% % To this end, we define the positive and negative confidence interval bounds  (denoted as~$\delta_\mathcal{S}(\pi, j)^+$ and ~$\delta_\mathcal{S}(\pi, j)^-$, respectively) separately as follows.
% % %
% % \begin{equation}
% %     \delta_\mathcal{S}(\pi, j)^+ = \min(\hat{p}_j^\pi + \delta_\mathcal{S}(\pi, j),1).
% % \end{equation}
% % %
% % \begin{equation}
% %     \delta_\mathcal{S}(\pi, j)^- = - \max(\hat{p}_j^\pi - \delta_\mathcal{S}(\pi, j),0).
% % \end{equation}

% % Finally, given a command path~$\pi$ with~$m$ MC samples~$\pi^e_i=\mathcal{M}(\pi, \Nloc^i, \Ncon^i)$, we have a probability of~$1-\alpha$ (CL) to inspect POI in range
% % \begin{equation}
% % \sum_{j=1}^{j=m} \hat{p}_j^\pi+[\delta_\mathcal{S}(\pi, j)^-,+\delta_\mathcal{S}(\pi, j)^+].
% % \end{equation}

% % % \begin{equation}
% % % \label{eq:bounding-coverage}
% % %     p(\vert  
% % %     \vert \hat{\mathcal{S}}(\pi) \vert - 
% % %     \vert \bar{\mathcal{S}}(\pi) \vert 
% % %     \vert 
% % %     \leq \delta_\mathcal{S}) \geq 1-\alpha.
% % % \end{equation}

% % \ignore{
% % \subsection{The uncertainty quantification operation \DA{continue (challenge \textbf{C2})}}
% % \label{subsec:The uncertainty quantification operation}

% % The uncertainty quantification operation is performed in advance of extending a node~$n$ from a vertex~$u$ by an edge~$e=(u,v)$ to a vertex~$v$.
% % The main goal of this operation is to calculate the POI probability array~$p_{I}$ given a single inspection at the end of this transition. 
% % The additional purpose is to calculate the expected path length~$E(l(u,v))$ (denoted as~$E(l)$) of this transition.

% % To this end,~\irisuu uses navigation and motion models~$\mathcal{N},\mathcal{M}$ combine with a Monte Carlo (MC) method to simultaneously represents~$m$ possible values for the true configuration~$P^t$ as shown in Algorithm~\ref{alg:Initialize and update the MC samples}. 
% % \begin{algorithm}
% % \caption{Initialize and update the MC samples}
% % \label{alg:Initialize and update the MC samples}
% % \begin{algorithmic}[1]
% % \DontPrintSemicolon
% %     \State \textbf{Init:} 
% %     \For {$j=1$ to $m$} \Comment{Initialize~$m$ MC samples}
% %     \State $q^e_{v_s,j} \leftarrow \text{distribution}$\
% %     \State $\hat{q}_{v_s,j} \leftarrow q_{c_{v_s}}$ \
% %     \State $q^t_{v_s,j} \leftarrow \hat{q}_{v_s,j} +q^e_{v_s,j}$  \
% %     \State $N^s_{v_s},N^e_{v_s} \leftarrow \text{distribution}$
% %     \EndFor
    
% %     \State \textbf{Step:}
% %     \For {$j=1$ to $m$} \Comment{Update the~$m$ MC samples}
% %     \State $q^t_{v,j} \leftarrow \mathcal{M}(q^t_{u,j},q^e_{u,j},q^c_u)$  \
% %     \State $\hat{q}_{v,j} \leftarrow \mathcal{N}(q^t_{u,j},\hat{q}_{u,j},N^s_{u},N^e_{u})$ \
% %     \State $q^e_{v,j} \leftarrow \hat{q}_{v,j} - q^t_{v,j}$\
% %     \State $N^s_{v,j} \leftarrow N^s_{u,j}$, $N^e_{v,j} \leftarrow N^e_{u,j}$\
% %     \EndFor
% % \end{algorithmic}
% % \end{algorithm}

% % That is, given a node at a vertex~$v$, we define each Monte Carlo sample as~$\text{MC}_{v,j}$ (for~$j=1,2,\ldots,m$) that represent a tuple of~$(q^e_{v,j},N^s_{v,j},N^e_{v,j})$  where~$q^e_{v,j}$ is the configuration error so that given the command configuration~$q^c_v$ the true configuration of this sample is~$q^t_{v,j} = q^c_v + q^e_{v,j}$.
% % In addition,~$N^s_{v,j},N^e_{v,j}$ are the navigation system parameters that require to update the~$q^t_{v,j}$ value using~$\mathcal{N},\mathcal{M}$. Here we assume that these parameters~$N^s_{v,j},N^e_{v,j}$ do not change during the operation and as a result it is exist that~$N^s_{v,j}=N^s_{u,j}~\text{and}~N^e_{v,j}=N^s_{u,j}$. 



% % Then, given the~$m$ configurations samples~$q^t_{v,j}$ we calculate~$m$ POI set~$I_{v,j} = \mathcal{S}(q^t_{v,j})$. Each POI set~$I_{v,j}$ is converted into a POI array~$\bar{I}_{v,j}$ with size~$k$ (size of~$\mathcal{I}$) where each element~$\bar{I}_{v,j,i}$ is equal to~$0$ or~$1$ to represent whether a POI~$i$ is inspected.
% % Finally, we summarize all the samples and determine the probability POI array as~$p_{I_v}$ by the average value of all~$m$ options of~$\bar{I}_{v,j,i}$, such that each element~$i$ is defined by:
% % \begin{equation}\label{eq:probabilityPOIarray}
% %     p_{I_i} = \frac{1}{m} \sum_{j=1}^{j=m} \bar{I}_{v,j,i}.
% % \end{equation}

% % An example of calculating X is described in Figure~\ref{fig:Workspace}.
% %  \begin{figure*}[htpb!]
% %     \centering
% %      \includegraphics[]{figs/Workspace.pdf}
% %      \caption{}
% % \label{fig:Workspace}
% % \end{figure*}

% % Similarly, the~$m$ configurations samples~$q^t_{v,j}$ are using also to calculate the expected path length~$E(l)$. 
% % In particular, given the previous and the current configurations samples~$(q^t_{u,j}~ \text{and}~ q^t_{v,j})$, the expected value~$E(l)$ is defined by:
% % \begin{equation}\label{eq:expectedPathLength}
% %     E(l) = \frac{1}{m}\sum_{j=1}^{j=m} l(q^t_{u,j},q^t_{v,j})
% % \end{equation}
% % }

% % % \subsection{Modifying primitive search operations (challenge \textbf{C2})}
% % % \label{subsec:c2_1}

% % % \DA{You can add ignore to this comment or to move it.
% % % I know that you did not finish editing, but ...:
% % % \begin{enumerate}
% % %     \item When we talk about stochasticly dominates with a probability of~$\gamma_{\mathcal{S}}$ or~$\gamma_{\mathcal{\ell}}$.
% % % Is it enough to calculate the probability?
% % % Do we not have to decide in the end whether to do it or not?
% % % This may requires a threshold value.
% % % For this, you need some~$\tau_\gamma$ or~$\tau_\alpha$.
% % % \item Given that we are looking for a threshold value, then referring to the k POI:
% % % I do not understand well in statistics and it seems ok (and very similar to the following methods) to use the overall calculation of~$\gamma_{\mathcal{S}}$.
% % % However, maybe we should follow a common methods to determined the threshold such as Family-wise error rate (FWER) which is:~$\tau_{\alpha_{fixed}} = 1-(1-\tau_\alpha)^m$, 
% % % or use an approximation of Bonferroni method:~$\tau_{\alpha_{fixed}} = \frac{\tau_\alpha}{m}$.
% % % \end{enumerate}
% % % }




% In order to overcome this uncertainty and determine whether~$\vert \expS \vert \geq \kappa \cdot \vert \bar{\mathcal{S}}(\pi^*) \vert$ we can use the null hypothesis testing~(see sec~\ref{subsec:Null Hypothesis Testing}).
% That is, we perform the null hypothesis testing by defining the null hypothesis as~$H_0$ as~$\vert \expS \vert = \kappa \cdot \vert \bar{\mathcal{S}}(\pi^*) \vert$ and the alternative hypothesis~$H_1$ as~$\vert \expS \vert \geq \kappa \cdot \vert \bar{\mathcal{S}}(\pi^*) \vert$.
% As a result the value of~$t$ is:
%~$$
%      t = \frac{\vert \expS \vert - \kappa \cdot \vert \hat{\mathcal{S}}(\pi^*) \vert}
%                  {\sqrt{
%                     \frac{\vert \expS \vert \cdot~(1 - \vert \expS \vert)} {m}
%                     +
%                     \frac{\kappa \cdot \vert \hat{\mathcal{S}}(\pi^*) \vert \cdot~(1 - \kappa \cdot \vert \hat{\mathcal{S}}(\pi^*) \vert)} {m}
%                  }}.
%~$$
% Then, using standard t-statistic tables using~$t$ as an input yield the p-value of~$\gamma \left( \vert \expS \vert \geq \kappa \cdot \vert \hat{\mathcal{S}}(\pi^*) \vert \right)$.
% Finally, this~$\gamma \left( \vert \expS \vert \geq \kappa \cdot \vert \hat{\mathcal{S}}(\pi^*) \vert \right)$ is the p-value for the sub-optimality coverage. 


% the value of~$\vert \estS \vert$ and~$\vert \hat{\mathcal{S}}(\pi^*) \vert$ can be bounded in CI given a desired CL using lemma~\ref{lemma:Bounding executed path's expected coverage}.
% That is, given any desired CL of~$1-\alpha$ we can say that~$ \vert \bar{\S}(\pi) \vert \in 
%     \left[ 
%         \sum_{j=0}^{j=k} \left( \delta_{\mathcal{S},j}^- \right), \sum_{j=0}^{j=k} \left( \delta_{\mathcal{S},j}^+ \right)
%     \right]$, and~$ \vert \bar{\S}(\pi^*) \vert \in 
%     \left[ 
%         \sum_{j=0}^{j=k} \left( \delta_{\mathcal{S}^*,j}^- \right), \sum_{j=0}^{j=k} \left( \delta_{\mathcal{S}^*,j}^+ \right)
%     \right]$.
% Then, we can use the lower bound of~$ \vert \bar{\S}(\pi^*) \vert$ and say that~$\vert \estS \vert$ satisfies~$\vert \estS \vert \geq \kappa \cdot \vert \sum_{j=0}^{j=k} \delta_{\mathcal{S}^*,j}^-$.

% \vspace{2mm} 
% \begin{lemma}[Bounding executed path's sub-optimality]
% Let~$\pi$ be the path obtained by executing the command path~$\pi_{u}$ of~$n^\text{goal}$, and let~$\bar{\ell}(\pi^*)$ be the expected shortest path length of such a path.


% and the estimated expected length~$\estL$, satisfies~$\estL \leq~(1+\epsilon) \cdot \bar{\ell}(\pi^*) + \delta_\ell^+$.
% \end{lemma}


% \vspace{2mm}
% \begin{proof}
% During the search, the nodes in the closed and open list are guaranteed to be \ek-bounded~(see~\cite{fu2019toward} for a proof sketch). 
% Thus, the estimated coverage and length of~$n^\text{goal}$ is \ek-bounded to the \pap optimal inspection plan that can be defined as~$n^\text{goal}$ as~$\vert \bar{\mathcal{S}}(\pi^*) \vert$ and~$\bar{\ell}(\pi^*)$. . 
% However, there is uncertainty for the expectation values.
% % means that there is a CL that the expectation values can be in the CI~(defined in Lemma~\ref{lemma:Bounding executed path's expected length} and~\ref{lemma:Bounding executed path's expected coverage}). 
% Thus, given any desired CL we can use the lower bound of the CI coverage and say that~$\vert \estS \vert$ satisfies~$\vert \estS \vert \geq \kappa \cdot \vert \bar{\mathcal{S}}(\pi^*) \vert -\sum_{j=0}^{j=k} \delta_{\mathcal{S},j}^-$ Similarly, we can use the lower bound of the CI length and say~$\bar{\ell}(\pi)$, satisfies~$\estL$, satisfies~$\estL \leq~(1+\epsilon) \cdot \bar{\ell}(\pi^*) + \delta_\ell^+$.
% \end{proof}




% \end{lemma}

% As a result, we can say with a CL of~$1-\alpha$ that:
% \begin{itemize}
%     \item The executed path~$\pi$ will be at least
%    ~$$
%       \bar{\S}(\pi) \geq  \sum_{j=0}^{j=k} \left( \hat{p}^{\pi_u}_j \right)
   
%         \left( - \delta_{\mathcal{S},j}^- \right), \sum_{j=0}^{j=k} \left( \hat{p}^{\pi_u}_j + \delta_{\mathcal{S},j}^+ \right)
%     .
%    ~$$
% \end{itemize}

% However, since  

% \begin{lemma}[Bounding executed path's sub-optimality]
% During the search, the nodes in the closed and open list are guaranteeing to be \ek-bounded. As a result, the \pap properties represent the optimal inspection plan and the \ap estimated values are \ek-bounded~(see~\cite{fu2019toward} for a proof sketch).
% However, since  



% \end{lemma}

% \vspace{2mm}
% \begin{proof}
% During the search, the remaining nodes in the OPEN list subsumed all other nodes reaching the same vertex and are maintaining the \pap properties~$\tilde{\rm{IPV}}_u$ and~$\tilde{\ell}_u$.


% The subsuming operation maintained the \pap  with other node in the OPEN set except for nodes that were dominated by the nodes of CLOSED set.
% \end{proof}

%  


% Using this calculation, we say with probability of existing path with more coverage than  at most~$\tau_\text{BH}(\Pval_u)$, that there is no other path with smaller expected length that achieves coverage larger or equal to~$\kappa \cdot \vert \mathcal{I} \vert~$. 



% \subsubsection{Demo illustration problem}
% In this section we illustrate \irisuu method using a demo problem. 
% The problem includes a requirement to inspect 3 POI by selecting command path~$\pi$ along a roadmap~$\mathcal{G}$ with 5 vertices and 5 edges in presence of 3 obstacles~(Figure.~\ref{fig:Illustration}).
%  \begin{figure}[ht]
%     \centering
%      \includesvg[inkscapelatex=false, width=0.5\textwidth]{figs/Illustration.svg}
%      \caption{A roadmap~$\mathcal{G}$ with A,B,C,D,E vertices and 5 edges. In addition, the obstacles are marked in brown rectangles and the POI are marked in red circles.}
%      \label{fig:Illustration}
% \end{figure}

% As depicted in Fig.\ref{fig:Illustration_calc} the algorithm was performed using~$3$ MC samples and initiated the first search node from a vertex A as~$n_A := \langle  IPV = \{0.5,0.4,0\},\hat{l} = 0 \rangle$.
% Then, the search is split into two branches~$\{A \rightarrow B, A \rightarrow C\}$.
% In each branch, the value of the IPV and~$\hat{l}$ of the extended node is updated using the value of~$n_A$ and the transition value table.
% For instance, the IPV of~$n_{A \rightarrow B}$ is updated to:
% \begin{equation*}
%     \begin{split}
% IPV = \{1-(1-1)\cdot(1-0.5),\\
%         1-(1-0.67)\cdot(1-0.4),\\
%         1-(1-0)\cdot(1-0)\} = \\
%         =\{1,0.8,0\}.
% \end{split}
% \end{equation*}
% In the same way, the estimated length of~$n_{A \rightarrow B}$ is updated to:
%~$$\hat{l} = 0 + 1.5.$$

% Then, following this guideline, the branches extend and reach a vertex D where the two branches meet together. 
% That is, the first branch has values of:
%~$$n_{A \rightarrow B \rightarrow D} := \langle  IPV = \{1,0.8,0.67\},\hat{l} = 3.5 \rangle,$$ and the second branch has values of:
%~$$n_{A \rightarrow C \rightarrow D} := \langle  IPV = \{0.5,0.4,0.89\},\hat{l} = 3.8 \rangle.$$

%  \begin{figure}[ht]
%     \centering
%      \includesvg[inkscapelatex=false, width=0.5\textwidth]{figs/Illustration_calc.svg}
%      \caption{Extending the search nodes}
%      \label{fig:Illustration_calc}
% \end{figure}

% At this point the algorithm test the node pruning operation. 
% To do so, we use the comparison equations~(Eq.~\ref{eq:p-value-populations},~\ref{eq:p-value-proportions}).
% We can see the results in Fig.\ref{fig:Illustration_calc1}.
%  \begin{figure}[ht]
%     \centering
%      \includesvg[inkscapelatex=false, width=0.5\textwidth]{figs/Illustration_calc_1.svg}
%      \caption{Pruning operation result}
%      \label{fig:Illustration_calc1}
% \end{figure}
% The comparison of the path length result with~$t = 2.32$~\ref{eq:p-value-populations}, then assign is into the t-statistic table result with~$\gamma_{\ell} = 0.92$.
% In a similar way, the comparison of the coverage was performed using Eq.\ref{eq:p-value-proportions} and result with~$t_1 = 1.73,t_2=1.09,t_3=-0.67$, where~$i$ index in~$t_i$ is refer to the POI number. Assign these value into the t-statistic result with~$\gamma_{\mathcal{S}_1} = 0.88,\gamma_{\mathcal{S}_1} = 0.80,\gamma_{\mathcal{S}_1} = 0.28$. Thus, the total value of~$\gamma_\mathcal{S}$ is equal to~$0.2$.
% Following this calculation we say that~$n_{A \rightarrow B \rightarrow D}$ stochastically dominates~$n_{A \rightarrow C \rightarrow D}$ with probability of~$\gamma_{\ell} \cdot \gamma_\mathcal{S} = 19[\%]$.

% \DA{Notice that we get only~$19[\%]$ for the pruning operation. This~(maybe) highlights the need to set a limit for this action}

% It can be seen that the search is not over yet, and that branch~$n_{A \rightarrow B \rightarrow D}$ still does not provide full coverage for the entire POI. However, even at this stage we can evaluate the quality of the solution using equations~\ref{eq:CI_calculation_value},~\ref{eq:CI_calculation_proportions}.
% That is, suppose we require a CL of~$95[\%]$. Then, because of the small number of samples~($3$) we will have to use~$T^*$, when in this case we get~$T^*=4.3$.
% Calculating the values of~$n_{A \rightarrow B \rightarrow D}$ into these equations produces~$\delta_\ell(\pi) = 0.5$.
% Thus, we have a CL of~$95[\%]$ the path length is in~$[3,4]$.

% Similarly, the confidence interval of each POI is:~$\delta_\mathcal{S}_1 = 0, \delta_\mathcal{S}_2 = 0.99, \delta_\mathcal{S}_3 = 1.167$, where the index~$i$ in~$\delta_\mathcal{S}_i$ is the number of the POI.
% Then, due to the very low number of samples, the values of~$\delta_\mathcal{S}_2$ and~$\delta_\mathcal{S}_3$ are high. 
% In this case, the CI value of each POI is limited to~$[0,1]$.
% That is, as state, we need to calculate each side separately and consider the limited values of~$[0,1]$:
% Thus, the positive side is~$1+\textbf{0},0.8+\textbf{0.2},0.67+\textbf{0.33}$, where the value of~$0,0.2,0.33$ are~$\delta_\mathcal{S}(\pi, j)^+$. In addition, the negative side is~$1-\textbf{0},0.8-\textbf{0.8},0.67-\textbf{0.67}$ where the value~$0,-0.8,-0.67$ are~$\delta_\mathcal{S}(\pi, j)^-$.
% Finally, we can say that we have CL of~$95[\%]$ that the number of the POI inspected is in~$[1,3]$.





% % \subsubsection{Bounding path quality}
% % Given a command path~$\pi$ for which we sampled~$m$ execution paths~$\pi^e_1, \ldots, \pi^e_m$,
% % we can bound the quality of our estimated length and coverage.
% % Specifically, following the approach described in Sec.~\ref{subsec:MC-methods} we have the following results:

% % For any, desired CL between zero and one there is a probability of~$1-\alpha$~(with~$\alpha := 1 - \text{CL}$) that the expected path length~$\bar{\ell}(\pi)$ 
% % will be in the interval~$\estL \pm \delta_\ell(\pi)$,\footnote{Strictly speaking,~$\delta_\ell~(\pi)$ should include~$\alpha$ as an additional parameter and should be written as~$\delta_\ell~(\pi, \alpha)$. However, this is omitted for brevity. We do the same for the following derivations.}
% % where 
% % \begin{equation}
% % \delta_\ell(\pi):= 
% %     Z^*(\text{CL}) 
% %         \cdot 
% %     \frac{
% %          \sqrt{\sum_{j=1}^m{\left(\ell(\pi^e_j) - \estL \right)^2 }}
% %         }
% %         {m}.
% % \end{equation}
% % %
% % Stated alternatively,
% % \begin{equation}
% % \label{eq:bounding-length}
% %     \probP
% %      \left(
% %       \vert  \estL -\estL \vert \leq \delta_\ell(\pi) 
% %      \right) 
% %      \geq 1-\alpha.
% % \end{equation}


% % To bound the expected coverage~$\vert \expS \vert~$, we first bound the uncertainty for each individual POI.
% % Specifically, or any, desired CL between zero and one there is a probability of~$1-\alpha$~(with~$\alpha := 1 - \text{CL}$) that the~$j$'th POI will be in the interval~$\hat{p}^{\pi}_j \pm \delta_\mathcal{S}(\pi, j)$
% % where 
% % \begin{equation}
% % \delta_\mathcal{S}(\pi, j):= 
% %     Z^*(\text{CL}) 
% %         \cdot 
% %     \sqrt\frac{
% %           \hat{p}^{\pi}_j \cdot~(1- \hat{p}^{\pi}_j)
% %         }
% %         {{m}}.
% % \end{equation}

% % We assume independence between inspecting different POIs which allows us to use  the Wald confidence interval~\cite{fagerland2015recommended}.
% % Namely, we define the total confidence interval as the sum of all the confidence intervals of the individual POIs~$\delta_\mathcal{S}:=\sum_{j=1}^{j=m}\delta_\mathcal{S}(\pi, j)$.
% % Subsequently, there is a probability of~$1-\alpha$ that the number of the inspected POI will be in the interval~$\vert \estS \vert  \pm \delta_\mathcal{S}$.

% % In practice, naive calculation of confidence intervals may yield results out of the range~$[0,1]$ which is meaningless when discussing probabilities.
% % To this end, we define the positive and negative confidence interval bounds ~(denoted as~$\delta_\mathcal{S}(\pi, j)^+$ and ~$\delta_\mathcal{S}(\pi, j)^-$, respectively) separately as follows.
% % %
% % \begin{equation}
% %     \delta_\mathcal{S}(\pi, j)^+ = \min(\hat{p}_j^\pi + \delta_\mathcal{S}(\pi, j),1).
% % \end{equation}
% % %
% % \begin{equation}
% %     \delta_\mathcal{S}(\pi, j)^- = - \max(\hat{p}_j^\pi - \delta_\mathcal{S}(\pi, j),0).
% % \end{equation}

% % Finally, given a command path~$\pi$ with~$m$ MC samples~$\pi^e_i=\mathcal{M}(\pi, \Nloc^i, \Ncon^i)$, we have a probability of~$1-\alpha$~(CL) to inspect POI in range
% % \begin{equation}
% % \sum_{j=1}^{j=m} \hat{p}_j^\pi+[\delta_\mathcal{S}(\pi, j)^-,+\delta_\mathcal{S}(\pi, j)^+].
% % \end{equation}

% % % \begin{equation}
% % % \label{eq:bounding-coverage}
% % %     p(\vert  
% % %     \vert \estS \vert - 
% % %     \vert \expS \vert 
% % %     \vert 
% % %     \leq \delta_\mathcal{S}) \geq 1-\alpha.
% % % \end{equation}

% % \ignore{
% % \subsection{The uncertainty quantification operation \DA{continue~(challenge \textbf{C2})}}
% % \label{subsec:The uncertainty quantification operation}

% % The uncertainty quantification operation is performed in advance of extending a node~$n$ from a vertex~$u$ by an edge~$e=(u,v)$ to a vertex~$v$.
% % The main goal of this operation is to calculate the POI probability array~$p_{I}$ given a single inspection at the end of this transition. 
% % The additional purpose is to calculate the expected path length~$E(l(u,v))$~(denoted as~$E(l)$) of this transition.

% % To this end,~\irisuu uses navigation and motion models~$\mathcal{N},\mathcal{M}$ combine with a Monte Carlo~(MC) method to simultaneously represents~$m$ possible values for the true configuration~$P^t$ as shown in Algorithm~\ref{alg:Initialize and update the MC samples}. 
% % \begin{algorithm}
% % \caption{Initialize and update the MC samples}
% % \label{alg:Initialize and update the MC samples}
% % \begin{algorithmic}[1]
% % \DontPrintSemicolon
% %     \State \textbf{Init:} 
% %     \For {$j=1$ to~$m$} \Comment{Initialize~$m$ MC samples}
% %     \State~$q^e_{v_s,j} \leftarrow \text{distribution}$\
% %     \State~$\hat{q}_{v_s,j} \leftarrow q_{c_{v_s}}$ \
% %     \State~$q^t_{v_s,j} \leftarrow \hat{q}_{v_s,j} +q^e_{v_s,j}$  \
% %     \State~$N^s_{v_s},N^e_{v_s} \leftarrow \text{distribution}$
% %     \EndFor
    
% %     \State \textbf{Step:}
% %     \For {$j=1$ to~$m$} \Comment{Update the~$m$ MC samples}
% %     \State~$q^t_{v,j} \leftarrow \mathcal{M}(q^t_{u,j},q^e_{u,j},q^c_u)$  \
% %     \State~$\hat{q}_{v,j} \leftarrow \mathcal{N}(q^t_{u,j},\hat{q}_{u,j},N^s_{u},N^e_{u})$ \
% %     \State~$q^e_{v,j} \leftarrow \hat{q}_{v,j} - q^t_{v,j}$\
% %     \State~$N^s_{v,j} \leftarrow N^s_{u,j}$,~$N^e_{v,j} \leftarrow N^e_{u,j}$\
% %     \EndFor
% % \end{algorithmic}
% % \end{algorithm}

% % That is, given a node at a vertex~$v$, we define each Monte Carlo sample as~$\text{MC}_{v,j}$~(for~$j=1,2,\ldots,m$) that represent a tuple of~$(q^e_{v,j},N^s_{v,j},N^e_{v,j})$  where~$q^e_{v,j}$ is the configuration error so that given the command configuration~$q^c_v$ the true configuration of this sample is~$q^t_{v,j} = q^c_v + q^e_{v,j}$.
% % In addition,~$N^s_{v,j},N^e_{v,j}$ are the navigation system parameters that require to update the~$q^t_{v,j}$ value using~$\mathcal{N},\mathcal{M}$. Here we assume that these parameters~$N^s_{v,j},N^e_{v,j}$ do not change during the operation and as a result it is exist that~$N^s_{v,j}=N^s_{u,j}~\text{and}~N^e_{v,j}=N^s_{u,j}$. 



% % Then, given the~$m$ configurations samples~$q^t_{v,j}$ we calculate~$m$ POI set~$I_{v,j} = \mathcal{S}(q^t_{v,j})$. Each POI set~$I_{v,j}$ is converted into a POI array~$\bar{I}_{v,j}$ with size~$k$~(size of~$\mathcal{I}$) where each element~$\bar{I}_{v,j,i}$ is equal to~$0$ or~$1$ to represent whether a POI~$i$ is inspected.
% % Finally, we summarize all the samples and determine the probability POI array as~$p_{I_v}$ by the average value of all~$m$ options of~$\bar{I}_{v,j,i}$, such that each element~$i$ is defined by:
% % \begin{equation}\label{eq:probabilityPOIarray}
% %     p_{I_i} = \frac{1}{m} \sum_{j=1}^{j=m} \bar{I}_{v,j,i}.
% % \end{equation}

% % An example of calculating X is described in Figure~\ref{fig:Workspace}.
% %  \begin{figure*}[htpb!]
% %     \centering
% %      \includegraphics[]{figs/Workspace.pdf}
% %      \caption{}
% % \label{fig:Workspace}
% % \end{figure*}

% % Similarly, the~$m$ configurations samples~$q^t_{v,j}$ are using also to calculate the expected path length~$E(l)$. 
% % In particular, given the previous and the current configurations samples~$(q^t_{u,j}~ \text{and}~ q^t_{v,j})$, the expected value~$E(l)$ is defined by:
% % \begin{equation}\label{eq:expectedPathLength}
% %     E(l) = \frac{1}{m}\sum_{j=1}^{j=m} l(q^t_{u,j},q^t_{v,j})
% % \end{equation}
% % }

% % % \subsection{Modifying primitive search operations~(challenge \textbf{C2})}
% % % \label{subsec:c2_1}

% % % \DA{You can add ignore to this comment or to move it.
% % % I know that you did not finish editing, but ...:
% % % \begin{enumerate}
% % %     \item When we talk about stochasticly dominates with a probability of~$\gamma_{\mathcal{S}}$ or~$\gamma_{\mathcal{\ell}}$.
% % % Is it enough to calculate the probability?
% % % Do we not have to decide in the end whether to do it or not?
% % % This may requires a threshold value.
% % % For this, you need some~$\tau_\gamma$ or~$\tau_\alpha$.
% % % \item Given that we are looking for a threshold value, then referring to the k POI:
% % % I do not understand well in statistics and it seems ok~(and very similar to the following methods) to use the overall calculation of~$\gamma_{\mathcal{S}}$.
% % % However, maybe we should follow a common methods to determined the threshold such as Family-wise error rate~(FWER) which is:~$\tau_{\alpha_{fixed}} = 1-(1-\tau_\alpha)^m$, 
% % % or use an approximation of Bonferroni method:~$\tau_{\alpha_{fixed}} = \frac{\tau_\alpha}{m}$.
% % % \end{enumerate}
% % % }




==> sections/OldText.tex <==

\subsection{Modifying primitive search operations (challenge \textbf{C2})}
\label{subsec:c2_1}

In this section we define the actions: extending, dominating and subsuming. 

\subsubsection{Node definition}
\label{subsubsec:Node definition}
First, we assume that given a command path~$\pi$ we have~$m$ execution paths~$\pi^e$ (Using motion model of Eq.~\ref{eq:motion_model_paths}). 
Given these~$m$ possible path we assume to have the inspection probability vector of~$\rm{IPV}(\pi)$ (Eq.~\ref{eq:IPV}) and
estimated expected coverage~$\vert \hat{\mathcal{S}}(\pi) \vert$ (Eq.~\ref{eq:estimated expected coverage}). 
Furthermore, we assume to have the estimated expected length~$\hat{\ell}(\pi)$ (Eq.~\ref{eq:estimated expected length}).
% In addition, we define~$\alpha_{\text{diff}}^{(\mathcal{S}(\pi_u))}$ and~$\alpha_{\text{diff}}^{(\ell(\pi_u))}$ 
% Then, we define the node~$n$ (of the search algorithm) as a tuple of~$(\pi,\pi^e,\rm{IPV}(\pi),\hat{\ell}(\pi),\alpha(\mathcal{S}(\pi)),\alpha(\ell(\pi))$, where~$\pi$ is the command path and~$\pi^e$ is the~$m$ executing paths.
% In addition,~$\rm{IPV}(\pi)$ is the inspection probability vector  and~$\hat{\ell}(\pi)$ the estimated expected length.
% Moreover,~$\alpha(\mathcal{S}(\pi))$ and~$\alpha(\ell(\pi))$ are the p-value of the comparison tests (to be defined shortly and used in the following operations).
Finally, we define the node~$n$ (of the search algorithm) as a tuple of~$(\pi,\pi^e,\rm{IPV}(\pi),\hat{\ell}(\pi))$.

Specifically, we denote the node~$n_u =(\pi_u,\pi_u^{e},\rm{IPV}(\pi_u),\hat{\ell}(\pi_u)$ to represent a path~$\pi_u$ that starting at $q_{\rm start}$ and ending at some configuration $u$.

\subsubsection{Extending operation}
\label{subsubsec:Extending operation}
Extending a node~$n_u$ with the path~$\pi_{u \rightarrow v}$ (from a configuration~$u$ to~$v$) will create a node~$n_v = (\pi_v,\pi^e_v,\rm{IPV}(\pi_v),\hat{\ell}(\pi_v))$, where:
\begin{enumerate}
    \item $\pi_v$ is the result of concatenating the path~$\pi_u$  with~$\pi_{u \rightarrow v}$ (from a configuration~$u$ to~$v$) such that the path~$\pi_v$ is defined as:
    $$\pi_v:= \pi_u + \pi_{u \rightarrow v}.$$
    \item Each executing path~$\pi^{e_u}_i$ (element~$i$ of~$\pi^{e_u}$) is the result concatenating it by~$\pi^{e_{u \rightarrow v}}_i$ such that:~
    $$\pi^{e_v}_i = \pi^{e_u}_i +\pi^{e_{u \rightarrow v}}_i. $$
    \item Given estimated expected length of the segment~$\hat{\ell}(\pi_{u \rightarrow v})$, then the The estimated expected length of~$\pi_v$ is determined by:
    $$\hat{\ell}({{\pi}}_v):= \hat{\ell}({{\pi}}_u) +\hat{\ell}(\pi_{u \rightarrow v}).$$
    \item In our model the inspection action is preformed discreetly along the path segments and we assume that each such an action is independent. Thus, given the IPV of the path segment~$\pi_{u \rightarrow v}$ then, each element~$j$ of~$\rm{IPV}(\pi_v)$ is determined by:
    $$\hat{p}_j^{\pi_v} := 
     1-(1-\hat{p}^{\pi_{u \rightarrow v}}_{j}) \cdot (1-\hat{p}_j^{\pi_{u}}).$$
\end{enumerate}

\subsubsection{Dominating operation}
\label{subsubsec:Dominating operation}
Given a node~$n_u$ and a node~$n'_u$ that both starting at $q_{\rm start}$ and ending at some configuration $u$. Then, for testing whether~$n_u$ dominates $n'_u$ we first perform the p-value comparison of the length and coverage. 
That is, we calculate~$\alpha_p(\bar{\ell}(\pi_u))~\geq~\bar{\ell}(\pi'_u)))$ (see Eq.~\ref{eq:p-value-populations}), and for each POI we calculate~$\alpha_p(\hat{p}_j^{\pi_u}~\geq~\hat{p}_j^{\pi'_u})$ (see Eq.~\ref{eq:p-value-proportions}).
Then, given user-provided~$\tau_{\alpha}$, we say that~$n_u$ dominates $n'_u$ 
if~$\alpha_p(\bar{\ell}(\pi_u))~\geq~\bar{\ell}(\pi'_u))) \leq \tau_{\alpha}$,
and 
for each POI~$\alpha_p(\hat{p}_j^{\pi_u}~\geq~\hat{p}_j^{\pi'_u})\leq \tau_{\alpha}$. 

\DA{What to do with multiple hypothesis?}

% Then, we temporary assign~$\alpha_p^{\bar{\ell}}$ to express the updated p-value for the previous comparisons and the current comparison of the expected length, such that:
% \begin{equation}
%     \alpha_p^{\bar{\ell}}:=1-(1-\alpha_p(\bar{\ell}(\pi_u)~\geq~\bar{\ell}(\pi'_u))\cdot\alpha_p^{\ell(\pi_u)}).
% \end{equation}
% Similarly, we temporary assign~$\alpha_p^{\mathcal{S}}$ to express the updated p-value for the previous comparisons and the current comparison of the POI inspection, such that for each POI~$j$ is defined by:
% \begin{equation}
%     \alpha_p^{\mathcal{S}_j}:=1-(1-\alpha_p(\hat{p}_j^{\pi_u}~\geq~\hat{p}_j^{\pi'_u})\cdot\alpha_p^{\hat{p}_j^{\pi_u}}).
% \end{equation} 

% Then, we use the Bonferroni’s method for multiple test p-value~[ref{todo}], and determined the threshold of the POI testing to be~$\frac{\tau_{\alpha_p}}{m}$ (where~$m$ is the number of Monte Carlo sample)
% .
% Then, if~$\alpha_p^{\bar{\ell}} \leq \tau_{\alpha_p}$ and for each POI~$\alpha_p^{\mathcal{S}} \leq \frac{\tau_{\alpha_p}}{m}$ we say that~$n_u$ dominates $n'_u$ and update the value of the p-value of~$n_u$ by the temporary values. Namely:
% \begin{equation}
%     \begin{split}
%         \alpha_p^{\ell(\pi_u)} = \alpha_p^{\bar{\ell}},\\
%         \alpha_p^{\mathcal{S}(\pi_u)} =  \alpha_p^{\mathcal{S}}.
%     \end{split}
% \end{equation}










\OS{This is a place where I threw some old text that may be reused}



\section{Problem Definition}
\label{Sec:ProblemDefinition}

\OS{I think this section should be divided into three parts:
(i) robot navigation model
(ii) planning phases (offline vs. online - planning vs execution)
(iii) inspection planning}

In this section we provide a formal definition of the inspection-planning problem under execution uncertainty.
In this problem, we are given 
a robot $\mathcal{R}$ operating in a workspace~$\mathcal{W} \subset \mathbb{R}^3 $  amidst a set of (known) obstacles~$ \mathcal{W}_{obs} \subset \mathcal{W}$.
A \emph{configuration}~$q$ is a $d$-dimensional vector uniquely describing the robot's poistion and orientation and let~$\mathcal{X}\subset\mathbb{R}^d$ denote the robot's \emph{configuration space}.
Let $\text{Shape}: \mathcal{X} \rightarrow 2^\mathcal{W}$ be a function mapping a configuration~$q$ to the workspace region occupied by $\mathcal{R}$ when placed at $q$.
We say that~$q \in \mathcal{X}$ is \emph{collision free} if~$\text{Shape}(q) \bigcap \mathcal{W}_{obs} = \emptyset$.

The robot receives as input a set of \emph{points of interest} (POI)  $ \mathcal{I} = \{i_1, \ldots, i_k \} \subset \mathcal{W}$ which should be inspected using some on-board inspection sensors (e.g., a camera). We model the inspection  sensors as a mapping~$\mathcal{S}: \mathcal{X}\rightarrow 2^\mathcal{I}$, where~$2^\mathcal{I}$ is the power set of~$\mathcal{I}$, such that~$\mathcal{S}(q)$ denotes the subset of~$\mathcal{I}$ that can be inspected from configuration~$q\in \mathcal{X}$.
We define a \emph{path}~$P$ in~$\mathcal{X}$ as a sequence of configurations~$(q_0,q_1,\ldots )$ 
%(vertices) 
connected by straight-line segments 
%(edges) 
in~$\mathcal{X}$.
As we will see, we will often treat paths as (one-dimensional) graphs and thus we will often refer to configurations along the path as \emph{vertices} and to the straight-line segments connecting them as edges.
Finally, by a slight abuse of notation we define $\mathcal{S}(P):=\bigcup_{i} \mathcal{S}(q_i)$ to be the POI that can be inspected by traversing the path~$P$. 
Note that in our model, we only inspect POI along path vertices.

\OS{define different stages of planning process}

As we are concerned with planning in a prepossessing stage while accounting for execution uncertainty, we will consider several types of paths:
%
A \emph{command path}~$P^c = \{ q^c_0,q^c_1,\ldots\,q^c_{n-1} \}$ is a path computed offline which  should be interpreted as a sequence of~$n$ \emph{command configurations} that the robot is expected  to visit in the execution stage.
%
The \emph{executed path}~$P^t=\{q^t_0,q^t_1,\ldots\,q^t_{n-1}\}$ is the set of configurations visited in the execution stage while following a given command path $P^c$. Note that $P^t$ may differ from~$P^c$ due to localization uncertainty.
%

\OS{CONTINUE HERE}

Then, we assume that in the first step~$(i = 0)$,~$q^t_0$ and an estimated configuration denoted as~$\hat{q}_0$ can be received as input from an external system.

In addition, we assume the existence of a navigation model~$\mathcal{N}$ such that given navigation sensors parameters~(denote as~$N^s$), estimator parameters~(denote as~$N^e$), the current true configuration~$q^t_i$ and previous estimated configuration~$\hat{q}_{i-1}$, it returns an estimated configuration~$\hat{q}_i$, formally:~$\hat{q}_i =\mathcal{N}(q^t_i,\hat{q}_{i-1},N^s,N^e)$.
At each step, the robot reaches~$q^t_i$ approximated as~$\hat{q}_i$ and determines that~$q^c_i$ is visited if~$\hat{q}_i=q^c_i$.
However,~$\hat{q}_i$ may be different from~$q^t_i$ so we define~$q^e_i$ as an error configuration such that~$q^e_i = \hat{q}_i - q^t_i$.
Then, for each next step~($i \geq 1$) we define a motion model~$\mathcal{M}$ such that given~$q^t_{i-1}$,~$q^e_{i-1}$ and~$q^c_i$ it returns the updated true configuration~$q^t_i$, formally:~$q^t_i = \mathcal{M}(q^t_{i-1},q^e_{i-1},q^c_i)$.
Notice that, we assume that in the first step~$(i = 0)$,~$q^t_0$ and~$\hat{q}_0$ can be received as input from an external system.


We are ready to define our problem. 
We assume that the robot starts its task in a configuration~$q^t_0$ that is estimated as~$\hat{q}_0$.
Then, our goal is to compute a command-planning path $P^c$, which yields an execution path $P^t$, such that the expression $|\mathcal{S}(P^t)|$ is maximized.
In addition,~$P^t$ has to be as short as possible and collision-free.

\OS{*** David's explanation regarding model (there is a relevant figure in slack***}
%
\OS{
Just trying to clarify the concepts a bit:
Navigation Model refers only to the robot's ability to know or evaluate its configuration as a function of information coming from the navigation sensors from the true configuration $q^t$ (translation between $q^t$ and $q^e$).
Then there should be a Guidance and Control Model (that we have chosen to skip this step in defining the problem), which accepts the estimate configuration $q^e$ and the command configuration $q^c$ and translates it into commands such as engine operating power, etc. - suppose we denote this in $\delta$.
Only then, the Motion Model is relevant, which receives the control commands $\delta$, the real configuration $q^t$, and calculates the next real configuration.
%
The addition of the simplified description is relevant to both the Navigation Model and the Guidance and Control Model and the Motion Model when it means ``giving up'' on a full and complex modeling in favor of something fast and simple.
If there are no Ideal Navigation Model errors then $q^e$ is always equal to $q^t$. Because in this ideal case there is no need to model the motion because we assume that the robot will always reach $q^c$ (except for the accuracy tolerance of the guidance and control system which is usually very small).
%
As a result of all these definitions, it can be understood that the true configurations of the robot varies depending on the precision of $q^e$. And here is the difference between open-loop and closed-loop:
In the case of closed-loop the true configuration of the robot is unique and known (to the motion model). As a result the navigation sensors receive information of a single real configuration (but noisy etc.).
In open-loop, however, the true configuration is not unique.
}

\section{new problem definition}
\OS{add here text on inspection planning}

In this work we are studying the problem of offline inspection planning under uncertainty.
%
Specifically, we assume that the robot operates under two sources of uncertainty: 
(i)~\emph{localization uncertainty} and
(ii)~\emph{control uncertainty}.

%
The localization uncertainty is the main source of error that corresponds with the fact that certain navigation model parameters that determine the robot's pose (position and attitude) are not accurately known and need to be modeled as a random variable.
This may include navigation sensor parameters such as the biases an inertial measurement unit~\ref{}.
%
The secondary uncertainty is the control uncertainty stems from the kinematics constraints
corresponds with the fact that even given no localization uncertainty, when following a given (pre-computed) path $P$ there is uncertainty with respect to reaching an exact location.

We assume that we have access to a distribution $\Dloc$ for which the parameters governing the localization uncertainty~$\Nloc$ is drawn.
Similarly, we assume that we have access to a distribution $\Dcon$ for which the parameters governing the control uncertainty $\Ncon$ is drawn.
%
Finally, we assume that we have a motion model $\mathcal{M}$ that, given a path $P$, localization and control uncertainty parameters $\Nloc, \Ncon$ outputs the path that the robot will take when following $P$ assuming that its uses the parameters $\Nloc, \Ncon$. 

We are finally ready to formally introduce the offline inspection planning under uncertainty.
%
However, before doing so, we need to define the expected length and inspection of a path computed in an offline stage.
%
To do so, recall that we assume that we are given 
a robot $\mathcal{R}$
        operating in a workspace~$\mathcal{W}$,
        a set of POIs $\mathcal{I}$,
        a sensor model $\mathcal{S}$
        and a collision-free start configuration $q_{\rm start}$  (i.e., ${\rm Shape}(q_{\rm start}) \notin \mathcal{X}_{\rm obs}$).


\vspace{3mm}
\begin{dfn}
The \emph{expected length} of a path $P$ is a path that maximizes
\begin{equation}
\bar{\ell}(P)
    := E_{\Nloc \sim \Dloc, \Ncon \sim \Dcon}
        \left[
            \ell
                \left(
                    \mathcal{M}(P,\Nloc, \Ncon)
                \right)
        \right].
\end{equation}

\end{dfn}
%

\vspace{3mm}
\begin{dfn}
The \emph{expected coverage} of a path $P$ is a path that maximizes
\begin{equation}
\bar{\mathcal{S}}(P)
    := E_{\Nloc \sim \Dloc, \Ncon \sim \Dcon}
        \left[
            \vert
            \mathcal{S}
                \left(
                    \mathcal{M}(P,\Nloc, \Ncon)
                \right)
            \vert
        \right].
\end{equation}

\end{dfn}

\DA{TO-DO: converting~$\bar{\mathcal{S}}(P)$ into a scalar that expressing the sum of POI probabilities or into a vector}


\vspace{3mm}
\begin{prob}
%\label{prob-1}
    In the \emph{offline inspection planning under uncertainty} we wish to compute in an offline phase a path $P$ that maximizes its expected coverage~$\bar{\mathcal{S}}(P)$.
    Out of all such paths we wish to compute whose expected length~$\bar{\ell}(P)$ is maximal.
\end{prob}
\vspace{3mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As we cannot directly compute 
$\bar{\ell}(P)$ and $\bar{\mathcal{S}}(P)$ 
we will use \emph{estimations} of these values and denote the \emph{estimated path length}
and
\emph{estimated path coverage}
as
$\hat{\ell}(P)$ and $\hat{\mathcal{S}}(P)$, respectively.
As a result, we define the problem as follows: 
%

\vspace{3mm}
\begin{prob}
% \label{prob-2}
  In the \emph{offline inspection planning under uncertainty} we wish to compute in an offline phase a path $P$ that maximizes its estimated expected coverage~$\hat{\mathcal{S}}(P)$.
  Out of all such paths we wish to compute whose estimated expected length~$\hat{\ell}(P)$ is maximal.
\end{prob}
\vspace{3mm}

However, calculating  the values of~$\hat{E}[\mathcal{S}]$ and~$\hat{E}[l]$ accurately, may requires an high-computational effort. Thus, it will be useful to quantify the difference between the estimated and expected path length and coverage. 
This will be done using the notion of a \emph{confidence level} and \emph{confidence interval}.
%
Specifically, given a path $P$ and estimations $\hat{\ell}(P)$ and $\hat{\mathcal{S}}(P)$, we say that we have a confidence level of~$\alpha$ that the estimations are inside confidence intervals of~$\delta_{\ell}$ and~$\delta_{\mathcal{S}}$, such that:
$$
\vert 
 \bar{\ell}(P) - \hat{\ell}(P)
\vert
 \leq \delta_{\ell}
 \text{ and }
\vert 
 \bar{\mathcal{S}}(P) - \hat{\mathcal{S}}(P)
\vert
 \leq \delta_{\mathcal{S}}.
$$

Using these notations, we define the problem as follows: 

\vspace{3mm}
\begin{prob}
% \label{prob-3}
      In the \emph{offline inspection planning under uncertainty} we wish to compute in an offline phase a path $P$ that maximizes its estimated expected coverage~$\hat{\mathcal{S}}(P)$, both with maximizing~$\alpha$ and minimizing~$\delta_{\mathcal{S}}$.
      Out of all such paths we wish to compute whose estimated expected length~$\hat{\ell}(P)$ is maximal, both with maximizing~$\alpha$ and minimizing~$\delta_{\ell}$.
\end{prob}
\vspace{3mm}

Nonetheless, an optimal solution to problem~\ref{prob-3} also may requires an high-computational effort. Thus, we would like to allow sub-optimal requirements using  two parameters~($\epsilon \geq 0$ and~$p \in (0, 1]$) such that the proposed path is at most~$1+\epsilon$ of the optimal path length while covering at least~$p$-percent of the required POI set covered by the optimal path. As a result, we define the problem as follows: 


\DA{TO-DO: Insert~$\epsilon$ and~$p$ into prob 4. Currently, this is a copy from prob 3}
\vspace{3mm}
\begin{prob}
% \label{prob-4}
      In the \emph{offline inspection planning under uncertainty} we wish to compute in an offline phase a path $P$ that maximizes its estimated expected coverage~$\hat{\mathcal{S}}(P)$, both with maximizing~$\alpha$ and minimizing~$\delta_{\mathcal{S}}$.
      Out of all such paths we wish to compute whose estimated expected length~$\hat{\ell}(P)$ is maximal, both with maximizing~$\alpha$ and minimizing~$\delta_{\ell}$.
\end{prob}
\vspace{3mm}






\section{Random spew of thoughts}


\OS{Since we use the \iris machinery, we actually don't compute a minimal-length path but a bounded sub-optimal approximation of it (with respect to path length). Can we say that we compute a bounded-optimal approximation solution to Prob.~\ref{prob-1}? If so, the statements should probably be probabilistic assuming that the number of MC paths used $m$ tends to $\infty$.}
%As shown by Fu et al.~\cite{fu2019toward, FuSA21}, the offline inspection planning (without accounting for execution uncertainty) is already extremely challenging from a computational point. Thus, in this work we relax the requirement to compute.

\OS{Do we want to limit the paper to graph search?}

\OS{Here I really go on a tangent}

In essence, every node in the search tree is a random variable.
%
We could consider the search tree in an MCTS style. This is a reasonable ask from a reviewer. Why didn't we do it? How hard is it to do?
Once the problem is framed the way it is, we need to think of algorithms to solve searches on stochastic trees. 
Isn't this actually an MDP (or maybe a POMDP)? 
Can be use Value Iteration / Policy Iteration or even LAO*? I think there is a fundumental difference but I'm not sure.
\DA{I think the difference between these methods is because it's because of lack of observation. The POMDP method for example assumes that \textbf{there is an observation} from the real world (or from a simulation). But, since we are both offline and open-loop and at the planing stage then the measurements are not considered observation, and there is no ability for one measurement from Monte Carlo to have a more significant weight than others.
The lack of observation is the main reason why we did not use these methods, although there are similarities.}
\section{Algorithmic Approach}
In this work we take an open-loop planning approach in which we compute in an offline stage a command path $P^c$ that may differ from the path $P^t$ that will be executed by the robot.
%
To estimate $P^t$, we assume that the offline has access to a motion model~$\mathcal{M}$ which, in turn, is a function of the navigation model~$\mathcal{N}(N_s, N_e)$ 
%that usually returns stochastic values of~$\hat{q}_i$.
As an accurate motion model is typically computationally expensive to execute a common approach is to use a simplified motion model during offline planning.

To this end, we use a simplified motion model~$\mathcal{M}'$ (to be detailed in Sect.~\ref{Sec:Modeling the localization uncertainty}) with which we can define the estimated true path as~$\hat{P^t}$ and estimate the POI set as~$\mathcal{S}(\hat{P}^t)$.
As a result, the problem is re-defined as follows:
Assuming the robot begins its mission at~$\hat{q}^t_0$ (as a result of a command to start in configuration~$q^c_0$), the problem calls for computing command-path~$P^c$ which yields an estimated execution path $\hat{P}^t$, such that the expression $|\mathcal{S}(\hat{P}^t)|$ is maximized.
Finally, to evaluate our approach, we assume to have access to an external simulator that allows us to test the planning quality with~$|\mathcal{S}(P^t)|$.



\subsection{Incremental Random Inspection-roadmap Search (IRIS)}

IRIS is a computationally-efficient inspection-planning algorithm that interleaves sampling-based motion planning and graph search to enable the computation of a provably near-optimal inspection path~\cite{fu2019toward}.

IRIS incrementally constructs a roadmap~$\mathcal{G}$ using Rapidly-exploring Random Graphs (RRG)~\cite{karaman2011sampling}, where~$\mathcal{G}=(\mathcal{V},\mathcal{E})$ is a motion-planning roadmap in which every vertex~$v \in V$ is a robot configuration~$q \in \mathcal{X}$ and every edge~($u,v$) denotes the transition from configuration~$u$ to~$v$.
In addition, IRIS defines a \emph{path pair}~$\text{PP}_v = (P_v,\tilde{P}_v)$ represents a paths starting at~$q_s$ and end at a vertex~$v \in \mathcal{V}$ where~$P_v$ and ~$\tilde{P}_v$ are an \emph{achievable path} (AP) and a \emph{potentially achievable path} (PAP) to the vertex~$v$, respectively.
The PAP is intended to bound the AP quality in the search algorithm (to be detailed shortly) with two parameters~($\epsilon \geq 0$ and~$p \in (0, 1]$) such that the AP is at most~$1+\epsilon$ of the PAP length while covering at least~$p$-percent of the POI set covered by the PAP.

To compute the planned path, IRIS performs a search algorithm where the search node is defined as a tuple~$n = (v, I_v,\text{PP}_v)$, where~$I_v$ is the POIs covered by the AP~$P_v$.
This path pair~$\text{PP}_v$ is used to define the POI sets~$(\mathcal{S}(P_v),\mathcal{S}(\tilde{P}_v))$ and the minimum costs~$l(P_v),l(\tilde{P}_v)$, and for convenience, we define~$(\mathcal{S}(P_v),\mathcal{S}(\tilde{P}_v))$ as~$(I_v,\tilde{I}_v)$ and~$l(P_v),l(\tilde{P}_v)$ as~$l_v,\tilde{l}_v$.
Thus, here we describe the search algorithm with an equivalent definition for the node~$n$, such that the node~$n$ is defined as a tuple~$(v, P_v, I_v,l_v,\tilde{I}_v,\tilde{l}_v)$ \footnote{In the IRIS algorithm, the path pair is intended to define these parameters and we want to explain our updating through it. In addition,~$\tilde{P_v}$ is not part of the node~$n$ since the PAP is not necessarily a realizable path, and it is needed only to determine~$\tilde{I}_v,\tilde{l}_v)$.}. 
 
%Then, during the search algorithm (to be defined shortly) the solution quality is guaranteed by having~$\text{PP}_v$ maintained to be~$\epsilon,p$-bounded such that (i)~$l_v \leq (1 + \epsilon)\tilde{l}_v$ and (ii)~$|I_v| \geq p \dot |\tilde{I}_v|$.

%Then, IRIS define an \emph{inspection graph}~$G_s = (\mathcal{V}_s,\mathcal{E}_s)$.~$G_s$ represents a path beginning at a start configuration~$q_s$, where each vertex~$\mathcal{V}_s$ is composed of a vertex~$v \in \mathcal{V}$ of the original graph~$\mathcal{G}$ and the POI sets of the path pair~$(I_v,\tilde{I}_v)$. In addition, each edge~$\mathcal{E}_s$ is the costs of the path pair~$l_v,\tilde{l}_v$.
 

The search algorithm is detailed \cite{fu2019toward} and here is only a briefly describing of it. 
The algorithm sorts the node into an OPEN and CLOSED set. 
It starts with an empty CLOSED set and an OPEN set with a trivial path pair,~$PP_{q_s}$, where both AP and PAP represent the trivial path~$\{q_s\}$.
At each iteration, it pops the most promising node from the OPEN set and checks if the search can terminate. If not, the node is added to the CLOSED set and \emph{extended} with its neighbors.

\begin{definition}
\textbf{Extending operation}: 
Extending a node$n =  (u,P_u,I_u,l_u,\tilde{I}_u,\tilde{l}_u)$ by an edge~$e = (u,v)$, yields an extended node$n =  (v,P_v,I_v,l_v,\tilde{I}_v,\tilde{l}_v)$, in which the AP parameters are updating such that~$P_v = P_u +e$,~$l_v = l_u+l(e)$,~$I_v = I_u \bigcup I_v$. In a similar way the PAP parameters are updating such that,~$\tilde{l}_v = \tilde{l}_u+l(e)$ and~$\tilde{I}_v= \tilde{I}_u \bigcup \mathcal{I}_{v}$.
\end{definition}


Then, for each extended node, the algorithm tests if and how to add it to the OPEN set, by the following operations.
As a starting point, If there exists a node from the CLOSED set that can \emph{dominates} it then the extended node is discarded. 

\begin{definition}
	\textbf{Dominating operation}: 
	Given any node~$n'$ from the CLOSED set and the extended node~$n$, then~$n'$ is said to be dominates~$n$ if~$l'_v \leq l_v$ and~$I'_v \supseteq I_v$.
\end{definition}


Then, to reduce the number of paths considered by the search, the algorithm tests for each extended node~$n$ the \emph{subsuming operation}(to be defined shortly).
If there exists a node from the OPEN set~$n'$ that can subsume the extended node~$n$, then~$n'$ is updating and~$n$ is discarded.
Then, for any node in the OPEN set~$n'$ that can be subsumed by the extended node~$n$, then~$n$ is updating and~$n'$ is removed from the OPEN set. 
If the extended node~$n$ not being discard during this process then~$n$ is added to the OPEN set.

\begin{definition}
   \textbf{Subsuming operation}: For each two nodes~$n^1 =  (v,P_v^1,I_v^1,l_v^1,\tilde{I}_v^1,\tilde{l}_v^1)$ and~$n^2 =  (v,P_v^2,I_v^2,l_v^2,\tilde{I}_v^2,\tilde{l}_v^2)$ that end at the same vertex~$v$, the operation of~$n_1$ subsuming~$n_2$ (denoted as~$n_1 \bigoplus n_2$) will create a new node~$n^3$ that equals to~$(v,P_v^1,I_v^1,l_v^1, \tilde{I}_v^1 \cup \tilde{I}_v^2, min(\tilde{l}_v^1,\tilde{l}_v^2))$. 
\end{definition}


The subsuming operation allows to reduce the number of paths considered by the search. 
However, to ensure that the solution returned by the algorithm approximates the optimal inspection path, subsuming only occurs when the resultant node~$n^3$ is~$\epsilon,p$-bounded such that (i)~$l_v^3 \leq (1 + \epsilon)\tilde{l}_v^3$ and (ii)~$|I_v^3| \geq p \dot |\tilde{I}_v^3|$.

IRIS's approach to speeding-up performance and to obtain a suitable path in a relatively short time is to start the search from a small size roadmap~$G$ and suboptimal values for~$\epsilon,p$ ($\epsilon \geq 0$ and~$p \leq 1]$).
Then, as time allows, the search is repeated while the roadmap~$G$ is incrementally densified, and the approximated parameters~$\epsilon,p$ are tightened~($\epsilon$ decreases and~$p$ increases). 
As a result, in each search iteration, the planned path is asymptotically converged to the optimal solution.




\subsection{Modifying primitive search operations (challenge \textbf{C2})---OLD}
\label{subsec:c2}

As stated,~\irisuu uses an inspection probability vector (Equation~\ref{eq:inspection probability vector}) instead of a POI set.
Thus, to consider this change in the algorithm, the terms~$I_u$ and~$\tilde{I}_u$ of the search node are replaced with the probability notation~$p_{I_u}$ and~$p_{\tilde{I}_u}$, respectively.
In addition, each node has to maintain the~$\text{MC}$ parameter that is required for the uncertainty quantification operation. 
As a result, the node~$n$ is re-defined as a tuple~$(u,P_u,p_{I_u},l_u,p_{\tilde{I}_u},\tilde{l}_u,\text{MC}_u)$.
and the algorithm operations (dominating, extending, and subsuming) are redefined also to match the probability notation in an equivalent algorithmic meaning.

\begin{definition}
\textbf{Dominating operation}: Given any node~$n'$ from the CLOSED set and the extended node~$n$, then~$n'$ is said to be dominates~$n$ if~$l'_v \leq l_v$ and each~$i=1, \ldots ,k$, holds that~$p_{I'_v} \geq p_{I_v}$, where~$p_{I'_v}$ and~$p_{I_v}$ are the POI probabilities elements of the CLOSED set node and the extended node, respectively.
\end{definition}

\OS{This definition is somewhat problematic. 
The fact that one inspection probability vector dominates another does not mean that one path is better than the other.
This is because each vector is a random variable.
We probably need to use CL+CI to say something here.
This is super important or else we give up on any guarantees (which I think we can provide if we do things carefully)}

\begin{definition}
\textbf{Extending operation}: 
Extending a node~$n =  (u,P_u,p_{I_u},l_u,p_{\tilde{I}_u},\tilde{l}_u,\text{MC}_u)$ by an edge~$e = (u,v)$ starts with the uncertainty quantification operation which updates~$\text{MC}_v$ and calculates the POI probability array~$p_I$(Equation~\ref{eq:probabilityPOIarray}) and the expected length~$E(l)$ (Equation~\ref{eq:expectedPathLength}).
This extending operation result with an extended node~$n =  (v,P_v,p_{I_v},l_v,p_{\tilde{I}_v},\tilde{l}_v,MC_v)$, in which~$P_v = P_u +e$,~$l_v = l_u+E(l)$ and~$\tilde{l}_v = \tilde{l}_u+l(e)$. 
In addition,~$p_{I_v}$ is updating such that each element~$p_{I_v}^i = 1-(1-p_I)\cdot(1-p_{I_u}^i)$ where~$p_{I_v}^i$ and~$p_{I_u}^i$ represent the probability to inspect the POI~$i$ from the vertices~$v$ and~$u$ respectively.  
In a similar way,~$p_{\tilde{I}_v}^i$ is updating such that~$p_{\tilde{I}_v}^i = 1-(1-p_I)\cdot(1-p_{\tilde{I}_u}^i)$. 
\end{definition}

\begin{definition}
  \textbf{Subsuming operation}: Given two nodes~$n^1 =  (v,P_{v}^1,p^1_{I_{v}},l^1_{v},p^1_{\tilde{I}_{v}},\tilde{l}^1_{v},\text{MC}^1_{v})$ and~$n^2 =  (v,P_{v}^2,p^2_{I_{v}},l^2_{v},p^2_{\tilde{I}_{v}},\tilde{l}^2_{v},\text{MC}^2_{v})$ that end at the same vertex~$v$. 
  Then, the operation of~$n_1$ subsuming~$n_2$ (denoted as~$n_1 \bigoplus n_2$) will create a new node~$n^3=(v,P_{v}^1,p^1_{I_{v}},l^1_{v},\text{max}(p_{\tilde{I}^1_{v}},p_{\tilde{I}^2_{v}}), \text{min}(\tilde{l}^1_v,\tilde{l}^2_v),\text{MC}^1_{v})$ where the notation~$\text{max}(p_{\tilde{I}^1_{v}},p_{\tilde{I}^2_{v}})$ is a new array that takes the maximum value of each element. 
\end{definition}




% \section{Methods}
% \label{Methods}

% The motion plan of IRIS is interpreted as a command path~$P^c$ that the robot is instructed to visit in the execution stage. However, it is usually different from the executed path~$P^t$ and as a result the executed POI set~$\mathcal{S}(P^t)$ may differ from the planning set~$\mathcal{S}(P^c)$.
% To this end, below we present our method \emph{IRIS-under-uncertainty},~$\text{IRIS-U}^2)$, that considers the uncertainty of the execution within the IRIS inspection-planning algorithm.

% \subsection{\irisuu}
% \label{IRIS-U}
% \irisuu method aims to allow execution uncertainty to be considered throughout casting it into a POI uncertainty.


 
% That is, to inspect the POI the robot is equipped with a sensor model~$\mathcal{S}$ that returns the POI set that is inspected from a given configuration.
% Due to uncertainty in the execution process, the robot reaches true configuration~$q^t_i$ (that may be different from the command configuration~$q^c_i$) and the POI set of~$i$ is~$\mathcal{S}(q^t_i)$.
% However, the value of~$q^t_i$ is not known precisely during the planning and we can only estimate it as~$\tilde{q}^t_i$.
% Thus, we define whether each POI is inspected with a probability value in range~$[0,1]$ (instead of a binary notation (0 or 1)), expressing the belief in the inspection success of each POI. 

% To do so, we cast the POI set~$\mathcal{I}$ into an array~$\hat{\mathcal{I}}$ in size of the goal POI set~$\mathcal{I}$.
% In particular, suppose~$\mathcal{I}$ includes~$k$ POI, then~$\hat{\mathcal{I}} = \{\text{POI}_1,\text{POI}_2,\ldots,\text{POI}_k \}$, where each~$\text{POI}_i = \hat{\mathcal{I}}_i $ express whether a POI~$i$ is inspected.
% Then, for each command configuration~$q^c_i$, we calculate~$m$ possible options of~$\mathcal{I}_i$ using~$m$ possible options of the true configuration~$q^t_i$ (to be detailed shortly).
% Each option~$j$ for~$j=1,2,\ldots m$ are used to determine a different array~$\hat{\mathcal{I}}_{ij}$ (where~$i$ is the configuration index and~$J$ is the possible index).
% Finally, we define the probability POI array of configuration~$i$ as~$p(\hat{\mathcal{I}}_i)$ denote by the average value of all~$m$ options of the POI array, formally:
% \begin{equation}
%     p(\hat{\mathcal{I}}_i) = \frac{1}{m} \sum_{j=1}^{j=m} \hat{\mathcal{I}}_{ij}  
% \end{equation}

% In addition, inspection operations are performed during the planning at each arrival to configuration~$i$.
% Thus, we define~$p(\hat{\mathcal{I}})$ (without the configuration index~$i$) as the total POI array probability maintained by each node of the search graph.
% Then, given a current total POI array probability~$p(\hat{\mathcal{I}})$ and probability POI array (of configuration~$i$)~$p(\hat{\mathcal{I}}_i)$, we define the update value of the total POI array probability as~$p(\hat{\mathcal{I}})^{\text{update}}$, according to the following equation:
% \begin{equation}\label{eq:combineInspectOperationPOI}
%     p(\hat{\mathcal{I}})^{\text{update}} = 1 - (1-p(\hat{\mathcal{I}}_i))(1-p(\hat{\mathcal{I}}))
% \end{equation}

% In a similar way, the~$m$ possible options of~$q^t_i$ are using also to update the value of the edge length of the~$i$ configuration with the expected value denote as~$E(l)_i$ . In particular, for each option~$j$ (~$j=1,2,\ldots m$) of the previous and current true configurations~$q^t_{i-1},q^t_{i}$ , we define the~$j$ possible length as~$l(q^t_{{ij}-1},q^t_{ij})$ and the expected value~$E(l)_i$, formally:
% \begin{equation}
%     E(l)_i = \frac{1}{m}\sum_{j=1}^{j=m} l(q^t_{{ij}-1},q^t_{ij})
% \end{equation}

% In addition, the total edge length maintained by each node of the search graph is defined as~$E(l)$ (without the configuration index~$i$).
% Then, given a current total edge length~$E(l)$ and edge length (of configuration~$i$)~$E(l)_i)$, we define the updated value of the total edge length as~$E(l)^{\text{update}}$, according to the following equation:
% \begin{equation}\label{eq:combineInspectOperationLength}
%     E(l)^{\text{update}} = E(l) + E(l)_i
% \end{equation}

% We can now reformulate the problem objective using this notation. That is, we aim to compute path~$P^c$ while maximizing~$p(\hat{\mathcal{I}})$ and minimizing~$E(l)$.

% It remains to describe how the determine the~$m$ possibilities of~$q^t_i$.
% To do so, we represent the possible values of~$q^t_i$ with an execution-process model using Monte Carlo samples calculated simultaneously during planning.

% This process is defined as follow:
% We define each sample~$j$ ($j=1,2,\ldots, m$) as a tuple of the parameters required for the motion model, formally:
% %\begin{equation}
% %    MC_j = (\vec{b_a}_j,\vec{b_g}_j,\sigma_{\text{coverage}}_j,t^{W^{\text{denied}}}_j)
% %\end{equation}
% Then, each sample independently performs a motion model calculation as depicted in Algorithm~\ref{alg:motion-model algorithm}.

% By using such an approach, it is not necessary to minimize the LU for the inspection task. However, to avoid collisions, we suggest limiting the LU value.
% That is, if 
% Notice that, exist~$e_{q_i}$ sample such that~$e_{q_i}> e_q^{\text{max}}$ the new extension node will be removed.
% %     {Remove new extension node
% % This determination is made for each sample individually. That is, for each sample, we calculate the expected value of the true configuration as assuming the previous error value, such that~$q^t_i_{\text{expected}} = q^c_i + e_q_{i-1}$. Then, if~$q^t_i_{\text{expected}} \in W^{\text{coverage}}$ we update~$q^t_i$ using Equation~\ref{eq:qt_wcov}, otherwise we update its value using Equation~\ref{eq:qt_wden}.

% By using this approach, we suggest adding a property of the~$MC$ sample to the node tuple, such that~$(v,\mathcal{I}_{v}, PP_{v}, MC)$
% By using this approach, we re-define the extend operation. That is, extending the path pair~$PP_u$ by the edge~$e = (u,v)$, yields an extended path pair$PP_v$ in which~$P_v = P_u +e$ and~$\tilde{P}_v = \tilde{P}_u +e$ as the same of the original algorithm.

% In contrast, because of the error configuration value~$e_q$, the edge length~$l(e)$ and the POIs inspected did not remain the same. 
% By the~$MC$ property, the value of the edge length~$l(e)$ is updated using Equation~\ref{eq:combineInspectOperationLength} and the value of the total POI probability is updated using Equation~\ref{eq:combineInspectOperationPOI}.

% This operation is performed on the currently extended node path~$P$ and any path~$P'$ from the CLOSED set that starts and ends at the same
% vertices. That is,~$P'$ is dominates~$P$ if~$l(P') \leq l(P)$ and~$S(P') \supseteq S(P)$ and the current extended node is removed.

% In addition, we need to re-define the \emph{dominance} operation. 
% That is, the POI set is casting to a POI array so also the \emph{dominance} operation definition does not remain the same. That is, in the POI set notation, any path~$P'$ from the CLOSED set that starts and ends at the same
% vertices as the currently extended node path~$P$ is defined to dominate the current node, if~$S(P') \supseteq S(P)$.

% In the notation of POI array, given a two POI array~$p(\hat{\mathcal{I}})_1$ and~$p(\hat{\mathcal{I}})_2$, then~$p(\hat{\mathcal{I}})_1$ is dominates$p(\hat{\mathcal{I}})_2$ if any POI probability value in~$p(\hat{\mathcal{I}})_1$ is larger than~$p(\hat{\mathcal{I}})_2$.   

% The IRIS-U algorithm to update the value of~$p(\hat{\mathcal{I}})$ and~$E(l)$ is detailed in Algorithm~\ref{alg:IRIS-U algorithm}

% %\begin{algorithm}[H]
% %\DontPrintSemicolon
% %\SetAlgoVlined
% %
% %\state \textbf{Init:} 
% %
% %\state Initialize~$m$ MC motion-model samples.
% %
% %\state Calculate~$m$ POI array~$\hat{\mathcal{I}}_0$ using~$m$ options of~$q^t_0$.
% %
% %\state $p(\hat{\mathcal{I}}) \gets \frac{1}{m} \sum_{j=1}^{j=m} \hat{\mathcal{I}}_{0j}$
% %
% %\state $E(l) \gets \frac{1}{m}\sum_{j=1}^{j=m} l(q^t_{{0j}-1},q^t_{0j})$
% %
% %\state \textbf{Step:}
% %
% %\state Update~$m$ MC motion-model samples.
% %
% %\If{exist $e_{q_i}$ sample such that~$e_{q_i}> e_q^{\textbf{max}}$}
% %    {Remove new extension node}
% %\Else{
% %\state Calculate~$m$ POI array~$\hat{\mathcal{I}}_i$ using~$m$ options of~$q^t_i$.
% %
% %\state $p(\hat{\mathcal{I}}) = 1 - (1-\frac{1}{m} \sum_{j=1}^{j=m} \hat{\mathcal{I}}_{ij})(1-p(\hat{\mathcal{I}}))$.
% %
% %\state $E(l) \gets E(l) + \frac{1}{m}\sum_{j=1}^{j=m} l(q^t_{{ij}-1},q^t_{ij})$
% %}
% %\label{alg:IRIS-U algorithm}
% % \caption{IRIS-U algorithm}
% %\end{algorithm}

% Notice that, given a roadmap~$G$ and~$k$ POI, there may be a case where there is a solution to the original IRIS algorithm while following the LU there is no solution. Thus, IRIS-U continues the IRIS approach to incrementally increasing the roadmap~$G$ to asymptotic convergences to the optimal solution.
% In addition, according to the MC theory (detailed in Section~\ref{Monte Carlo methods}), to get an optimal solution we need to choose~$m \rightarrow \infty$. However, using a large number of samples during the search will significantly increase the computation time. 
% Thus, initially, we will perform a search with a relatively low number of~$m$. Then, as time allows, we will gradually increase~$m$ so the solution converges asymptotically to the optimal solution.
% Alternatively, we can use the Function~\ref{eq:CICL} and stop the search with a sufficient CL and CI.

 

% The method can access via 'git@github.com: DavidAlpert11/IRIS-UAV-MC.git'



% Recall that for the bridge inspection, the mission is done by a UAV equipped with a GNSS-INS navigation system which affects the localization uncertainty of the execution performance.
% To simulate this system, we assume that the workspace~$\mathcal{W}$ is divided into two navigation regions~$W^{\text{coverage}}$ and~$W^{\text{denied}}$, which represents the regions with and without a GNSS signal, respectively. The division of the workspace into these two regions is important because performing a command path throughout~$W^{\text{coverage}}$ allows the UAV to use its full navigation capabilities and achieve low localization uncertainty. In contrast, performing the command path throughout~$W^{\text{denied}}$ relies mainly on IMU measurements, which can produce errors due to bias, scale factor, cross-coupling, and random noise.
% Specifically, we assume that under the bridge the GNSS receiver suffers from GNSS outages. As a result, we define~$W^{\text{denied}}$ to be within the range of~$50 \leq x \leq 100$,~$-11 \leq y \leq 1$, and~$-20 \leq z \leq 0$, and~$W^{\text{coverage}}$ otherwise. 

% During the execution phase, a UAV simulator (see Appendix~\ref{app:UAV simulator}) allows us to test and evaluate the UAV's execution performance in different scenarios. The simulator employs an Extended Kalman Filter (EKF) motion model that fuses measurements from the GNSS and the INS to provide reliable navigation solutions. However, the~$\mathcal{M}_{\text{full}}$ motion model requires a significant amount of computation time. Therefore, to speed up calculations during the planning phase, we choose to use a simplified GNSS-INS motion model denoted as~$\MsimpleBridge$.
% This motion model~$\MsimpleBridge$ is based on~\cite{bookGroves} and estimates the location errors at each node, assuming that the robot moves at a constant speed in a straight line between nodes. In particular, we defined~$\MsimpleBridge$ as follows. Let
% $$\pi^c:= \langle x_1^c,y_1^c,z_1^c,\phi_1^c,\psi_1^c,\theta_1^c \rangle,\langle x_2^c,y_2^c,z_2^c,\phi_2^c,\psi_2^c,\theta_2^c \rangle,\ldots,$$
% be a command-path, and let define any sample of the execution path as:
% $$\pi^e:= \langle x_1^e,y_1^e,z_1^e,\phi_1^e,\psi_1^e,\theta_1^e \rangle,\langle x_2^e,y_2^e,z_2^e,\phi_2^e,\psi_2^e,\theta_2^e \rangle,\ldots.$$
% In addition, let us assume that the robot follows its orientation command perfectly such that~$[\phi_j^e,\psi_j^e,\theta_j^e] = [\phi_j^c,\psi_j^c,\theta_j^c]$. However, its location is affected by the localization uncertainty of each region differently and we simulate each configuration~$q_i$ as:
% \begin{enumerate}
% \item If~$q_i \in W^{\text{coverage}}$, we assume that the navigation system can use both the GNSS and INS. Thus we model the configuration location as:
% \begin{equation}\label{eq:qt_wcov}
% [x_i^e,y_i^e,z_i^e] = [x_i^c,y_i^c,z_i^c] + \mathcal{N} \thicksim \left(0,\sigma_{\text{coverage}} \right),
% \end{equation}
% where~$\sigma_{\text{coverage}}$ is the standard deviation of~$W^{\text{coverage}}$ and we assume that~$\sigma_{\text{coverage}}=1$.
% \item If~$q_i \in W^{\text{denied}}$, we assume that the navigation system can use only the INS system. In addition, in most cases, the accelerometer and gyro unknown biases of the IMU are the dominant source of error and are denoted by the vectors~$\vec{b_a} = \mathcal{N}(0,\sigma_{b_a})$ and~$\vec{b_g} = \mathcal{N}(0,\sigma_{b_g})$, where~$\sigma_{b_a},\sigma_{b_g}$ are their standard deviation, respectively. These biases cause a significant error as time goes on and we model the accumulation error of~$\mathcal{W}^{\text{denied}}$, as:
% \begin{equation}\label{eq:qt_wden}
% [x_i^e,y_i^e,z_i^e] = [x_i^c,y_i^c,z_i^c] +\frac{1}{2}C_b^i \vec{b_a} t^2 + \frac{1}{6}C_b^i (\vec{b_g} \times \vec{g}) t^3.
% \end{equation}
% Here~$\vec{g}$ is the gravity vector defined as~$\left( 0,0,-g \right)$,~$C_b^i$ is the rotation matrix from the body frame to an inertial frame and~$t$ is continuous time in~$W^{\text{denied}}$.               
%         \end{enumerate}

\subsection{Result and implications of the Bridge scenario}
\label{subsec:Result and implications of the Bridge scenario} 

% \begin{figure}[tb]
%         \centering
%          \includegraphics[width=0.5\textwidth]{figs/bridgeScenarioResultspath.eps}
%          \caption{Command path of \iris (blue line) and \irisuu (red line) with~$m=50$ for the bridge scenario with the~$\MsimpleBridge$.}
%     \label{fig:Bridge_scenario_resultspath}
% \end{figure} 


==> sections/OldTheoretical.tex <==
\subsection{\irisuu---Theoretical guarantees}
\label{subsec:Theoretical guarantees}
In this section, we detail different statistical on the command path computed by \irisuu using the statistical methods outlined in Sec.~\ref{subsec:Monte-Carlo methods statistical tests}. 

% Recall that in Prob.~\ref{prob-4}, the goal is to find an optimal command path, denoted as~$\pi^*$, that maximizes POI coverage and has the minimal path length among all such paths. For sub-optimal solutions, we introduced two  approximation factors~$\epsilon \geq 0$ and~$\kappa \in (0, 1]$ such that the resulting command path~$\pi$ must satisfy the following constraints:
% \begin{equation}
% \begin{split}
% \vert \hat{\mathcal{S}}(\pi) \vert \geq & \kappa \cdot \vert \hat{\mathcal{S}}(\pi^*) \vert, \\
% \hat{\ell}(\pi) \leq & (1+\epsilon) \cdot \hat{\ell}(\pi^*).
% \end{split}
% \end{equation}

% The \irisuu algorithm follows the \iris objective and addresses this problem iteratively. In each iteration, the algorithm receives an input of a roadmap~$\G$ and uses~$m$ MC samples to find a goal node represented by the tuple:
% $$
% n^\text{goal} =
% \langle
% u, \pi_u, \Pi^e_u, \hat{\rm{IPV}}_u, \hat{\ell}_u,
% \tilde{\rm{IPV}}_u,\tilde{\ell}_u,\colProbHat{{,u}}
% \rangle.
% $$
% To find the resulting command path~$\pi_u$ of~$n^\text{goal}$, \irisuu simulate its~$m$ possible execution paths~$\Pi^e_u$ by a motion model~$\mathcal{M}$ and calculates the estimated POI IPV~$\hat{\rm{IPV}}_u$ and the estimated path length~$\hat{\ell}_u$ of the execution phase as well as the estimated collision probability~$\colProbHat{{,u}}$.
% At each iteration,~$\irisuu$ addresses a \pap~$\tilde{\pi}$ performance denoted as~$\tilde{\rm{IPV}}_u$ and~$\tilde{\ell}_u$ such that each node maintains:
% \begin{equation}
% \begin{split}
% \vert \hat{\mathcal{S}}(\pi_u) \vert \geq & \kappa \cdot \vert \hat{\mathcal{S}}(\tilde{\pi}_u) \vert, \\
% \hat{\ell}(\pi_u) \leq & (1+\epsilon) \cdot \hat{\ell}(\tilde{\pi}_u).
% \end{split}
% \end{equation}

% \OS{This is super weird! why is this in the theoretical guarantees? This looks like a description of the algorithm?}
% As the algorithm progresses, it iteratively densifies the motion-planning roadmap~$\G$ and tightens the requirements,~$\epsilon$ and~$\kappa$. 

% It has been previously proven in the original \iris (see~\cite{fu2019toward}) that as much the roadmap~$\G$ is more densified (includes more possible paths) and~$\epsilon \rightarrow 0, \kappa \rightarrow 1$, then without execution uncertainty the produced path~$\pi_u$ will converge to the optimal path~$\pi^*$.
% In \irisuu, we suggest continuing this objective and providing in this section theoretical guarantees to converge the optimal path~$\pi^*$ under execution uncertainty.
% To this end, we use the statistical methods outlined in sec.~\ref{subsec:Monte-Carlo methods statistical tests} and tighten also the value of MC samples~$m$ as the algorithm progresses. 




\vspace{2mm}
\begin{lemma}[Bounding executed path's expected coverage]
\label{lemma:Bounding executed path's expected coverage}
% Let~$\pi_{u}$ be the \ap of the goal node~$n^\text{goal}$.
% In addition, assuming a scenario with~$k$ POI where~$\hat{\rm{IPV}}(\pi_{u}) := \{ \hat{p}_1^{\pi_{u}}, \ldots, \hat{p}_k^{\pi_{u}} \}$ is the inspection probability vector of~$n^\text{goal}$, and~$\vert \hat{\S}(\pi_{u}) \vert = \sum_{j=1}^{j=k} \hat{p}_j^{\pi_{u}}$ is the estimated execution path coverage.
Let~$\pi_{u}$ be the \ap of the goal node~$n^\text{goal}$,~$\hat{\rm{IPV}}(\pi_{u}) := \{ \hat{p}_1^{\pi_{u}}, \ldots, \hat{p}_k^{\pi_{u}} \}$ the inspection probability vector of~$n^\text{goal}$, and~$\vert \hat{\S}(\pi_{u}) \vert = \sum_{j=1}^{j=k} \hat{p}_j^{\pi_{u}}$ the estimated execution path coverage of~$n^\text{goal}$.
%
Then, for any desired CL of~$1 - \alpha$, with~$\alpha \in [0,1]$
the executed path's expected coverage, denoted by~$\vert \bar{\S}(\pi_{u}) \vert$, has a lower bound value of:
\begin{equation}\label{eq:CI-coverage-lemma2}
    \vert \bar{\S}(\pi_{u}) \vert^- =  \sum_{j=1}^{j=k}  \hat{p}^-(\hat{p}_j^{\pi_{u}},m,\alpha). 
\end{equation}
% \begin{equation}\label{eq:CI-coverage-lemma2}
%     \vert \bar{\S}(\pi_{u}) \vert  \in 
%     \left[ 
%         \sum_{j=1}^{j=k}  \hat{p}^-(\hat{p}_j^{\pi_{u}},m,\alpha) , \sum_{j=1}^{j=k}  \hat{p}^+(\hat{p}_j^{\pi_{u}},m,\alpha) 
%     \right].
% \end{equation}
Here, the function~$\hat{p}^-$ is defined in Eq.~\ref{eq:Clopper-Pearson method}.   
\end{lemma}

\vspace{2mm}
\begin{proof}
Recall that~$\hat{p}_j^{\pi_{u}}$ is the estimated probability to inspect POI $j$ computed by $m$ independent samples of execution paths (represented by~$\Pi^e_u$). 
%
To compute the CI of~$\hat{p}_j^{\pi_{u}}$, we use  Eq.~\ref{eq:Clopper-Pearson method}. 
Specifically, 
for any desired CL of~$1 - \alpha$, with~$\alpha \in [0,1]$ the coverage lower bound of:
$$
    \hat{p}_j^{\pi_{u}}^- =  \hat{p}^-(\hat{p},m,\alpha).
$$

Now, since inspecting each POI does not affect the inspection of any other POI, thus their inspection outcomes are independent.
As a result, the CI of the sum of the POIs is a sum of~$m$ CI independent binomial distribution and can be computed by adding the standard errors of each individual CI~\cite{}. Namely,
$$
    \vert \bar{\S}(\pi_{u}) \vert^-  = \sum_{j=1}^{j=k}  \hat{p}_j^{\pi_{u}}^- = \sum_{j=1}^{j=k} (\hat{p}_j^{\pi_{u}},m,\alpha)
$$
\end{proof}

Lemma~\ref{lemma:Bounding executed path's expected coverage} provides bounds the expected coverage of the executed path. The following lemma refines this by providing a connection between the system's parameters $m$ and $\kappa$ and the lower bound presented in Lemma~\ref{lemma:Bounding executed path's expected coverage}. As we will see, this will allow us to provide clear guidelines on how to choose $m$ and $\kappa$.

% \begin{color}{red}
% Now we can take a one step ahead. Recall that the user chooses the approximation parameter~$\kappa$ to bound the estimated POI coverage~$\vert \hat{\S}(\pi_{u}) \vert$ of the executed path such that~$\vert \hat{\S}(\pi_{u}) \vert = \sum_{j=1}^{i=k}  \hat{p}_j^{\pi_u} 
%     \geq 
% \kappa  \cdot
% \sum_{j=1}^{i=k}  \hat{p}_j^{\tilde{\pi}_u},$ (see Eq.\ref{eq:ek-bounded}).
% However, the value of~$\vert \hat{\S}(\pi_{u}) \vert$ is estimated with only a limited number of~$m$ MC samples and according to lemma~\ref{lemma:Bounding executed path's expected coverage} its lower bound is defined by~$\sum_{j=1}^{j=k}  \hat{p}^-(\hat{p}_j^{\pi_{u}},m,\alpha)$ which is depending in~$\kappa$ as well as~$m$ and~$\alpha$.
% Thus, we wish to allow the user to choose for each iteration of \irisuu the minimal tuple~$\langle \kappa,m,\alpha \rangle$ such that we can be sure that the resultant executed path's expected coverage will exceeds a desire value.
% In order to calculate that lower bound we need to know the value of each~$\hat{p}_j^{\pi_{u}}$ and before running the algorithm we do not know that value but only that~$\sum_{j=1}^{j=k} \hat{p}^-(\hat{p}_j^{\pi_{u}},m,\alpha) \geq \kappa \cdot k$.
% Let's define it as an optimization problem:
% \begin{prob}\label{prob_choose_sub_optimal_parameters}
% We aim to find:
%   ~$$\min_{m, \kappa,\alpha} \vert \bar{\mathcal{S}}({\pi}_{u}) \vert = \min_{m, \kappa,\alpha} \sum_{j=1}^{j=k} \hat{p}^-(\hat{p}_j^{\pi_{u}},m,\alpha)$$
% subject to
% \begin{align*} 
% \sum_{j=1}^{j=k} \hat{p}_j^{\pi_u} &\geq \kappa \cdot k, \ \quad \forall j, 0 \leq \hat{p}_j^{\pi_u} \leq 1 . 
% \end{align*}
% \end{prob}
% \end{color}


\vspace{2mm} 
\begin{lemma}[\parbox{0.48\linewidth}{\centering {Bounding executed path's \\ sub-optimal coverage}}]
% \begin{lemma}[Bounding executed path's sub-optimal coverage]
\label{lemma:Bounding executed path's sub-optimal coverage}
~

Let~$\pi_{u}$ be the \ap of the goal node~$n^\text{goal}$ and let~$\hat{\rm{IPV}}(\pi_{u}) := \{ \hat{p}_1^{\pi_{u}}, \ldots, \hat{p}_k^{\pi_{u}} \}$ be the inspection probability vector of~$n^\text{goal}$
such that
that~$\sum_{j=1}^{j=k} \hat{p}_j^{\pi_u} \geq \kappa \cdot k$.
%
If we set~$\vert \bar{\mathcal{S}}^-({\pi}_{u}) \vert := \sum_{j=1}^{j=k} \hat{p}^-(\hat{p}_j^{\pi_{u}},m,\alpha)$ 
then, for any values of $m,k$ and $\alpha$ we have that
\begin{equation}
\label{eq:lemma_pj_kappa}
    \min_{\hat{\rm{IPV}}(\pi_{u})} \vert \bar{\mathcal{S}}^-({\pi}_{u}) \vert
    = \sum_{j=1}^{j=k} \hat{p}^-(\hat{p}_j^{\pi_u},m,\alpha) 
    = k \cdot \hat{p}^-(\kappa,m,\alpha).
\end{equation}
Namely, minimizing~$\vert \bar{\mathcal{S}}^-({\pi}_{u}) \vert$ s.t.
(i)~$\hat{p}_j^{\pi_{u}} \in [0,1]$
and
(ii)~$\sum_{j=1}^{j=k} \hat{p}_j^{\pi_u} \geq \kappa \cdot k$
yields that 
$\forall j,\hat{p}_j^{\pi_{u}} = \kappa$.
\end{lemma}

\begin{proof}
Throughout this proof, we assume that~$m$ and~$\alpha$ are fixed.
As we will analyze $\hat{p}^-(\kappa,m,\alpha)$, it will be convenient to consider only the first variable.
To this end, we denote 
$$f(x): = \hat{p}^-(x,m,\alpha).$$ 
Thus, we need to show that~$\min_{x_j} \sum_{j=0}^{j=k} f(x_j)$ s.t. 
(i)~~$\forall j, x_j \in [0,1]$
and
(ii)~$\sum_{j=1}^{j=k} x_j \geq k \cdot \kappa$ 
is~$k \cdot f(\kappa)$ which means that~$\forall j,x_j = \kappa$. 

\begin{color}{red}
Recall that $\kappa \in [0,1]$. Thus, given the constraints that $\sum_{j=1}^{j=k} x_j \geq k \cdot \kappa$ and $\forall j, x_j \in [0,1]$, then if $\kappa=1$, it follows that $\forall j, x_j = 1$. In this case, the minimum value of $\sum_{j=0}^{j=k} f(x_j)$ is equal to $k \cdot f(\kappa) = k \cdot f(1)$.

Now, consider the case where $\kappa < 1$ and there exists a constant $\kappa' \in [\kappa,1)$ such that $\sum_{j=1}^{j=k} x_j = k \cdot \kappa' \geq k \cdot \kappa$. we can prove that $\min_{x_j} \sum_{j=0}^{j=k} f(x_j) = k \cdot f(\kappa')$ by contradiction.

That is, consider that minimizing~$\sum_{j=0}^{j=k} f(x_j)$ is achieved for some values~$x_1^*, \ldots, x_k^*$ which are not all equal to~$\kappa'$.
Thus, there must exist some~$j$ s.t. ~$x_j^* > \kappa'$, and assume w.l.o.g that this happens for $j=1$. Namely~$\exists \delta_1 >0$ s.t. $x_1^*  = \kappa'  + \delta_1$.
Since the average of all~$x_j$ is equal to $\kappa'$, there must exist some~$j > 1$s.t.~$x_j^* < \kappa'$, and assume w.l.o.g that this happens for~$j=2$. Namely~$\exists \delta_2 >0$ s.t. $x_2^*  = \kappa'  - \delta_2$.
\end{color}
Let~$\delta = \min(\delta_1, \delta_2)$. Then, consider the following solution $x_1', \ldots, x_k' $ to our minimization problem:
$x_1' = x_1^* - \delta$, 
$x_2' = x_2^* + \delta$
and
$x_j' = x_j^*$ for $2<j\leq k$.
Notice that this is a valid solution (i.e.,~$\forall j, x_j' \in [0,1]$ and~$\sum_{j=1}^{j=k} x_j' \geq k \cdot \kappa'$). 
%
We will show that $\sum_{j=0}^{j=k} f(x_j') < \sum_{j=0}^{j=k} f(x_j^*)$ which will lead to a contradiction that minimizing~$\sum_{j=0}^{j=k} f(x_j)$ is  achieved for  $x_1^*, \ldots, x_k^*$.


As $x_j' = x_j^*$ for $2<j\leq k$, to show that $\sum_{j=0}^{j=k} f(x_j') < \sum_{j=0}^{j=k} f(x_j^*)$, it suffices to show that
$$
f(x_1') + f(x_2') < f(x_1^*) + f(x_2^*).
$$
This will be done using the fact that $f(\cdot)$ is a strictly convex function (we will show this numerically shortly).
Namely, that~$\frac{\partial^2 f(x)}{\partial^2 x} >0,\forall x \in [0,1]$
which implies (see, e.g.,~\cite{grasmair2016basic}) that~$\forall \lambda$ s.t. $0 < \lambda < 1$  we have
%
\begin{equation}\label{eq:convex_property_1}
 f(\lambda x_1 + (1-\lambda) x_2) < \lambda f(x_1) + (1-\lambda) f(x_2).
\end{equation}

Thus,
\begin{equation*} 
\begin{split}
    f(x_1') + f(x_2') 
        & = f(x_1^* - \delta) + f(x_2^* + \delta) \\
        & \stackrel{(1)}{=} f(x_1^* - \lambda (x_1^* - x_2^*)) + f(x_2^* + \lambda (x_1^* - x_2^*))\\
        & = f(\lambda x_2^* + (1-\lambda)x_1^*) + f(\lambda x_1^* + (1-\lambda)  x_2^*)\\
        & \stackrel{(2)}{<} (1-\lambda) f(x_1^*) +\lambda f(x_2^*) +
            \lambda f(x_1^*) + (1-\lambda) f(x_2^*) \\
        & = f(x_1^*) + f(x_2^*).
\end{split}
\end{equation*}
  Explanation for the non-trivial transitions:
  (1)~here, we use $\lambda= \delta / (x_1^* - x_2^*)$ and note that $0 < \lambda < 1$ \OS{why?},
  (2)~here, we use Eq.~\ref{eq:convex_property_1}.


\begin{color}{red}

We have now established that~$\min_{x_j} \sum_{j=0}^{j=k} f(x_j)$ is obtained when~$\forall j, x_j=\kappa'$ as expressed in Eq.~\ref{eq:proof_kappa'}:
\begin{equation}\label{eq:proof_kappa'}
\min_{x_j} \sum_{j=0}^{j=k} f(x_j)=k \cdot f(x_j)=k \cdot f(\kappa').
\end{equation}

It remains to prove that minimizing~$\min_{x_j} \sum_{j=0}^{j=k} f(x_j)$ yield that~$\kappa' = \kappa$ which will be done by contradiction. 
Specifically, suppose that minimizing~$\min_{x_j} \sum_{j=0}^{j=k} f(x_j) = k \cdot f(\kappa')$ (as given by Eq.~\ref{eq:proof_kappa'}) is achieved by values of~$x_j$ s.t. $\forall j, x_j = \kappa'> \kappa$.
Namely~$\exists \delta >0$ s.t. $\kappa' = \kappa  + \delta$.
However, the constraint $\sum_{j=1}^{j=k} x_j \geq k \cdot \kappa$ is still satisfied even when~$\sum_{j=1}^{j=k} x_j = k \cdot \kappa$, meaning that the solution~$\forall j,x_j=\kappa$ is also valid.
As a result, following Eq.~\ref{eq:proof_kappa'} yield that minimizing~$\min_{x_j} \sum_{j=0}^{j=k} f(x_j)$ results with~$k \cdot f(\kappa)$.
Then, we will show shortly that~$f(\kappa) <f(\kappa') = f(\kappa+\delta)$ which will lead to a contradiction that~$\kappa'>\kappa$.

%
This will be done using the fact that~$f(\cdot)$ is an increased function (we will show this numerically shortly).
Namely, that~$\frac{\partial f(x)}{\partial x} >0,\forall x \in [0,1]$
which implies that for~$x_1,x_2$ and~$f(x_1),f(x_2)$:
\begin{equation}\label{eq:f_is_an increased_function}
    x_1 < x_2 \iff f(x_1)< f(x_2)
\end{equation}
Thus, by setting~$x_1 = \kappa, x_2 = \kappa'=\kappa+\lambda$ we get that:
$$
\kappa < \kappa+\lambda \Rightarrow f(\kappa)< f(\kappa+\lambda).
$$

Finally, showing that $f$ is an increased and a strictly convex function is non-trivial and we resort to numerical methods.
%
\begin{figure}[tb]
\begin{subfigure}[c]{.24\textwidth}
  % \centering
  % include third image
  \includegraphics[width=\textwidth]{figs/derivative2_p_m_alpha01.eps}  
  \caption{$\alpha = 0.1$}
  \label{fig:sub-third}
\end{subfigure}
\begin{subfigure}[d]{.24\textwidth}
  % \centering
  % include fourth image
  \includegraphics[width=\textwidth]{figs/derivative2_p_m_alpha005.eps}  
  \caption{$\alpha = 0.05$}
  \label{fig:sub-fourth}
\end{subfigure}
\begin{subfigure}[c]{.24\textwidth}
  % \centering
  % include third image
  \includegraphics[width=\textwidth]{figs/derivative_p_m_alpha01.eps}  
  \caption{$\alpha = 0.1$}
  \label{fig:sub-third}
\end{subfigure}
\begin{subfigure}[d]{.24\textwidth}
  % \centering
  % include fourth image
  \includegraphics[width=\textwidth]{figs/derivative_p_m_alpha005.eps}  
  \caption{$\alpha = 0.05$}
  \label{fig:sub-fourth}
\end{subfigure}
\caption{Values of~$\frac{\partial^2 \hat{p}^-(\hat{p}_j^{\pi_u},m,\alpha)}{\partial^2 \hat{p}_j^{\pi_u}})$ (figs (a) and (b)) and~$\frac{\partial \hat{p}^-(\hat{p}_j^{\pi_u},m,\alpha)}{\partial \hat{p}_j^{\pi_u}}$ Versus~$\hat{p}_j^{\pi_u} \in [0,1]$ for different value of~$alpha$ and~$m$.}
\label{fig:numerically_p_plus}
\end{figure}

Specifically, recall that we used $f(x)$ to denote $\hat{p}^-(x,m,\alpha)$.
Thus, we wish to show that
$$\frac{\partial \hat{p}^-(\hat{p}_j^{\pi_u},m,\alpha)}{\partial \hat{p}_j^{\pi_u}},\frac{\partial^2 \hat{p}^-(\hat{p}_j^{\pi_u},m,\alpha)}{\partial^2 \hat{p}_j^{\pi_u}} >0),\forall \hat{p}_j^{\pi_u} \in [0,1].$$
This is demonstrated in Fig.~\ref{fig:numerically_p_plus} for different values of $m$ and $\alpha$.
\end{color}
\end{proof}


\paragraph*{Lemma~\ref{lemma:Bounding executed path's sub-optimal coverage}---implications}
Recall that Lemma~\ref{lemma:Bounding executed path's sub-optimal coverage} states that the for any desired CL, and regardless of the values of $m$ and $\kappa$, the minimum lower bound on the executed path's coverage is 
$
    \min_{\hat{\rm{IPV}}(\pi_{u})} \vert \bar{\mathcal{S}}^-({\pi}_{u}) \vert = k \cdot \hat{p}^-(\kappa,m,\alpha)
$.
%
This allows us to provide guidelines on how too choose the algorithm's parameters $m$ and $\kappa$ according to the desired CL which is application specific.
%
As an example, in Fig.~\ref{fig:CI lower bound of the POI coverage} we plot~$\hat{p}^-(\kappa,m,\alpha)$ for $\alpha = 0.05$ for various values of~$m$ and~$\kappa$.
%
Now, consider a user requirement that the POI coverage of the executed path will exceed~$93[\%]$ with a CL of~$95[\%]$ (\i.e., $\alpha = 0.05)$.
This corresponds to choosing any point on the line of~$93[\%]$ which can be, e.g.,~$m=70$ and~$\kappa = 0.99$ or~$m=95$ and~$\kappa=0.98$.


% It allow as to calculate only~$\hat{p}^-(\kappa,m,\alpha) =\frac{\vert \bar{\mathcal{S}}({\pi}_{u}) \vert}{k} $ and represent the minimum lower bound of the executed path's sub-optimal coverage in percentage.
% For instance, consider a user requirement that the POI execution coverage will exceed~$93[\%]$ with CL of~$95[\%]$ (\i.e., $\alpha = 0.05)$.
% Thus, assuming a user requirement to have a CL of~$95[\%]$ (\i.e., $\alpha = 0.05)$.
% Then, we can display in Fig.\ref{fig:CI lower bound of the POI coverage} the value of~$\frac{\vert \bar{\mathcal{S}}({\pi}_{u}) \vert}{k}$ in percentage  versus~$\kappa$ and~$m$.
% As a result, the user can choose some combination of~$m$ and~$\kappa$ to achieve a POI coverage requirement.
% For instance, if the user requirements is to result with~$\frac{\vert \bar{\mathcal{S}}({\pi}_{u}) \vert}{k} \geq 93[\%]$ it can be achieved by run \irisuu with some combination of~$\kppa$ and~$m$~(e.g.,~$\kappa = 0.99$ and~$m=70$ or~$\kappa = 0.98$ and~$m=95$ etc.). 

\begin{figure}[tb]
    \centering
     \includegraphics[width=0.5\textwidth]{figs/paretoCI.eps}
     \caption{
     Values (in percentage) of~$\hat{p}^-(\kappa,m,\alpha)$ for~$\alpha = 0.05$
     as a function of 
     the number of MC samples~$m$ ($x$-axis) and
     the coverage approximation factor~$\kappa$.
    }
\label{fig:CI lower bound of the POI coverage}
\end{figure}


\vspace{2mm}
\begin{lemma}[\parbox{0.48\linewidth}{\centering {Bounding executed path's \\ collision probability}}]
% \begin{lemma}[Bounding executed path's collision probability]
\label{lemma:Bounding executed path's collision}
~

Let~$\pi_{u}$ be the \ap of the goal node~$n^\text{goal}$
and~$\hat{\mathcal{C}}(\pi_u)$ be the estimated collision probability of~$n^\text{goal}$.
%
Then, for any desired CL of~$1 - \alpha$, with~$\alpha \in [0,1]$, 
the expected collision probability of the executed path~~$\bar{\mathcal{C}}(\pi_u)$ has an upper bound of: 
% 
\begin{equation}\label{eq:lemma2-collision}
    \bar{\mathcal{C}}(\pi_u)^+ = \hat{p}^+(\hat{\mathcal{C}}(\pi_u),m,\alpha). 
\end{equation}
% \begin{equation}\label{eq:lemma2-collision}
%     \bar{\mathcal{C}}(\pi_u) \in 
%     \left[ 
%     \hat{p}^-(\hat{\mathcal{C}}(\pi_u),m,\alpha),
%     \hat{p}^+(\hat{\mathcal{C}}(\pi_u),m,\alpha)
%     \right].
% \end{equation}
Here, the function~$\hat{p}^+$ is defined in Eq.~\ref{eq:Clopper-Pearson method}. 
\end{lemma}

\vspace{2mm}
\begin{proof}
We treat the executed path's collision probability as a random variable and recall that~$\hat{\mathcal{C}}(\pi_u)$ represents the collision probability of~$\pi_{u}$ given~$m$ samples.
Thus, Eq.~\ref{eq:lemma2-collision} is an immediate application of the Clopper-Pearson method~(see Eq.~\ref{eq:Clopper-Pearson method}).

That is, During the planning, there may be multiple optional paths available which can increase the likelihood of a false-negative outcome of the resulting path that indicates no collision even though a collision has actually occurred.
In particular, suppose we have~$n$ different optional paths where~$\pi_u$ is one of them.
Then for each optional path~$\pi'$, we have a probability of~$\alpha$ that~$
\bar{\mathcal{C}}(\pi')^+ > \hat{p}^+(\hat{\mathcal{C}}(\pi'),m,\alpha)$.
Thus, the probability of a false negative in the resulting path is~$1-(1-\alpha)^n$. 
% In our implementation instead of counting the possible optional paths we choose to repeat multiple time the collision calculation of each edge and save its maximum value. Then, in the termination criteria, we re-calculate the value of~$\hat{\mathcal{C}}(\pi_u)$ by each~$\zeta_{u \rightarrow v}^{\text{max}}$ (see sec.\ref{subsec:Termination criteria}).
% Thus, we can use the original value of~$\alpha$ to calculate the upper bound of the expected collision probability.
% Thus, if we have~$n$ optional paths, following Bonferroni et al.~\cite{weisstein2004bonferroni} the upper bound is defined by~$\frac{\alpha}{n}$ instead of~$\alpha$.
% In our implementation instead of counting the possible optional paths we choose to repeat multiple time the collision calculation of each edge and save its maximum value. Then, in the termination criteria, we re-calculate the value of~$\hat{\mathcal{C}}(\pi_u)$ by each~$\zeta_{u \rightarrow v}^{\text{max}}$ (see sec.\ref{subsec:Termination criteria}).
% Thus, we can use the original value of~$\alpha$ to calculate the upper bound of the expected collision probability.
\DA{maybe I have a counterexample :( what to do with a square roadmap~$A-B-C-D$ and we want to reach from~$A$ to~$D$ where there are two optional paths: (i) $A-B-D$ (ii)~$A-C-D$. In that case, if we don't count the possible paths, then in our implementation we check each edge only once. }.
\end{proof}

\paragraph*{Lemma~\ref{lemma:Bounding executed path's collision}---implications}
Similar to Lemma~\ref{lemma:Bounding executed path's sub-optimal coverage}, Lemma~\ref{lemma:Bounding executed path's collision} can be used as a guideline on how to choose the algorithm's parameters~$m$ and~$\rho_\text{coll}$ 
according to the desired CL.
%
As an example, in Fig.~\ref{fig:paretoCICollision} we plot~$\hat{p}^+(\rho_\text{coll},m,\alpha)$ for~$\alpha=0.05$ and various values of~$m$ and $\rho_\text{coll}$.
%
Now, consider a user requirement that the executed path's collision probability does not exceed $7[\%]$ with a CL of~$95[\%]$ (i.e.,~$\alpha=0.05$). This can be achieved by selecting a point on the~$7[\%]$ line, for instance,~$m=94$ and~$\rho_\text{coll}=0.02$.

% In this case, we aim in limiting the collision probability such that~$\hat{p}^+(\rho_\text{coll},m,\alpha)$ that can be denoted as~$\bar{\mathcal{C}}^-(\pi_u)$ will be lower than a desired value.
% %
% As an illustration, Fig.~\ref{fig:paretoCICollision} displays~$\bar{\mathcal{C}}^-(\pi_u)$ for a CL of~$\alpha=0.05$ and different values of~$m$ and $\rho_\text{coll}$. Suppose the user wants to ensure that the executed path's collision probability does not exceed $5[\%]$ with a CL of~$95[\%]$ (i.e., $\alpha=0.05$). This can be achieved by selecting a point on the~$5[\%]$ dashed line, for instance,~$m=102$ and~$\rho_\text{coll}=0.01$.
%

% \OS{OLD TEXT: what is $\kappa$ doing here?}
% Now recall that the user can choose a threshold value~$\rho_\text{coll}$ in order to require that the estimated collision probability~$\colProbHat{_{,u}}$ will be at most the value of~$\rho_\text{coll}$.
% However, the value of~$\colProbHat{_{,u}}$ is estimated with only a limited number of~$m$ MC samples and according to lemma~\ref{lemma:Bounding executed path's collision} its upper bound is defined by~$\hat{p}^+(\colProbHat{_{,u}},m,\alpha)$.
% Thus, we wish to allow the user to choose for each iteration of \irisuu the minimal tuple~$\langle \kappa,m,\alpha \rangle$ such that we can be sure that the expected collision probability~$\colProbBar{_{,u}}$ will be lower than a desire value.
% Thus, assuming a user requirement to have a CL of~$95[\%] alpha = 0.05)$.
% Then, we can display in Fig.\ref{fig:paretoCICollision} the minimum value of~$\hat{p}^+(\colProbHat{_{,u}},m,\alpha)$ versus~$\rho_\text{coll}$ and~$m$.
\begin{figure}[tb]
    \centering
     \includegraphics[width=0.5\textwidth]{figs/paretoCICollision.eps}
     \caption{Values (in percentage) of~$\hat{p}^+(\rho_\text{coll},m,\alpha)$ for~$\alpha = 0.05$ as a function of 
     the number of MC samples~$m$ ($x$-axis) and
     the coverage approximation factor~$\rho_\text{coll}$.}
\label{fig:paretoCICollision}
\end{figure}





\begin{lemma}[Bounding executed path's expected length]
\label{lemma:Bounding executed path's expected length}
Let~$\pi_{u}$ be the \ap of the goal node~$n^\text{goal}$.
Furthermore, let~$\hat{\ell}(\pi_u)$ and~$\hat{s}_{\hat{\ell}}(\pi_u)$ be the average and standard deviation of~$\pi_{u}$'s length, respectively.
%
Then, for any desired CL of~$1 - \alpha$, with~$\alpha \in [0,1]$, 
the expected collision probability of the executed path~~$\bar{\mathcal{C}}(\pi_u)$ is bounded such that: 
%
\begin{equation}
\label{eq:CI-length-lemma1}
    \bar{\ell}(\pi) \in \left[\bar{X}^-(\hat{\ell}(\pi_u),m,\alpha), \bar{X}^+(\hat{\ell}(\pi_u),m,\alpha) \right].
\end{equation}
Here,~$\bar{X}^-$ and~$\bar{X}^+$ are defined in Eq.~\ref{eq:Mean of a population} and require the estimated standard deviation~$\hat{s}_{\hat{\ell}}(\pi_u)$ to be available.
\end{lemma}

\begin{proof}
We treat the executed path's expected length as random variable and recall that~$\hat{\ell}(\pi_u)$ and~$\hat{s}_{\hat{\ell}}(\pi_u)$ are the average and standard deviation of~$\pi_{u}$'s length given~$m$ samples.
%
Thus, Eq.~\ref{eq:CI-length-lemma1} is an immediate application of Eq.~\ref{eq:Mean of a population-base}.
\end{proof}

\paragraph*{Lemma~\ref{lemma:Bounding executed path's expected length}---note}
Both Lemma~\ref{lemma:Bounding executed path's sub-optimal coverage} and 
Lemma~\ref{lemma:Bounding executed path's collision} gave clear guidelines on how to choose algorithms parameters for desired confidence levels.
%
This was possible because there exists a bound on the best possible outcome (i.e., $100[\%]$ coverage of POIs and  $0[\%]$ collision probability) and the system parameters $\kappa$ and $\rho_\text{coll}$ are defined with respect to these bounds.
%
In contrast, there is no a-priori bound on the path length and the system parameter $\eps$ is only defined with respect to the (unknown) optimal length (i.e.,  $\hat{\ell}_u \leq~(1+\epsilon) \cdot \tilde{\ell}_u$).
%
However, for the path length we can bound the estimated variance~$\hat{s}_{\hat{\ell}}$ using Eq.~\ref{eq:variance_bound_Sheskin} which is done in the following Lemma.

\begin{lemma}[\parbox{0.58\linewidth}{\centering {Bounding the variance of \\ executed path's expected length}}]
\label{lemma:Bounding executed path's expected variance length}
~

Let~$\pi_{u}$ be the \ap of the goal node~$n^\text{goal}$
and let~$\hat{s}_{\hat{\ell}}(\pi_u)$ be the standard deviation of~$\pi_{u}$'s length.
%
Then, for any desired CL of~$1 - \alpha$, with~$\alpha \in [0,1]$, 
the variance of the expected path length~$\bar{s}_{\hat{\ell}}^2$ is bounded such that: 
%
\begin{equation}\label{eq:CI-length-variance}
    \bar{s}_{\hat{\ell}}^2 \in \left[\bar{s}^-(\hat{s}_{\hat{\ell}},m,\alpha), \bar{s}^+(\hat{s}_{\hat{\ell}},m,\alpha) \right].
\end{equation}
Here,~$\bar{s}^-$ and~$\bar{s}^+$ are defined in Eq.~\ref{eq:variance_bound_Sheskin}.
\end{lemma}

\begin{proof}
We treat the executed path's expected length as a random variable and recall that~$\hat{s}_{\hat{\ell}}(\pi_u)$ is the standard deviation of~$\pi_{u}$'s length given~$m$ samples.
%
Thus, Eq.~\ref{eq:CI-length-variance} is an immediate application of Eq.~\ref{eq:variance_bound_Sheskin}.
\end{proof}

\OS{Note to self---continue here}

% Based on Lemma~\ref{lemma:Bounding executed path's expected length} and~\ref{lemma:Bounding executed path's expected variance length} we can take the sigma level objective (see sec~\ref{subsec:Monte-Carlo methods statistical tests}):

 \vspace{2mm}
\begin{lemma}[\parbox{0.48\linewidth}{\centering {Bounding executed path's \\ expected possible length}}]
% \begin{lemma}[Bounding executed path's expected possible length]
\label{lemma:Bounding executed path's expected possible length}
~ 

Let~$\pi_{u}$ be the \ap of the goal node~$n^\text{goal}$ and let~$\hat{\ell}(\pi_u)$ and~$\hat{s}_{\hat{\ell}}$ be the average path length and the standard deviation of the~$m$ execution paths~$\Pi^e_{u}$ that follows~$\pi_{u}$ as a command path, respectively.
In addition, let~$\bar{X}^-(\hat{\ell}(\pi_u),m,\alpha)$ and~$\bar{X}^+(\hat{\ell}(\pi_u),m,\alpha)$ be the CI bound of~$\hat{\ell}(\pi_u)$ (see Lemma~\ref{lemma:Bounding executed path's expected length}. 
Similarly, let~$\bar{s}^-(\hat{s}_{\hat{\ell}},m,\alpha)$ and~$\bar{s}^+(\hat{s}_{\hat{\ell}},m,\alpha)$ be the CI bound of~$\hat{s}_{\hat{\ell}}$ (see Lemma~\ref{lemma:Bounding executed path's expected variance length}. 
Then, for any~$\alpha \in [0,1]$ we say with CL of~$1-\alpha$ that we have a safety probability~$p_{\text{sig lvl}}(n)$ that any possible value of the path length will be within in a CI such that:
\begin{equation}\label{eq:CI_sigma_level_possible}
\begin{split}
    \text{Pr}[X] \in 
    ([ &\bar{X}^-(\hat{\ell}(\pi_u),m,\alpha) - n \bar{s}^+(\hat{s}_{\hat{\ell}},m,\alpha), \\
    &\bar{X}^+(\hat{\ell}(\pi_u),m,\alpha) + n \bar{s}^+(\hat{s}_{\hat{\ell}},m,\alpha)
    ])
    \geq p_{\text{sig lvl}}(n).
\end{split}
\end{equation}
Where~$n$ is the sigma level and~$p_{\text{sig lvl}}(n)$ is the safety probability as detailed in the explanation of Eq.\ref{eq:CI_sigma_level}.
\end{lemma}

\vspace{2mm}
\begin{proof}
We treat the executed path's expected length as a random variable and recall that~$\hat{\ell}(\pi_u)$ and~$\hat{s}_{\hat{\ell}}(\pi_u)$ are the mean and standard deviation of~$\pi_{u}$'s length, respectively, given~$m$ samples.
%
Thus, Eq.~\ref{eq:CI_sigma_level_possible} is an immediate application of Eq.~\ref{eq:CI_sigma_level}.
\end{proof}

% \DA{We need to think about it a lot. Because~$\bar{\ell}(\pi)$ and~$\bar{s}_{\hat{\ell}}$ are not an exact value there is only a CL for it.
% Thus, maybe the value of~$p_{\text{sig lvl}}(n)$ need to be updated following this CL in~\cite{shimoyama2008development}}



% Notice that the bounding executed path's sub-optimal \textbf{length}, requires addressing the standard deviation of the \pap path length during the search and can be done in future work. 




==> sections/RelatedWork.tex <==
\section{Related Work}
\label{Sec:RelatedWork}
\subsection{Localization uncertainty}
Localization uncertainty is one of the main reasons of planning uncertainty. 
It can be solved using a variety of methods such as extended Kalman filter (EKF), and particle filter (PF)~\cite{pf_ekf} that used to computes the posterior distribution. 
The EKF approximates the posterior distribution using a covariance matrix~$P$  which is updated according to the estimated motion states and sensor measurements. 
The state variables are propagates using the equations of motion, and the received measurement is used to update both the estimated states and the covariance matrix.
The PF approximates the posterior distribution with a discrete density of~$N$ particles, which serves as hypotheses for the possible location. 
As long as no new sensors measurement is received, the particles states is updated according to a motion model. 
When a measurement receives, each particle get a suitable weight that represents its adjustment to the measurement and used for a re-sampling of the particles states.

\subsection{Planning under uncertainty}
Planning under uncertainty, in its general form, can be formulated as a partially observable markov decision making (POMDP) problem. POMDP is an extension of an MDP which model the system dynamics with a hidden Markov model that connects unobservant system states to observations.
The agent goal is to maximize a reward with sequence of actions that change the system states.
Each discrete point in time, the agent can get an observations that depend on the current state. The agent uses these observations to form a belief state which is expressed as a probability distribution over the states.
This method is very common in many applications such that artificial intelligence and automated planning~\cite{POMDP}. MOMDPs stand between MDPs and POMDPs. In MOMDPs some state components are fully observable and known with certainty, whereas some others are partially observable~\cite{MOMDP}. The distinction amongst fully and partially observable state components allows for a factored representation that reduces the high dimensional of the belief space.

\subsection{Closed or open loop planning}
The planning generates a sequence of actions to take from the initial state and it can be either closed or open loop. The open-loop system is often called the non-feedback system in which the sequence of actions and states' change is determined only according to a predetermined model (deterministic or stochastic).
In the closed-loop system, measurements and observations are also considered. 
In most cases, the use of the observations helps to get more accurate planning, however, usually entails a high computational cost. 
POMDP and MOMDP methods are closed-loop system which update the states and actions depending on the observation. The EKF and PF are also closed-loop system that use the observation to update the covariance matrix or to re-sample the particles.

The use of observations in path planning is very effective in online planning during execution or simulation. 
However, in each simulation different observations are obtained. Thus, the planning is performed several times with different simulations where the goal is to test the solution quality by the paths variety.
In the case of a safe path requirement, we would like to examine which the paths are within a safety volume and do not collide with obstacles~\cite{Safe_path_planning6},~\cite{localization_inspection_goal}. 
Checking the solution several time with a different simulation can provide reliable information about the safety probability of the path. Finally, once a variety of safe paths are obtained, we can randomly select one of the paths (or run the planning on the observations of the execution).
However, In the inspection scenario, even small location errors can cause the POI to be missed or hidden with an obstacle. That is, in different simulations we may get completely different paths.
Thus, we choose to consider our problem as an open-loop system without observations. This will give us the ability to consider different possible paths within one planning process.
 








==> sections/Results.tex <==
\section{Results}
\label{Sec:Results}

In this result we assume that the roadmap~$G$ is predetermined. However, \irisuu continues the IRIS approach to incrementally increasing optimal demands. That is, according to the MC theory (detailed in subsection~\ref{subsec:Monte Carlo methods}), to get an optimal solution we need to choose~$m \rightarrow \infty$. However, using a large number of samples during the search will significantly increase the computation time. Thus, initially, we will perform a search with a relatively low number of~$m$. Then, as time allows, we will gradually increase~$m$ so the solution converges asymptotically to the optimal solution.

\subsection{The toy scenario results}
 
Table~\ref{tbl:Toyscenarioresults} show the results of the toy scenario. 
~
\begin{table}[h!]
\centering
\begin{tabular}{|p{2.9cm}|p{1.2cm}|p{2.5cm}|  }
\hline
Method & POI success [\%] &  Generated nodes [\#] \\
\hline
IRIS & 66 &1.456e4 \\
Minimization of localization uncertainty & 93   & 1.543e5 \\
Limitation of localization uncertainty & 95 &1.915e4 \\
\irisuu [5 MC] &96 & 1.196e5 \\
\irisuu [10 MC]     &96 & 5.378e5 \\
\irisuu [20 MC]  & 97 & 1.380e6 \\
\irisuu [90 MC] & 99 & 2.600e10   \\

\hline

\end{tabular}
\caption{Toy scenario results}
\label{tbl:Toyscenarioresults}
\end{table}

The reference algorithm achieves only~$66[\%]$ POI success. 
In contrast, the other methods yielded significantly good results.
The minimizing approach results in with~$93[\%]$ POI success but with a significant increase of the calculation time. 
The Limitation approach improves the results up to~$95[\%]$ POI success even without significantly increasing the calculation time. 
We will note that this is the maximum possible to achieve with these methods under the conditions of this scenario.
In contrast, this result can be further improved through the \irisuu algorithm and yield~$96[\%]$ POI success for~$5$ MC samples till~$99[\%]$ for 90 MC samples.
% In addition, as the number of samples increases so does the level of certainty and the probability of success in the simulation converges asymptotically to the optimal solution.
However, in this scenario, the improvement entails a relatively high computational cost for the resulting improvement.

% According to the theory of CL and CI, the use of a large number of samples improves both the mean and the standard deviation as can be seen in Figure~\ref{fig:boxplotPOI_TOY} (todo update the fig, maybe use more than 20 MC in the simulation).

% \begin{figure}[h!]
%     \centering
%      \includegraphics[width=0.5\textwidth]{figs/boxplotPOI_TOY.png}
%     %  \caption{Each Monte Carlo sample has 3 steps: (1) A navigation model that calculates the possible location errors for the next vertex~$k+1$. (2) Updating the possible location. (3) Calculate the cost and POI. Finally, all samples are used to calculate the $Cost,POI$ expectation.}
%     \caption{Box plot of $\text{ \irisuu of toy scenario}
     
% \label{fig:boxplotPOI_TOY}
% \end{figure}

\subsection{The bridge scenario results}



\subsection{Near-optimal planning under localization uncertainty }

\textbf{TODO - run and test results} 
As can be seen, the results of \irisuu yield high percentages of POI, however, the computational cost is large so that above~$5$ MC it becomes significantly high. 
In order to ensure the solution quality (CL and CI), we would like to use a larger number than 5 MC samples.
To this end, our proposal is to use IRIS ability to provide near-optimal planning and run \irisuu with the demand POI less than ~$100[\%] (p<1)$.
That is, If we can settle for less than 100 percent success then the running time is significantly shortened.
This means that on the one hand, we require less POI. However, on the other hand, because of the faster computation time, we will be able to plan a path that produces more POI per time in the execution and a higher level of solution quality.






% \begin{table}[h!]
% \centering
% \begin{tabular}{|p{2.9cm}|p{1.2cm}|p{2.5cm}|  }
% \hline
% Method & $I_{\text{success}}$ &  Generated nodes [\#] \\
% \hline
% Reference & 70 &2.971e4 \\
% 1:0.8 &83 & 1.172e5 \\
% 0.9:0.7      &92 & 5.139e5 \\
% 0.8:0.6   & 93 & 4.019e6 \\
% 0.7:0.5  & 97 & 1.455e7   \\

% \hline

% \end{tabular}
% \caption{Bridge scenario - probability function}
% \label{tbl:Toyscenarioresults}
% \end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{|p{2.9cm}|p{1.2cm}|p{2.5cm}|  }
% \hline
% Method & $I_{\text{success}}$ &  Generated nodes [\#] \\
% \hline
% Reference & 70 &2.971e4 \\
% 1:0.8 &76 & 4.662e4 \\
% 0.9:0.7      &89 & 3.046e5 \\
% 0.8:0.6   & 92 & 7.594e5 \\
% 0.7:0.5  & 95 & 2.554e6   \\

% \hline

% \end{tabular}
% \caption{Near-Optimal - Bridge scenario - probability function}
% \label{tbl:Toyscenarioresults}
% \end{table}






==> sections/referencearc.tex <==

% @article{gustafsson2010particle,
%   title={Particle filter theory and practice with positioning applications},
%   author={Gustafsson, Fredrik},
%   journal={IEEE Aerospace and Electronic Systems Magazine},
%   volume={25},
%   number={7},
%   pages={53--82},
%   year={2010},
%   publisher={IEEE}
% }

% @incollection{POMDP,
%   title={Planning and acting in partially observable stochastic domains},
%   author={Kaelbling Leslie Pack, Littman Michael L, Cassandra Anthony R},
%   publisher = { Artificial Intelligence, vol 101},
%   pages={99-134},
%   year={1998}
% }

% @incollection{MOMDP,
%   title={POMDP and MOMDP solutions for structural life-cycle cost minimization under partial and mixed observability},
%   author={Papakonstantinou Konstantinos G, Andriotis Charalampos P, Shinozuka Masanobu},
%   publisher = {Structure and Infrastructure Engineering, vol 14},
%   pages={869-882},
%   year={2018}
% }
  
% @article{szrek2021accuracy,
%   title={Accuracy evaluation of selected mobile inspection robot localization techniques in a gnss-denied environment},
%   author={Szrek, Jaros{\l}aw and Tryba{\l}a, Pawe{\l} and G{\'o}ralczyk, Mateusz and Michalak, Anna and Zi{\k{e}}tek, Bart{\l}omiej and Zimroz, Rados{\l}aw},
%   journal={Sensors},
%   volume={21},
%   number={1},
%   pages={141},
%   year={2021},
%   publisher={Multidisciplinary Digital Publishing Institute}
% }


 
%  @incollection{AutonomousExplorationandInspectionPath,
% author={Christos Papachristos,Mina KamelMarija ,PopovićShehryar KhattakAndreas ,BircherHelen OleynikovaTung ,DangFrank MascarichKostas ,AlexisEmail}
% title={Autonomous Exploration and Inspection Path Planning for Aerial Robots Using the Robot Operating System},
% bookTitle={Robot Operating System (ROS): The Complete Reference (Volume 3)},
% year={2019},
% publisher={Springer International Publishing},
% pages={67-111},
% }

% @INPROCEEDINGS{AutonomousExplorationandInspectionPath, 
% author = "{A. Bircher, K. Alexis, M. Burri, P. Oettershagen, S. Omari, T. Mantel and R. Siegwart}",
% booktitle = {Robotics and Automation (ICRA), 2015 IEEE International Conference on}, 
% title={Structural Inspection Path Planning via Iterative Viewpoint Resampling with Application to Aerial Robotics},
% year={2015}, 
% month={May}, 
% pages={6423-6430}, 
% }

% @incollection{confidenceinterval,
%   title={Using the confidence interval confidently},
%   author={Hazra, Avijit},
%   publisher = { Journal of Thoracic Disease},
%   year={2017}
% }

 


% @incollection{IMU_only,
%   author={D. H. Titterton and J. L. Weston},
%   title={Strapdown Inertial Navigation Technology -2nd Edition The Institution of Electrical Engineers},
%   year={2006},
%   publisher={IEEE Aerosp. Electron. Syst. Mag., vol. 20, no. 7}
%   pages={33–34}
% }

% @incollection{lee2017introduction,
%   title={Introduction to Navigation Systems},
%   author={Lee, Junghyun},
%   booktitle={Multi-purposeful Application of Geospatial Data},
%   year={2017},
%   publisher={IntechOpen}
% }

% @incollection{Sphere-Sphere-Intersection,
% title={Sphere-Sphere Intersection},
%   author={Wolfram MathWorld},
%   year={2021},
%   publisher={https://mathworld.wolfram.com/Sphere-SphereIntersection.html}
% }

% @incollection{Groves,
%   author={Groves, Paul},
%   title={Principles of GNSS, Inertial, and Multisensor Integrated Navigation Systems, Second Edition},
%   year={2013},
%   publisher={Artech}
% }
% @incollection{GNSS_availability,
%   author={Kleijer Frank ,Odijk Dennis, Verbree Edward},
%   title={Prediction of GNSS availability and accuracy in urban environments case study schiphol airport},
%   year={2009},
%   publisher={Location Based Services and TeleCartography II}
% }
 
 % @incollection{Safe_path_planning6,
%   title={Solving path planning problems in urban environments based on a priori sensor availability and execution error propagation},
%   author={Delamer Jean-Alexis, Watanabe Yoko},
%   publisher = { AIAA SciTech Forum, San Diego, California},
%   year={2019}
% }
